Advancing Model Pruning via Bi-level Optimization

The deployment constraints in practical applications necessitate the pruning of large-scale deep learning models, i.e., promoting their weight sparsity. As illustrated by the Lottery Ticket Hypothesis (LTH), pruning also has the potential of improving their generalization ability. At the core of LTH, iterative magnitude pruning (IMP) is the predominant pruning method to successfully find 'winning tickets'. Yet, the computation cost of IMP grows prohibitively as the targeted pruning ratio increases. To reduce the computation overhead, various efficient 'one-shot' pruning methods have been developed, but these schemes are usually unable to find winning tickets as good as IMP. This raises the question of how to close the gap between pruning accuracy and pruning efficiency? To tackle it, we pursue the algorithmic advancement of model pruning. Specifically, we formulate the pruning problem from a fresh and novel viewpoint, bi-level optimization (BLO). We show that the BLO interpretation provides a technically-grounded optimization base for an efficient implementation of the pruning-retraining learning paradigm used in IMP. We also show that the proposed bi-level optimization-oriented pruning method (termed BiP) is a special class of BLO problems with a bi-linear problem structure. By leveraging such bi-linearity, we theoretically show that BiP can be solved as easily as first-order optimization, thus inheriting the computation efficiency. Through extensive experiments on both structured and unstructured pruning with 5 model architectures and 4 data sets, we demonstrate that BiP can find better winning tickets than IMP in most cases, and is computationally as efficient as the one-shot pruning schemes, demonstrating 2-7 times speedup over IMP for the same level of model accuracy and sparsity.

==> Deprecated_NO_USE/Version_Camera_05161900/Sec3_SL.tex <==
In this section, we begin by providing a brief   background of neural  network pruning, including the predominant   iterative magnitude pruning (IMP) method and the 
associated lottery ticket hypothesis (LTH)
\cite{frankle2018lottery} to find high-quality subnetworks (known as `winning tickets') that--when trained in isolation--reach test accuracy comparable to or even better than the original dense network. 
However, the superior performance of IMP is accompanied with a prohibitive computation cost, as will be exemplified in Fig.\,\ref{fig: one_shot_results}. In  order to overcome the computational difficulty of IMP, we next introduce the  one-shot   pruning method and elaborate on its comparison with IMP. Spurred by the pros and cons of current pruning methods, we eventually state the problem to be studied in this paper. 
 

\paragraph{{Heuristics-based IMP.}}
The heuristics-based IMP is the  currently prevailing approach  to
identify the `winning ticket' in model pruning, so as to attain model sparsity without suffering  performance loss\,\cite{frankle2018lottery,Renda2020Comparing,frankle2020linear,blalock2020state,chen2020lottery,chen2021lottery}. 
For example, the current  state-of-the-art (SOTA) implementation of IMP in \cite{ma2021sanity} can lead to a pruned ResNet-20 on
% \SL{[This example  number needs to be   better aligned with the later figure, then you can cite it here.]}
CIFAR-10 with 74\% sparsity and $92.12\%$ test accuracy, {
which is comparable to the performance of the original dense model}; see Fig.\,\ref{fig: one_shot_results}. 
% For the larger-size {ResNet-18} model, IMP   can identify a sparser network with   {$95\%$ sparsity and $94.81\%$ test accuracy, yielding the $0.5\%$ improvement over the original dense model}; \SL{see Fig.\,xxx in Sec.\,xxx}.
The algorithm of IMP typically contains two key ingredients: \textbf{(i)} a \textit{temporally-evolved pruning schedule} (given by the growing model sparsity over pruning iterations), and \textbf{(ii)} the \textit{pruning-retraining learning mechanism} applied at each pruning round. 
% To be more specific, 
% IMP  repeatedly trains, prunes, and resets the network over multiple rounds (say $n$ rounds). 
For (i), supposing that there exist $n$ pruning rounds, each round  prunes $(p\%)^{\frac{1}{n}} $ of the model
weights that survive the previous round, where $p\%$ denotes the final pruning ratio to be achieved.
%This leads to a pruning mask $\mathbf m$ at each round. 
For (ii), 
the non-zero remaining weights at each pruning round are re-set to the  weights at initialization or at an early-training epoch \cite{Renda2020Comparing}, and   re-trained till convergence. 
In brief, IMP  repeatedly trains, prunes, and resets the network over multiple rounds. 

 

% A common example, the Lottery Ticket Hypothesis (LTH), can achieve comparable or even better performance with a sparsity of over $95\%$ in its state-of-the-art (SOTA) implementation\,\cite{ma2021SanityCheckLTH}. 
% In general, the heuristics-based IMP adopts a sparsifying-retraining paradigm which consists of multiple iterative cycles: \underline{\textit{(1)}} \textbf{training} dense model with several epochs; \underline{\textit{(2)}} \textbf{pruning} $p\%$ redundant model weights with certain heuristics-based criteria (\emph{e.g.} model weight magnitude) to obtain the new mask; \underline{\textit{(3)}} \textbf{fine-tuning} the sparse network with the found mask and rewound weights for accuracy recovery. 

\begin{wrapfigure}{r}{85mm}
\vspace*{-5mm}
\centerline{
\begin{tabular}{cc}
\hspace*{0mm}\includegraphics[width=.3\textwidth,height=!]{figure/performance_comparison.pdf}  
&\hspace*{-4mm}\includegraphics[width=.31\textwidth,height=!]{figure/time_comparison_long.pdf}
% \\
% \hspace*{2mm}\footnotesize{(a) Test accuracy vs. pruning ratio.} &   \footnotesize{(b) Runtime of pruning.}
\end{tabular}}
\vspace*{-2mm}
\caption{\footnotesize{
Illustration of the pros and cons of different pruning methods executed over (ResNet-20, CIFAR-10).
(a) Test accuracy vs. different pruning ratios: IMP significantly outperforms one-shot pruning methods (\textsc{OMP}\,\cite{frankle2018lottery}, \textsc{ProsPr}\,\cite{alizadeh2022prospect}, \textsc{Grasp}\,\cite{wang2020pick}, \textsc{Snip}\,\cite{lee2018snip}, \textsc{SynFlow}\,\cite{tanaka2020pruning}). (b) Computation time of pruning to different sparsity levels:  IMP becomes much more computational intensive when pruning is targeted for a higher sparsity level. 
%We highlight we adopt the SOTA implementation of OMP  following\,\cite{ma2021sanity} and other methods following their original settings.
% \SL{For (a): Update x-y axis and mark the $95\%$ or $99\%$ pruning point.}
% \SL{For (b): [X-axis: Pruning method, add the dense model training time.]}
% \SL{Illustration of  the pros and cons of different pruning methods executed over (ResNet-xxx, CIFAR-10).
% (a) Test accuracy against pruning ratio: IMP significantly outperforms one-shot pruning methods (OMP [refs], ....). (b) Computation time of pruning to different sparsity levels:  IMP becomes much more computational intensive when pruning is targeted for a higher sparsity level ($99\%$ vs. $60\%$).
% }
% Performance and efficiency comparison between IMP (LTH) and various one-shot pruning methods on CIFAR10 and ResNet20. One-shot methods save pruning time at the cost of significant performance drop compared to IMP (LTH).
% \SL{Why ResNet20? Not ResNet18?}
}}
  \label{fig: one_shot_results}
  \vspace*{-7mm}
\end{wrapfigure}

%\SL{[I stop here]}
Yet, the superior pruning accuracy   of IMP is at the cost of  computation efficiency. For ease of illustration, Fig.\,\ref{fig: one_shot_results} shows the example of pruning ResNet-20 over CIFAR-10 and demonstrates   the accuracy and the computation time of various pruning methods versus the growing sparsity ratio.
%and (b) the computation time of model pruning with different sparsity levels.
% \SL{For ease of illustration, Fig.\,\ref{fig: one_shot_results} shows a pruning example that unveils (a) the accuracy performance of various pruning methods versus the growing sparsity ratio, and (b) the computation time of model pruning with different sparsity levels.}
As we can see, IMP outperforms   the other pruning baselines and finds 
the sparsest winning ticket (marked by the red star in Fig.\,\ref{fig: one_shot_results}a) using $n = 6$ pruning rounds. 
However, this leads to $3\times$ more than the cost of training a dense model from scratch.
% \SL{the $95\%$-sparsity ResNet-18 model with $94.81\%$ test accuracy on CIFAR-10 takes $n = xxx$ pruning rounds. This leads to $xxx$-min runtime, which is $xxx$ times higher than training a dense model and $xxx$ times higher than pruning to the $60\%$  sparsity level.} 
%and thus hampers the pruning efficiency 
%
\iffalse
Although IMP-based pruning approaches have become the rising star sub-field in pruning, its current success largely sacrifices the pruning efficiency. Within each pruning cycle, the sparse structure is obtained by removing a small fixed pruning ratio (\emph{e.g.}, $20\%$ in LTH) of the \textbf{remaining weights} to make the final sparse model match the full performance of the dense model. Thus, the required pruning iterative numbers as well as their training time grow exponentially as the sparsity increases. For example, the SOTA implementation of LTH\,\cite{ma2021SanityCheckLTH} has to go through 22 pruning cycles to arrive at a sparsity of $99\%$. In such a case, the immense training time consumption has become one clear obstacle of IMP from scaling to large model architectures and datasets\,\cite{zhang2021efficient}.
\fi 
%
\paragraph{IMP vs. one-shot pruning.}
To reduce the computation cost of IMP, different kinds of `accelerated' pruning methods were developed  \cite{zhang2021efficient, frankle2018lottery, wang2020pick,lee2018snip,tanaka2020pruning, alizadeh2022prospect}; And many of them
  fall into the \textit{one-shot pruning} category: The network is directly pruned to the eventual target sparsity level  and retrained once. 
%: the network is trained once, p% of weights are pruned, and the surviving weights are reset.
% which refines the sparse mask directly to the given sparsity only one time. 
In particular, the one-shot magnitude pruning (OMP) has been served as an important baseline that  simplifies IMP directly \cite{frankle2018lottery}.
\textsc{OMP} obeys the pruning-retraining paradigm, but it  prunes the model to the target sparsity using only one pruning round. 
% \SL{Although some existing work\,\cite{ma2021SanityCheckLTH} observed that OMP and the other one-shot pruning methods (e.g., ProsPr\,\cite{alizadeh2022prospect}) could find winning tickets and achieve similar accuracy performance to IMP. However, this conclusion is model/dataset-specific. }
% Although some preliminary results showed that 
% existing work\,\cite{ma2021sanity}(\YH{cite TBD}) observed that OMP and the other one-shot pruning methods (e.g., \textsc{ProsPr}\,\cite{alizadeh2022prospect}) could find winning tickets and achieve similar accuracy performance to IMP at low sparsity levels. However, this conclusion is model/dataset-specific. 
However,  the promise of current one-shot pruning methods is dataset/model-specific \cite{ma2021sanity, su2020sanity_random_win} and mostly lie in the low-sparsity regime \cite{alizadeh2022prospect}.
As systematically studied in \cite{frankle2020pruning,ma2021sanity}, there exists a clear performance gap between one-shot pruning and IMP.
Fig.\,\ref{fig: one_shot_results} also justifies the above limitation.
% However, the degradation in accuracy of the one-shot methods is still significant compared to IMP (LTH), making them impractical to real world applications\,\cite{frankle2020pruning}.
As we can see, although one-shot pruning  is   computationally light (Fig.\,\ref{fig: one_shot_results}b), it suffers from an evident accuracy drop compared to IMP (Fig.\,\ref{fig: one_shot_results}a), especially at the large sparsity levels.
%For example, \textsc{OMP} and \textsc{ProsPr} \cite{alizadeh2022prospect}, the SOTA methods of one-shot pruning,   yield  over $2\%$ and $10\%$ accuracy drop compared to IMP at the $74\%$ and  $98\%$ sparsity level, respectively.
Thus,  there exists a strong demand for the algorithmic advancement of model pruning that can   enjoy the dual advantages of one-shot pruning and IMP.
%\textit{i.e.}, improve the tradeoff  between computation efficiency and pruning accuracy. 
% Even the SOTA one-shot pruning method \textsc{ProsPr}\,\cite{alizadeh2022prospect} also suffers from an accuracy drop of over $10\%$ compared to IMP when $99\%$ parameters are pruned.
% As demonstrated in Figure\,, all one-shot  
%\todo{I don't see 99\% sparsity level in Figure~\ref{fig: one_shot_results}. Do we mean 90\%?
%
%\YY{Solved.}}
%
%the observed accuracy-efficiency tradeoff
%the accuracy-efficiency tradeoff of one-shot pruning is based on the heuristics-based one-shot pruning 
%This efficiency-performance trade-off is primarily due to the heuristic nature, which is insufficient to find satisfactory masks with an extreme sparsity using the radical pruning ratio as OMP does.
%
\paragraph{Problem Statement.}
As described above, the existing  one-shot pruning methods do not suffice to close the performance gap with IMP. One possible root cause is its strong   dependence   on  the heuristics-based weight sparsification strategy. This leaves the question of  whether 
computation efficiency and pruning accuracy could be co-improved through a more rigorous and dedicated optimization-based approach. 
% a theoretically-grounded optimization-based approach can renovate one-shot pruning so as to improve the computation complexity of pruning while attaining the accuracy performance comparable to IMP.
% Based on the aforementioned dilemma between performance and pruning cycle number in heuristics-based pruning methods, we ask the following question:
Thus, we ask:  \textit{Beyond heuristics, how to establish the \textbf{optimization basis} of a successful pruning mechanism that can attain high pruning  accuracy (like IMP) as well as high   computation efficiency (like one-shot pruning)?}
% \begin{center}
%     \textit{Beyond heuristics, how to establish the \textbf{optimization basis} of a successful pruning mechanism that can close the gap between pruning accuracy (e.g., achieved by IMP) and computation efficiency (e.g., achieved by OMP)?}
% \end{center}


%\newpage 


==> Deprecated_NO_USE/Version_Camera_05161900/Sec4_SL.tex <==
In this section, we   re-investigate the problem of model pruning through the lens of   bi-level optimization (BLO), and show that BLO  not only provides a natural interpretation of the pruning-retraining learning paradigm but also brings in additional   design flexibilities for model pruning.
Next, we establish  the algorithmic foundation of BLO-enabled model pruning (termed bi-level pruning or {\biprune}), extended from  the implicit gradient approach. Further, we     show that {\biprune} %is a special class of BLO problems and 
can be solved as easily as the first-order alternating optimization by taking advantages of the   bi-linear nature of the pruning variables. Lastly, we summarize the   {\biprune} algorithm and its   implementation details.  

% We will show the benefits as well as the mathematical challenges brought by the BLO formulation. Next, we point out that the bi-linearity of the pruning problem falls into a special class of the BLO and thus, can be solved as easily as the first-order alternating optimization. Finally, we propose {\biprune}, an efficient first-order BLO-based model weight pruning algorithm.

\paragraph{A BLO viewpoint on model pruning}
As described in Sec.\,\ref{sec: preliminary}, the pruning-retraining learning paradigm covers   two kinds of tasks: \ding{182} pruning  to determine the sparse pattern of model weights, and \ding{183} training remaining non-zero weights  to recover the model accuracy. 
In existing optimization-based pruning methods \cite{wen2016learning,zhang2018systematic,hoefler2021sparsity,wang2020proximal}, the tasks \ding{182}-\ding{183} are  achieved by merely  optimizing   model weights,   together with penalizing their sparsity-inducing norms, \textit{e.g.}, the $\ell_1$  and $\ell_2$ norms \cite{bach2012optimization}. Different from the above formulation, we propose to  separate optimization variables involved in the pruning tasks  \ding{182} and \ding{183}. This leads to    the (binary) pruning mask variable $\mask \in \{ 0, 1\}^n$ and the model weight variable $\btheta \in \mathbb R^n$, respectively. Here $n$ denotes the total number of model parameters. 
Accordingly, the pruned model is given by $(\mathbf m \odot  \btheta)$, where $\odot$ denotes the element-wise multiplication. As will be evident later, this  \textit{variable disentanglement} enables us to 
explicitly depict the co-evolving of pruning and retraining through BLO, and    helps us to    customize  the pruning task with high flexibility.
%so as to leverage more advanced optimization techniques to achieve a better pruning solution than heuristics-based search. 



% the model mask\,$\mask$ and the corresponding model weights\,$\btheta$. In the widely accepted sparsifying-retraining pruning paradigm, the masks $\mask$ are highly dependent on the model weights $\btheta$ as the magnitude of $\btheta$ serves as the pruning criterion. In the BLO formulation, $\mask$ and $\btheta$ are optimized independently using disparate variables. This \textit{disentanglement} gives the mask variables $\mask$ more flexibility to search better optima than the heuristics-based methods. More importantly, it facilitates us to interpret the sparsifying-retraining paradigm from a bi-level optimization viewpoint. 



In what follows, we elaborate on how BLO can be established to co-optimize the pruning mask $\mathbf m$  and the retrained sparse model weights $\boldsymbol \theta$. 
%Let $\ell$ denote the training loss and .
%Let $k$ denote the targeted sparsity number, determined by the pruning ratio $p = k/d$. 
Given the pruning ratio $p\%$, the sparsity constraint   is given by $\mathbf m \in  \mathcal{S} $, where $\mathcal S = \{ \mathbf m\,|\, \mathbf m \in \{ 0, 1\}^n, \mathbf  1^T \mathbf m \leq k \}$ and $k = p\% n$.
Our goal is to  prune the original   model \textit{directly} to the targeted sparse number $k$ (\textit{i.e.}, without calling for the IMP-like sparsity schedule as described in Sec.\,\ref{sec: preliminary}) and obtain the optimized sparse model $(\mathbf m \odot \btheta)$. To this end, we interpret the pruning task (\textit{i.e.}, \ding{182}) and the model retraining task (\textit{i.e.}, \ding{183}) as \textit{two optimization levels}, where the former is formulated as an \textit{upper-level} optimization problem, and it relies  on the optimizer of the \textit{lower-level}  retraining task. We then cast the model pruning problem as the following BLO problem (with \ding{183} being nested inside \ding{182}):
\todo{Mention structured pruning? For structured pruning, manipulate m with Kronecker and transfer the element-wise pruning unit to a structured one.

% \YY{In actual implementation, we use individual m for each $\theta$, but with specific structural patterns. I agree with Pari that we can mention such manipulation.}
}%

\vspace*{-6mm}
{\small{
\begin{align}
% \vspace*{-3mm}
\displaystyle
    \begin{array}{llll}
\displaystyle \minimize_{\mathbf \mask \in \mathcal{S}}         & \underbrace{\ell(\mask \odot {\btheta}^*(\mask))}_\text{ \ding{182}: Pruning task}; 
& \quad 
  \st &  \underbrace{\displaystyle {\btheta}^*(\mask) = \argmin_{\btheta \in \mathbb{R}^n} \overbrace{ \ell(\mask\odot \btheta) + \frac{\gamma}{2} \|\btheta\|_2^2}^\text{$\Def g(\mask, \btheta)$}}_\text{\ding{183}: Sparsity-fixed model retraining},
    \end{array}
    \label{eq: prob_bi_level}
\end{align}
}}%
where $\ell$ denotes the model training loss (\textit{e.g.}, cross entropy), 
$\mathbf m$ and $\btheta$ are the upper-level and lower-level optimization variables respectively, 
${\btheta}^*(\mask)$ signifies the lower-level solution by minimizing the objective function $g$ given the pruning mask $\mathbf m$, 
and $\gamma > 0$ is a regularization parameter introduced to strongly convexify the lower-level optimization so as to stabilize the gradient flow from   $\btheta^*(\mathbf m)$ to $\mathbf m$ and thus the   convergence of BLO \cite{shaham2015understanding,hong2020two}.
%As will be evident later, the introduction of $\lambda$
In a sharp contrast to existing single-level optimization-based model pruning methods \cite{wen2016learning,zhang2018systematic,hoefler2021sparsity,wang2020proximal}, the BLO formulation \eqref{eq: prob_bi_level} brings in  \underline{two advantages}. 

\underline{First}, BLO has flexibility to use   {mismatched} pruning and retraining objectives at the upper and   lower optimization levels, respectively. This flexibility exists  for customizing not only the regularized lower-level   objective function in \eqref{eq: prob_bi_level}
but also optimization algorithm per level. To be more specific, one can  update the upper-level pruning mask $\mask$ using a data batch (called $\mathcal B_2$) distinct from the one (called $\mathcal B_1$) used for  obtaining the lower-level solution ${\btheta}^*(\mask)$. The resulting BLO procedure can then mimic the idea of  meta learning to improve model generalization \cite{deng2021meta}, where the lower-level problem fine-tunes $\btheta$ using $\mathcal B_1$, and the upper-level problem validates the generalization of the sparsity-aware finetuned model $(\mathbf m \odot \boldsymbol \theta^* (\mathbf m))$ using $\mathcal B_2$.
%By doing so, the idea of meta learning (to improve model generalization)  can be infused into  model   


\underline{Second}, BLO enables us to explicitly model and optimize the coupling  between the retained model weights $\btheta^*(\mathbf m)$ and the   pruning mask $\mathbf m$ through the implicit gradient (IG)-based optimization routine. Here IG refers to  the gradient of the lower-level solution $\btheta^*(\mathbf m)$ with respect to (w.r.t.) the upper-level variable $\mathbf m$, and its derivation  calls the implicit function theory \cite{gould2016differentiating}.
The use of     IG makes our proposed BLO-oriented pruning \eqref{eq: prob_bi_level} significantly different from the greedy alternating minimization  \cite{csiszar1984information} that learns the upper-level and lower-level variables independently (\textit{i.e.}, minimizes one variable by fixing the other). We refer readers to the following  section for the detailed  IG theory.
 We will also show in Sec.\,\ref{sec: exp} that
 %assisted by the theoretically-grounded  BLO, 
 the pruning strategy acquired from \eqref{eq: prob_bi_level} can   outperform IMP in many pruning scenarios but is much more efficient in computation as it does not call for the scheduler of iterative pruning   ratios. 
 
% A sparse model (\emph{a.k.a.} a pruned model) is defined as $f(\mask \odot \btheta)$, namely the element-wise product of a dense network $f(\btheta, \cdot)$ and a binary mask $\mathbf m$. The pruning mask $\mask \in {\{0, 1\}}^d$ has the same shape as the model parameter $\btheta$ and localizes the non-zero weights with a certain sparsity ratio $p$, where $d={\|\btheta\|_0}$ demotes the dimension of the model parameter. 
% A pruning algorithm aims to find the sub-network of the given model architecture with a certain sparse level while maintaining the performance of the pruned model at a high level. 
% The pruning problem can be readily reformulated to a hierarchical optimization problem, where the model parameter $\mask$ and the mask $\btheta$ are jointly optimized. This nested structure presents a standard bi-level optimization (BLO) formulation, which is given by% 
% {
% \small
% \begin{align}
% % \vspace*{-3mm}
% \displaystyle
%     \begin{array}{ll}
% \displaystyle \minimize_{\mathbf \mask\in \mathbb \{0, 1\}^{d}}         & f(\mask, {\btheta}^*(\mask)) 
% \\
%   \st &  \displaystyle {\btheta}^*(\mask) = \argmin_{\btheta \in \mathbb{R}^d}  g(\mask, \btheta) + \frac{\gamma}{2} \|\btheta\|_2^2,
%     \end{array}
%     \label{eq: prob_bi_level}
% \end{align}
% }%

% where $f$ and $g$ denote the upper-level and the lower-level objective functions, and $\gamma > 0$ is a quadratic regularization parameter. 
% In the BLO formulation, the upper-level problem aims to find the pruning mask based on the given model parameter $\btheta$, while the lower-level problem retrains the model parameter with the fixed sparse mask. 
% The reasons for introducing the quadratic regularization term $\frac{\gamma}{2} \|\btheta\|_2^2$ are two-fold. First, it stabilizes the lower level problem via regularization. Second, it enforces the strong convexity of the lower-level problem. A different regularizer might be adopted in different use cases. 
% % For example, in implicit MAML\,\cite{rajeswaran2019meta} used $\| \mathbf y - \mathbf x\|_2^2$ as the regularizer. 
% For example, implicit MAML\,\cite{rajeswaran2019meta} used the $\ell_2$ regularizer to stablize the parameter update. 
% Such a strongly convex regularization term is also common in the BLO analysis \cite{shaham2015understanding} to stabilize the alternative optimization convergence of BLO.

% The BLO interpretation of model pruning provides multiple advantages in contrast to the conventional sparsity promoting optimization based methods ($\btheta$-only):

% \ding{172} Formulation-wise: the nested structure of \eqref{eq: prob_bi_level} allows for \emph{different} objective functions in different levels. This flexibility further enables us to use mismatched data batches for mask finding and model training, which has been verified to be very beneficial for improving the model generalization\,\cite{deng2021meta}.

% \ding{173} Optimization-wise: the BLO formulation is uniquely suited for characterizing structure of the pruning-retraining paradigm. Different from the single-level optimization problem, BLO will use a specialized optimization routine.

% \ding{174} Compared to IMP, BLO directly optimizes the mask $\mask$ to any given sparsity in one sole pruning cycle. There is no need to adopt a small pruning ratio and achieve the large sparsity in multiple pruning cycles. This characteristic resembles one-shot pruning methods and accounts for the \textit{sparsity-agnostic} computational costs of the BLO-based pruning method.

\paragraph{Optimization foundation of {\biprune}.}
The key optimization challenge of solving the {\biprune} problem \eqref{eq: prob_bi_level} lies in the computation of IG (implicit gradient). Prior to developing an effective solution, we first elaborate on the \textit{IG  challenge}, the unique characteristic of BLO. In the context of gradient descent, the gradient of the   objective function in  \eqref{eq: prob_bi_level} yields

\vspace*{-5mm}
{
\small{
\begin{align}
\displaystyle
    \underbrace{\frac{d\ell(\mask \odot \btheta^*(\mask))}{d\mask}}_\text{Gradient of objective} = \nabla_{\mask} \ell(\mask \odot {\btheta}^*(\mask)) + \underbrace{
    \frac{{d ( {\btheta}^*(\mask)^{\top} )
    }
    %^{\top}
    }{d \mask}}_{\text{{IG}}} \nabla_{\btheta}\ell (\mask \odot \btheta^*(\mask)),
    \label{eq: GD_bi_level}
\end{align}}}%
where $\nabla_{\mask}$ and $\nabla_{\btheta}$  denote the \textit{partial derivatives} of the bi-variate function $\ell(\mask, \boldsymbol \theta)$  w.r.t. the variable $\mask$ and $\btheta$ respectively, 
$d \btheta^\top / d \mask  \in \mathbb R^{n \times n} $ denotes the vector-wise \textit{full derivative},  
and for ease of notation, we will omit
the transpose $\top$ when the context is clear.
In \eqref{eq: GD_bi_level}, the IG challenge refers to the demand for   computing gradients of  the implicit function $\btheta^*(\mask) = \argmin_{\btheta} g(\mask, \btheta)$ w.r.t. $\mask$, where recall from \eqref{eq: prob_bi_level}  that $ g(\mask, \btheta) \Def  \ell(\mask\odot \btheta) + \frac{\gamma}{2} \|\btheta\|_2^2 $.
\iffalse
To circumvent this difficulty, the conventional method is  \textit{gradient unrolling} that   approximates the lower-level solution $\btheta^*(\mask)$ using a single or a few unrolled gradient descent steps, \textit{e.g.}, 
$\btheta^*(\mask) \approx \btheta - \alpha \nabla_{\btheta} g(\mask, \btheta)$. However, this only gives a rough estimate of the lower-level solution and  lacks   theoretical rigorousness \cite{hong2020two}. Meanwhile, even in this over-simplified scenario, it is not difficult to see that the computation of   IG
%, \textit{i.e.}, $ \frac{{d {\btheta}^*(\mask)}^{\top}}{d \mask}$,  
relies on the computation of   second-order partial derivatives.
\fi 

%Different from gradient unrolling,
Next,
we derive the IG formula following the more rigorous implicit function theory \cite{gould2016differentiating,hong2020two,rajeswaran2019meta}.
%, where the stationary condition of the lower-level optimization in \eqref{eq: GD_bi_level} is treated as  a differentiable explicit   function
Based on the fact that the   $\btheta^*(\mask)$ is satisfied with the stationary condition of the lower-level objective function in \eqref{eq: GD_bi_level},  it is not difficult to obtain that 

\vspace*{-5mm}
{\small
\begin{align}
% & \displaystyle
%     %{\frac{d\btheta^*(\mask)}{d\mask}}^{\top} (\nabla_{\btheta \btheta} g(\mask, \btheta) + \gamma \mathbf{I}) + \nabla_{\mask\btheta} g(\mask, \btheta)%
%     \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) + \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%     \nabla^2_{\btheta} \ell(\mask \odot \btheta^*)
%   + \gamma \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%   = \mathbf 0; \nonumber \\
%  \Longrightarrow  &
\displaystyle  \frac{d\btheta^*(\mask)}{d\mask} %^{\top} 
 =  -   \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) [ \nabla^2_{\btheta } \ell(\mask \odot \btheta^*) + \gamma \mathbf I ]^{-1},
 \label{eq: exact_IG}
\end{align}
}%
where   $\nabla_{\mask \btheta}^2 \ell $ and $\nabla_{\btheta \btheta}^2 \ell $ denote the second-order partial derivatives of $\ell$ respectively, and $(\cdot)^{-1}$ denotes the matrix inversion operation. We refer readers to Appendix\,\ref{eq: app_IG} for the full derivation of \eqref{eq: exact_IG}.


% we   obtain 

% \vspace*{-6mm}
% {
% \small
% \begin{align}
% \displaystyle
%   %  \frac{d g(\mask, \btheta^*(m)))}{
%   %  d\btheta}
%   \nabla_{\btheta} g(\mathbf m, \btheta^* )
%     = \nabla_{\btheta} \ell(\mask \odot \btheta^* ) + \gamma \btheta^*  = \mathbf 0.
%     \label{eq: stationary}
% \end{align}
% }%
% where for ease of notation, we omit the dependence of $\btheta^*(\mask)$ w.r.t. $\mathbf m$.
% We   then take    derivative of the second equality of \eqref{eq: stationary} w.r.t. $\mask$ by using the implicit 
% function theory. This leads to \todo{\YH{Put Eq. 3-4 in the appendix or merge them into one proof? }}
% % $
% % {\frac{d\btheta^*(\mask)}{d\mask}}^{\top} (\nabla_{\btheta \btheta} g(\mask, \btheta) + \gamma \mathbf{I}) + \nabla_{\mask\btheta} g(\mask, \btheta) = \mathbf  0
% % $

% \vspace*{-5mm}
% {\small
% \begin{align}
% & \displaystyle
%     %{\frac{d\btheta^*(\mask)}{d\mask}}^{\top} (\nabla_{\btheta \btheta} g(\mask, \btheta) + \gamma \mathbf{I}) + \nabla_{\mask\btheta} g(\mask, \btheta)%
%     \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) + \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%     \nabla^2_{\btheta} \ell(\mask \odot \btheta^*)
%   + \gamma \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%   = \mathbf 0; \nonumber \\
%  \Longrightarrow  &
%  \frac{d\btheta^*(\mask)}{d\mask} %^{\top} 
%  =  -   \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) [ \nabla^2_{\btheta } \ell(\mask \odot \btheta^*) + \gamma \mathbf I ]^{-1}.
%  \label{eq: exact_IG}
% \end{align}
% }%
% where $\nabla_{\mask \btheta} \ell $ and $\nabla_{\btheta \btheta} \ell $ are the second-order partial derivatives of the bivariate function $\ell$, and $(\cdot)^{-1}$ denotes the matrix inversion operation.

Yet, the exact   IG formula \eqref{eq: exact_IG} remains difficult in calculation due to the presence of    matrix   inversion and   second-order partial derivatives.
\todo{$\gamma$ is critical in this derivation. Without $\gamma$, and with the $\nabla^2_{\btheta} = 0$ assumption, this does not go through. How do we best motivate the introduction of $\gamma$ in (1) since standard pruning setups and schemes dont introduce such regularization term?}
To  simplify it, 
we impose the Hessian-free assumption, 
$ \nabla^2_{\btheta} \ell = \mathbf 0$, which  is mild in general; For example,   the decision boundaries of neural networks with ReLU activations are piece-wise linear in  a tropical hyper-surface \cite{alfarra2020decision}, and this assumption 
%is   necessary as  computing the Hessian matrix w.r.t.   model parameters $\btheta$ would be practically infeasible, and it
has been widely used in meta learning \cite{finn2017model}. Given $ \nabla^2_{\btheta } \ell = \mathbf 0$,  the matrix inversion in \eqref{eq: exact_IG} can   be then mitigated, leading to the IG formula

\vspace*{-5mm}
{\small
\begin{align}
    \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
    =  -  \frac{1}{\gamma} \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ).
    \label{eq: IG_simplify}
\end{align}
}%

At the first glance, the computation of the simplified IG   \eqref{eq: IG_simplify} still requires the mixed (second-order) partial derivative $\nabla^2_{\mask \btheta} \ell$. However, {\biprune} is a special class of BLO problems with bi-linear variables 
$(\mask \odot \btheta)$. Based on this bi-linearity, we can prove that  IG  in \eqref{eq: IG_simplify} can be \textit{analytically} expressed using only \textit{first-order} derivatives; see the following theorem. 

% \begin{tcolorbox}[colback=black!5!white,colframe=white!20!black]
\begin{myprop}
\label{thr: ig}
Assuming $\nabla^2_{ \btheta} \ell = 0$, the implicit gradient \eqref{eq: IG_simplify} is then given by

\vspace*{-5mm}
{\small
\begin{align}
\displaystyle
\frac{d\btheta^*(\mask)}{d\mask} %^{\top} 
% =  -  \frac{1}{\gamma} \nabla_{{\mask} {\btheta}} \ell ({\mask} \odot {\btheta}^*) 
= -  \frac{1}{\gamma} \mathrm{diag}( \nabla_{\mathbf z} \ell(\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right.);
% := -\frac{1}{\gamma} \mathrm{diag}(\mathbf{A}).
\label{eq: IG_final}
\end{align}
}%
% The rationale behind Hessian-free assumption is that commonly used ReLU-based neural network tends to form a piece-wise linear decision boundary \emph{w.r.t.} the model parameter $\btheta$. This has been theoretically proved by \,\cite{alfarra2020decision}. Empirical results \cite{finn2017model} also suggest that the absence of the second-order derivative hardly harms the performance of the BLO algorithm. 
Further, the   gradient of the  objective function given by \eqref{eq: GD_bi_level} becomes

{\vspace*{-3mm}
{
\small
\begin{align}
\displaystyle
    \frac{d \ell(\mask \odot \btheta^*)}{d \mask} = ( \btheta^* 
    - 
    \frac{1}{\gamma} \mask \odot \gradzsimple) \odot \gradzsimple,
    \label{eq: upper_update_final}
\end{align}}}%
where for ease of notation    {$\gradzsimple$} signifies {$\gradz$}, and recall that $\odot$ denotes the element-wise multiplication.
\end{myprop}
%\end{tcolorbox}
\textbf{Proof}: Using chain-rule, we can obtain that

\vspace*{-4mm}
{\small
\begin{align}
&    \nabla_{\btheta}\ell(\mask \odot \btheta^*) = %\nabla_{\btheta^*} (\mask \odot \btheta^*)^\top
\mathrm{diag}(\mathbf m)
\gradzsimple = \mask \odot \gradzsimple;
    \label{eq: chainrule_theta} \\
\text{similarly,   } & \nabla_\mask \ell(\mask \odot \btheta^*) 
    % = \nabla_\mask (\mask \odot \btheta^*)^\top \gradzsimple 
    % = \mathrm{diag}(\btheta^*) \gradzsimple 
    = \mathrm{diag}(\btheta^*) \gradzsimple 
    = \btheta^* \odot \gradzsimple \label{eq: chainrule_mask}
\end{align}
}%%
where $\mathrm{diag}(\cdot)$ represents a diagonal matrix with $\cdot$ being the main diagonal vector.
% Similarly, we also have $\nabla_{\btheta^*}\ell(\mask \odot \btheta^*) = \mask \odot \gradzsimple$. 
% For simplicity, we denote $\gradz$ as $\gradzsimple$. 
Further, we can convert \eqref{eq: IG_simplify} to

\vspace*{-4mm}
{
\small
\begin{align}
\displaystyle
    \nabla^2_{{\mask} {\btheta}} \ell({\mask}  \odot {\btheta^*}) 
    % & = \nabla_{{\mask}} \left [ \mathrm{diag}({\mask}) {\gradzsimple} \right ] \\
    & \overset{\eqref{eq: chainrule_theta}}{=} \nabla_{{\mask}} \left [ {\mask} \odot  \nabla_{\mathbf z} \ell(\mathbf z) \right ]
    \nonumber \overset{\text{chain rule}}{=} 
    \mathrm{diag}( {\gradzsimple}) 
    + 
    \mathrm{diag}({\mask}) [ \nabla_{{\mask}} ( \nabla_{\mathbf z} \ell(\mathbf z) ) ]
    % \mask \odot 
    % [\btheta^* \odot \nabla_{\mathbf z \mathbf z} \ell (\mathbf z) 
    % \left |_{\mathbf z = {\mask} \odot {\btheta^*}} \right. 
     \nonumber \\
    & \overset{\eqref{eq: chainrule_mask}}{=}  \mathrm{diag}( {\gradzsimple}) 
    + 
    \mathrm{diag}({\mask}) [ \mathrm{diag}(\btheta^*) \nabla^2_{\mathbf z } \ell(\mathbf z) ] = \mathrm{diag}(\gradzsimple) ,\label{eq: ezBiP}
 \end{align}}%
where the last equality holds due to the Hessian-free assumption. With \eqref{eq: ezBiP} and \eqref{eq: IG_simplify} we can prove \eqref{eq: IG_final}.
% of $\nabla_{\btheta \btheta} \ell = \mathbf 0$.

Next, substituting the IG \eqref{eq: IG_final}  to the upper-level gradient \eqref{eq: GD_bi_level}, we  obtain that

\vspace*{-3mm}
{
\small
\begin{align}
\displaystyle
     \frac{d \ell(\mask \odot \btheta^*)}{d \mask} 
    & \,\,\,\,=\nabla_{\mask}\ell({\mask} \odot {\btheta}^*) - 
    {\frac{1}{\gamma}
    \gradzsimple
    % \mathbf{A}
    \odot \nabla_{{\btheta}} \ell({\mask} \odot {\btheta^*})
    } \nonumber \\
    &
    \underset{ }{\overset{\eqref{eq: chainrule_theta}, \eqref{eq: chainrule_mask}}{=}}  \btheta^* \odot \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right.
    - \frac{1}{\gamma} \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right. 
    \odot
    ( \mask \odot \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right. 
    ) 
    %\nonumber \\
   % & \,\,\,\,
    =  (\btheta^* - \frac{1}{\gamma} \mask \odot \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right.
    ) \odot \gradzsimple, \nonumber
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right. 
   % \label{eq: upper_final_proof}
\end{align}
}%
which leads to \eqref{eq: upper_update_final}. 
The proof is now complete. \hfill $\square$ 
\todo{Do we have any empirical evidence that shows that using \eqref{eq: upper_update_final} is better than using \eqref{eq: chainrule_mask}? That would be good to highlight advantage of BLO and IG. 

\YY{Pari means the significance of the extra term brought by IG.} }

The key insight drawn from Prop.\,\ref{thr: ig} is that the bi-linearity of pruning variables (\textit{i.e.}, $\mask \odot \boldsymbol \theta^*$) makes the  IG-involved gradient \eqref{eq: GD_bi_level} easily computed, and the   computational complexity is almost same as that of computing the first-order gradient $\nabla_{\mathbf z} \ell (\mathbf z)$ just once, as supported by   \eqref{eq: upper_update_final}.
%\todo{Pari: computational complexity corollary}
 
\begin{mycor}
Given $\mask \in \{0, 1\}^n, \btheta \in \mathbb R^n$ and that the computation of the gradient $\nabla_{\mathbf z} \ell (\mathbf z) \in \mathbb R^n$ takes $O(n)$ time, the computation of the loss gradient~\eqref{eq: GD_bi_level} with respect to the mask $\mask$ of the objective~\eqref{eq: prob_bi_level} using \eqref{eq: upper_update_final} in Proposition~\ref{thr: ig} takes $O(n)$ time.
\end{mycor}
% Thus, we can prove \eqref{eq: upper_update_final}. As \eqref{eq: upper_update_final} suggests, the upper-level gradient update only involves one backward-propagation and thus, the bi-level pruning can be solved as easily as a first-order alternating optimization problem.

%\SL{[I stop here.]}
\paragraph{{\biprune} algorithm and implementation.}
%Assisted by Prop.\,\ref{thr: ig}, 
We will next 
formalize the {\biprune} algorithm 
%solve the {\biprune} problem \eqref{eq: prob_bi_level} 
based on Prop.\,\ref{thr: ig} and the alternating gradient descent method \cite{hong2020two}. At iteration $t$, there exist two main steps.

\todo{\YY{Hi Pari, feel free to elaborate on the algorithm with the way that you think is the best}}

\ding{72} \textit{Lower-level SGD for model retraining}: 
Given $\mask^{(t-1)}$, $\btheta^{(t-1)}$, and 
$\mathbf z^{(t-1)} \Def \mask^{(t-1)} \odot \btheta^{(t-1)}$, we update $\btheta^{(t)}$ by applying SGD (stochastic gradient descent) to the lower-level problem of \eqref{eq: prob_bi_level},%


\vspace*{-5mm}
{\small 
\begin{align}
    \btheta^{(t)} & = \btheta^{(t-1)} - \alpha \nabla_{\btheta} g(\mask^{(t-1)}, \btheta^{(t-1)})  \nonumber \\
   &  \hspace*{-5mm}
   \overset{%\eqref{eq: stationary}, 
   \eqref{eq: chainrule_theta}}{=}
    \btheta^{(t-1)} - \alpha [ \mask^{(t-1)} \odot 
    \nabla_{\mathbf z} \ell(\mathbf z )\left | \right._{\mathbf z = \mathbf z^{t-1}} + \gamma \btheta^{(t-1)} ],
    %\nabla_{\btheta} g(\mask^{(t-1)}, \btheta^{(t-1)}) 
    \tag{$\btheta$-step}
    \label{eq: theta_step}
\end{align}}%
where $\alpha > 0$ is the lower-level   learning rate.

\ding{72} \textit{Upper-level PGD for pruning}: Given $\mask^{(t-1)}$, $ \btheta^{(t)}$, and $\mathbf z^{(t+1/2)} \Def \mask^{(t-1)} \odot \btheta^{(t)}$, we update   $\mask$ using   PGD (projected gradient descent) along the IG-enhanced descent direction \eqref{eq: GD_bi_level},%

\vspace*{-5mm}
{\small
\begin{align}
    \mask^{(t)} = & \mathcal P_{\mathcal S} \left [ 
    \mask^{(t-1)}  - \beta  \frac{d \ell(\mask \odot \btheta^{(t)})}{d \mask} \left | \right._{\mask =     \mask^{(t-1)} }
    \right ] \nonumber \\
\overset{\eqref{eq: upper_update_final}}{=}    
    &\mathcal P_{\mathcal S} \left [ 
    \mask^{(t-1)}  - \beta  \left ( \btheta^{(t)} - 
    \frac{1}{\gamma} \mask^{(t-1)} \odot \gradzsimple \left | \right._{\mathbf z = \mathbf z^{(t+1/2)}} \right ) \odot \gradzsimple  \left | \right._{\mathbf z = \mathbf z^{(t+1/2)}}
    \right ],
    \tag{$\mask$-step}
    \label{eq: m_step}
\end{align}}%
where $\beta > 0$ is the upper-level learning rate, and $\mathcal P_{\mathcal S}(\cdot)$ denotes the Euclidean projection   onto the constraint set $\mathcal S$ given by
$\mathcal S = \{ \mathbf m\,|\, \mathbf m \in \{ 0, 1\}^n, \mathbf  1^T \mathbf m \leq k \}$ in \eqref{eq: prob_bi_level} and is achieved by the top-$k$ hard-thresholding operation as will be detailed later.  

In {\biprune}, the \eqref{eq: theta_step} and \eqref{eq: m_step} steps execute iteratively till convergence. In practice, we find that {\biprune} converges very well; see Fig.\,\ref{fig: convergence} for an ablation study.
It is also worth noting that both \eqref{eq: theta_step} and \eqref{eq: m_step} steps only require the first-order information $\nabla_{\mathbf z} \ell (\mathbf z)$, demonstrating that the {\biprune} algorithm can be conducted as efficiently as first-order optimization. 
We present more implementation details of {\biprune}   below.


\ding{70} \textit{Discrete optimization over $\mask$:} We follow the  {`convex relaxation + hard thresholding'} mechanism used in \cite{sehwag2020hydra,ramanujan2020sHiddenSubnetwork}.
Specifically, we relax the binary masking variables   to continuous masking   scores $\mathbf m \in [\mathbf 0, \mathbf 1]$. We then acquire  loss gradients at  the backward pass based on the relaxed  $\mathbf m$. At the forward pass, we project it  onto the discrete constraint set $\mathcal S$ using the hard thresholding operator, where   its top $k$ elements  are set by  $1$s and the others by $0$s. 
%At  to tn he backward pass for grationadient calculation, we 

\ding{70} \textit{Data batch selection for lower-level and upper-level optimization:} We adopt different data batches (with the same batch size) when implementing \eqref{eq: theta_step} and \eqref{eq: m_step}. This is one BLO's advantage of, which owns the flexibility to customize the lower-level and upper-level optimization problems. And the use of diverse data batches  is beneficial to model generalization as shown in \cite{deng2021meta}. 
 
\ding{70} \textit{Hyperparameter tuning:} As described in \eqref{eq: theta_step}-\eqref{eq: m_step},  {\biprune} needs to set two learning rates $\alpha$ and $\beta$ for lower-level and upper-level optimization, respectively. We choose $\alpha = 0.01$ and $\beta = 0.1$ in all experiments, where we adopt the mask learning rate $\beta$ from Hydra\,\cite{sehwag2020hydra} and set a smaller lower-level learning rate $\alpha$, as $\btheta$ is initialized by a pre-trained dense model. We show ablation study on $\alpha$ in Fig.\,\ref{fig: ablation_study}(c).
% The more aggressive lower-level optimization is typically suggested by the convergence of BLO \cite{hong2020two}. 
BLO also brings in the low-level convexification parameter $\gamma $. We set $\gamma = 1.0 $ in   experiments and refer readers to {Fig.\,\ref{fig: ablation_study}(b)} for a sanity check. 

\ding{70} \textit{One-shot vs. multi-step SGD:}
In  \eqref{eq: theta_step}, the   one-step SGD is used and helps reduce the computation overhead. In practice, we also find that the one-step SGD is sufficient:  The use of multi-step SGD in {\biprune} does not yield much significant improvement over the one-step version; see {Fig.\,\ref{fig: ablation_study}(a)}.
%computation-friendly. 

\ding{70} \textit{Extension to structured pruning:}
We formulate and solve the {\biprune} problem in the context of unstructured (element-wise)  weight pruning. However, if define the pruning mask $\mask$ corresponding to model's structure units  (\textit{e.g.}, filters), then it is easy to apply {\biprune} to structured weight pruning; see Fig.\,\ref{fig: structured_performance_cifar} and Fig.\,\ref{fig: structured_performance_cifar_appendix} for empirical results.

\iffalse
Next we give some implementation remarks on our algorithm. We adopt the commonly used Cross-Entropy loss as our upper- and lower-level loss functions. To circumvent the difficulty from discrete optimization for binary mask $\mask$, we adopt the widely accepted 
\textbf{soft score + hard threshold} paradigm to deal with $\mask$. We first loosen the binary constraint of $\mask$ from $\{0, 1\}^n$ to $\mathbb R^{n}$ as the `mask score'. After each step, for any given sparsity ratio $p\%$, we update the true binary mask by setting the top $1-p\%$ elements with the highest score to $1$ and the rest to $0$. We emphasize the {\biprune} can be applied to the structured pruning setting simply by changing the threshold operation by wipe out the parameter patterns (\emph{e.g.}, the convolutional kernel) with the lowest score $\ell_2$ norms. In practice, we use different batches $\mathcal{B}_\alpha$ and $\mathcal{B}_\beta$ for upper- and lower-level updates for better generalization ability. {In practice, we will show that the performance of {\biprune} is not sensitive to the lower level step number $K$ in Sec\,\ref{sec: exp}. Thus, unless otherwise specified, we report the results with $K=1$.}
\todo{Can we discuss $\mask_t$ update more formally like $\mask_{t+1} \gets P_\mathcal{S} (\mask_t - \beta (7))$?}
\fi 
% For initialization, the model parameter $\btheta_0$ are initialized with \textit{Kaiming Normal}\,\cite{he2015delving} and 

\iffalse
The mask scores $\mask_0$ are scaled proportionate to the model weights\,\cite{sehwag2020hydra} and the initial binary mask $\mask$ is initialized \emph{w.r.t.} the score initialization $\mask_0$. We use separate learning rates for upper and lower-level problem namely $0.1$ for sparse mask and $0.01$ for model parameter. We further set the lower-level problem regularization coefficient to $0.1$.  We will show in Sec.\,\ref{sec: exp} these hyper-parameter choices are consistently used in all settings and are easy to tune.
\fi 
% In our algorithm, we choose the upper- and lower-level objective as the commonly used model training loss function $\ltr$, such as Cross-Entropy loss. 
% Our algorithm is shown in Algorithm\,\ref{alg: BiP}. 
% In our implementation, we adopt the \textbf{soft score + hard threshold} paradigm to train the discrete variable $\mask$. We first loosen the binary constraint of $\mask$ from $\{0, 1\}^d$ to $\mathbb R^{d}$ as the `mask score'. After each step, for any given sparsity ratio $p\%$, we update the true binary mask $\mathbf{z}^*$ by setting the top $1-p\%$ elements with the highest score to $1$ and the rest to $0$ (denoted as threshold operation $\mathcal{T}_{\{0,1\}^d}$ in \eqref{eq: threshold}). We emphasize the {\biprune} can be applied to the structured pruning setting simply by changing the threshold operation by wipe out the parameter patterns (\emph{e.g.}, the convolutional kernel) with the lowest score $\ell_2$ norms.

% We use separate learning rates for upper and lower-level problem namely $0.1$ for sparse mask and $0.01$ for model parameter. We further set the lower-level problem regularization coefficient to $0.1$.  We will show in Sec.\,\ref{sec: exp} these hyper-parameter choices are consistently used in all settings and are easy to tune.
% For initialization, 
% the model parameter $\btheta_0$ are initialized with \textit{Kaiming Normal}\,\cite{he2015delving} and the mask scores $\mask_0$ are scaled proportionate to the model weights\,\cite{sehwag2020hydra}. 
% The initial binary mask $\mathbf{z}^*$ is initialized \emph{w.r.t.} $\mask_0$. 

% \newpage 


==> Deprecated_NO_USE/Version_Camera_05161900/exp_SL.tex <==
In this section, we present extensive experiment results to show the effectiveness of {\biprune}  
%in both accuracy and   efficiency
across multiple model architectures,  various datasets, and different pruning setups. Compared to IMP, one-shot pruning, and optimization-based pruning baselines, 
we find that {\biprune} leads to better winning tickets in most cases and is computationally as efficient as one-shot pruning. 

\subsection{Experiment Setup}
\paragraph{Datasets and models.}
Following the pruning benchmark in \cite{ma2021sanity}, 
we consider 4 datasets including CIFAR-10\,\cite{krizhevsky2009learning}, CIFAR-100\,\cite{krizhevsky2009learning}, Tiny-ImageNet\,\cite{le2015tiny}, ImageNet\,\cite{deng2009imagenet}, and 5
architecture types  including  ResNet-20/56/18/50
% \SL{[do we really need RN here?]}
and VGG-16 \cite{he2016deep,simonyan2014very}. 
%ResNet\,\cite{he2016deep}, VGG\,\cite{simonyan2014very}\} for evaluation. 
Tab.\,\ref{table: impl_details} summarizes these dataset and model information and setups.  

% For more details on the dataset-model architecture combination, please refer to Table\,\ref{table: impl_details}.
% We summarize our detailed training setups and hyper-parameter selections in Table\,\ref{table: impl_details}. For both unstructured and structured pruning, we adopt two architecture series ResNet\,\cite{he2016deep} and VGG\,\cite{simonyan2014very} for four representative datasets, namely \emph{i.e.,} CIFAR-10\,\cite{krizhevsky2009learning}, CIFAR-100\,\cite{krizhevsky2009learning}, Tiny-ImageNet\,\cite{le2015tiny}, and ImageNet\,\cite{deng2009imagenet}. 



\paragraph{Baselines,  training, and evaluation.}
When comparing with {\biprune}, we mainly focus on 4 state-of-the-art (SOTA) pruning methods, \ding{172} IMP \cite{frankle2018lottery}, \ding{173} OMP \cite{frankle2018lottery},
% \SL{[refs; be consistent with earlier sections]}
 \ding{174} {\grasp} \cite{wang2019picking} (a one-shot pruning method by analyzing gradient flow at initialization), and \ding{175} {\hydra} \cite{sehwag2020hydra} (an optimization-based pruning method that optimizes masking scores). It is worth noting that there exist various implementations of IMP, \textit{e.g.}, specified by different learning rate and model initialization `rewinding' strategies \cite{Renda2020Comparing}. To make a fair comparison, we follow the recent IMP benchmark in \cite{ma2021sanity}, which can find the best winning tickets over current heuristics-based pruning baselines.
We also remark that {\hydra} is originally proposed for improving adversarial robustness of a pruned model, but it can be easily customized for standard pruning when setting the adversary's strength as $0$ \cite{sehwag2020hydra}. We choose {\hydra} as a baseline because it can be regarded as a specification of {\biprune}, given by a single-level sparse mask optimization task together with post-optimization weight re-training. 
When implementing {\biprune}, unless specified otherwise, we use the $1$-step SGD in \eqref{eq: theta_step}, and set the learning rates $(\alpha, \beta)$ and the lower-level regularization parameter $\gamma$ as described in the previous section. When implementing baselines, we follow their official code repository setups.
We evaluate the performance of {\biprune} and the above baselines mainly from two perspectives:14
(1) the test accuracy of the obtained sub-network, and (2) the runtime of pruning to reach the desired sparsity. 
We refer readers to Tab.\,\ref{tab: training_details}, Appendix\,\ref{app: training} for more training and evaluation details, such as training epochs, learning rate schedulers, and so forth. 

% In unstructured pruning settings, we compare {\biprune} with various heuristics-based and optimization-based baselines, including IMP\,\cite{frankle2019stabilizing}, OMP, \grasp\,\cite{wang2019picking}, and \hydra\,\cite{sehwag2020hydra}. To make a fair comparison, we adopt the recommended training settings from their papers and we adopt the SOTA implementation following\,\cite{ma2021sanity} for IMP and OMP. {\hydra} is an optimization-based baseline framework, which is originally designed for robust pruning, but can be customized to standard pruning as mentioned in its paper\,\cite{sehwag2020hydra}. 
%For complete and detailed training details please refer to Appendix\,\ref{app: training}.

% \begin{wrapfigure}{r}{85mm}
% \vspace*{-5mm}
% \centerline{
% \begin{tabular}{cc}
% \hspace*{0mm}\includegraphics[width=.3\textwidth,height=!]{figure/Global_Pruning_on_TinyImageNet_ResNet18.pdf}  
% &\hspace*{-6mm}\includegraphics[width=.3\textwidth,height=!]{figure/Global_Pruning_on_ImageNet_ResNet18.pdf}
% \\
% \hspace*{2mm}\footnotesize{(a) Tiny-ImageNet with ResNet-18} &   \footnotesize{(b) ImageNet with ResNet-50}
% \end{tabular}}
% % \vspace*{-2mm}
% \caption{\footnotesize{
% Unstructured pruning test accuracy (\%) v.s. sparsity (\%) on Tiny-ImageNet and ImageNet. Other settings remain the same as Fig.\,\ref{fig: unstructured_performance_cifar}.
% % Models are pruned up to $90\%$ following\,\cite{ma2021sanity}. 
% \YH{ImageNet is still incomplete.}}}
%   \label{fig: unstructured_performance_imagenet}
% %   \vspace*{-4mm}
% \end{wrapfigure}


% We consider two different structured pruning settings with different pruning granularity of a convolutional layer,  termed filter-wise and channel-wise pruning. In general, the parameters of a convolutional layer have a shape of [$c_{\text{out}}$, $c_{\text{in}}$, w, h], which denote the output channel number, input channel number, kernel width and kernel height respectively.
% The filter-wise pruning\,\cite{chen2022coarsening} remove the model 
% parameters following a basic pattern of [$c_{\text{in}}$, w, h] while the channel-wise following [$c_{\text{out}}$, w, h]. The sparsity ratio of each layer is kept the same as the target sparsity $p\%$. Please refer to Fig.\,\ref{fig: illustration} for illustration on the two settings.
% We choose the OMP and IMP as our baselines in both structured pruning settings. Due to the page limit, we only report the results of filter-wise pruning in the main paper and include the channel-wise in Appendix\,\ref{app: add_results}, while the both settings lead to consistent conclusions.


% \paragraph{Evaluation Setups.}
% We mainly evaluate the performance of {\biprune} and the other baselines from two perspectives. 
% %As our method is dedicated to achieve high pruning accuracy (like IMP) with less computational burden (like OMP), we
% particularly pay attention to the following two metrics:
% % to the quality of the sparse networks and the pruning efficiency.
% % evaluate the quality of the found sparse network (see \ding{182}-\ding{183}) and the pruning efficiency (see \ding{184}) when evaluating a method. In particular, we pay attention to the following metrics: 
% (1) the test accuracy of the obtained sub-network, and (2) the runtime of pruning to reach the desired sparsity. 

%  (How good?) the quality of the sub-networks: besides the test accuracy of the target sparsity, we also study the best winning tickets and the sparsest winning tickets that can be found by each method across different sparsities. The former reveals the maximum potential of a pruning method to improve the test accuracy over the dense model. The latter depicts how sparse the method can go without losing any accuracy.
% % : the improvement on the test accuracy of the best winning ticket compared to dense model. \ding{183} (How sparse?) the sparsest winning ticket: winning ticket with the largest sparsity found by each method 
% \ding{183} (How fast?) pruning efficiency: this includes the required time to reach the given sparsity as well as to find the best/sparsest winning tickets.
% % reach the given sparsity as well as 
% % this includes the time spent for finding the sparsest winning ticket and for the whole pruning process. For structured pruning in particular, we also compare the inference efficiency (FLOPs) of the found sparse networks.




\subsection{Experiment Results}

\paragraph{{\biprune}   identifies high-accuracy winning tickets.} 
In what follows, we peer into the quality of winning tickets identified by {\biprune}.
%\textit{pruning trajectory} (given by test accuracy vs. pruning ratio) of {\biprune} and baseline methods.
\textit{Two  key observations} can be drawn from our experiment results: (1)  {\biprune}   finds winning tickets of higher accuracy and/or higher  sparsity than  the baselines in most cases (as shown in Fig.\,\ref{fig: unstructured_performance_cifar} and Tab.\,\ref{tab: sparsest_wt}; (2)  The superiority of {\biprune} holds for both unstructured pruning and structured pruning (as shown in Fig.\,\ref{fig: structured_performance_cifar} and Fig.\,\ref{fig: structured_performance_cifar_appendix}
% \SL{, and xxx}
). 


\begin{figure}
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_ResNet20.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_ResNet56s.pdf} &
    \hspace*{-5mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_VGG16.pdf} \\
    
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-100_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-100_ResNet20s.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_TinyImageNet_ResNet18.pdf} &
    \hspace*{-5mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_ImageNet_ResNet50.pdf}
\end{tabular}}
\caption{\footnotesize{Unstructured pruning trajectory given by test accuracy (\%) vs. sparsity (\%) on various dataset-model pairs.
%with ResNet-18/20/56 and VGG-16.
The proposed \textcolor{Green}{\biprune} is compared with \textcolor{blue}{\hydra}\,\cite{sehwag2020hydra}, \textcolor{orange}{IMP}\,\cite{ma2021sanity}, \textcolor{ompcolor}{OMP}\,\cite{ma2021sanity}, \textcolor{Purple}{\grasp}\,\cite{wang2019picking}. And the performance of   dense model and that of the best winning ticket  are marked using   dashed lines in each plot. 
%the mean (solid line) and variance (shaded area) of accuracies over \SL{xxx} random trials are reported for each pruning method 
    The solid line and shaded area of each pruning method represent  the mean and variance of test accuracies over 3 independent trials. We observe that
    {\biprune}  consistently outperforms the other baselines.
}}
\label{fig: unstructured_performance_cifar}
\end{figure}



% \begin{table}[htb]
% \centering
% \caption{\footnotesize{The sparsest winning tickets found by different methods at different data-model setups. In each cell, $p\%$ ($t$ min) represents the sparsity as well as the time consumption to find the sparsest winning ticket. {\xmark} signifies that no winning ticket  is found  by a   pruning method. Given the data-model setup (\textit{i.e.}, per column),
% the sparsest winning ticket is highlighted in \textbf{bold}.
% \SL{[remove computation time from this table?]
% \SL{[wrap table?]}
% \SL{$aa, +bb$}
% }
% }}
% \label{tab: sparsest_wt}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{c|cccccc}
% \toprule[1pt]
% \midrule
% \multirow{2}{*}{Method} & \multicolumn{4}{c}{CIFAR-10}                               & \multicolumn{2}{c}{CIFAR-100} \\
%                         & ResNet-18    & ResNet-20    & ResNet-56    & VGG-16        & ResNet-18    & ResNet-20      \\ \midrule
% IMP        &  87\% (620 min) &\textbf{74}\% (200 min) & \textbf{74}\% (462 min) & 89\% (501 min) &  87\% (620 min) & \xmark       \\ % Grasp ResNet56 104 min
% OMP                     & 49\% (69 min) & \xmark & \xmark & 20\% (50 min) & 74\% (69 min)       & \xmark         \\
% \grasp                  & \xmark & \xmark & 36\% (104 min) & \xmark & \xmark       & \xmark         \\
% {\hydra}                & \xmark       & \xmark       & 20\% (188 min) & 87\% (108 min)  & \xmark       & 20\% (86 min)   \\
% {\biprune} & \textbf{89}\% (86 min)  & 67\% (65 min)  & \textbf{74}\% (179 min)  & \textbf{93}\% (118 min) &  \textbf{89}\% (86 min) & \textbf{49}\% (65 min) \\ \midrule
% \bottomrule[1pt]
% \end{tabular}%
% }
% \end{table}

% \begin{table}[htb]
% \centering
% \caption{\footnotesize{The sparsest winning tickets found by different methods at different data-model setups. \YY{Winning tickets refer to the sparse models with close performance to the dense ones.} In each cell, $p\%$ ($acc \pm std \%$) represents the sparsity as well as the test accuracy. The test accuracy of dense models can be found in the header. {\xmark} signifies that no winning ticket  is found  by a   pruning method. Given the data-model setup (\textit{i.e.}, per column),
% the sparsest winning ticket is highlighted in \textbf{bold}.
% % \SL{[remove computation time from this table?]
% % \SL{[wrap table?]}
% % \SL{$aa, +bb$}
% % \YY{Dense +-}
% % }
% \YY{test accuracy and std}
% }}
% \label{tab: sparsest_wt}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{c|cccccc}
% \toprule[1pt]
% \midrule
% \multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10}                               & \multicolumn{2}{c}{CIFAR-100} \\
%                         & ResNet-18    & ResNet-20    & ResNet-56    & VGG-16        & ResNet-18    & ResNet-20      \\ 
%                         & (94.77\%)      & (92.12\%)        & (92.95\%)       & (93.65\%)   & (76.67\%)   &   (68.69\%)      \\\midrule
% IMP        &  87\% (0.01\%$\uparrow$) &\textbf{74}\% (0.03\%$\uparrow$) & \textbf{74}\% (0.04\%$\uparrow$) & 89\% (0.03\%$\uparrow$) &  87\% (0.24\%$\uparrow$) & \xmark       \\ % Grasp ResNet56 104 min
% OMP                     & 49\% (0.03\%$\uparrow$) & \xmark & \xmark & 20\% (0.14\%$\uparrow$)  & 74\% (0.32\%$\uparrow$)    & \xmark         \\
% \grasp                  & \xmark & \xmark & 36\% (0.12\%$\uparrow$)& \xmark & \xmark       & \xmark         \\
% {\hydra}                & \xmark       & \xmark       & \xmark  & 87\% (0.08\%$\uparrow$)  & \xmark       & 20\% (0.25\%$\uparrow$)  \\
% {\biprune} & \textbf{89}\% (0.02\%$\uparrow$) & 67\% (0.02\%$\uparrow$) & \textbf{74}\% (0.18\%$\uparrow$) & \textbf{93}\% (0.1\%$\uparrow$) &  \textbf{89}\% (0.02\%$\uparrow$)  & \textbf{49}\% (0.09\%$\uparrow$)\\ \midrule
% \bottomrule[1pt]
% \end{tabular}%
% }
% \end{table}


\begin{table}[htb]
\centering
\caption{\footnotesize{The sparsest winning tickets found by different methods at different data-model setups. \YY{Winning tickets refer to the sparse models with average test accuracy no less than the dense ones.} In each cell, $p\%$ (acc$\pm$std\%) represents the sparsity as well as the test accuracy. The test accuracy of dense models can be found in the header. {\xmark} signifies that no winning ticket  is found  by a   pruning method. Given the data-model setup (\textit{i.e.}, per column),
the sparsest winning ticket is highlighted in \textbf{bold}.
% \SL{[remove computation time from this table?]
% \SL{[wrap table?]}
% \SL{$aa, +bb$}
% \YY{Dense +-}
% }
\YY{test accuracy and std}
}}
\label{tab: sparsest_wt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{c|cccccc}
\toprule[1pt]
\midrule
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10}                               & \multicolumn{2}{c}{CIFAR-100} \\
                        & ResNet-18                 & ResNet-20                         & ResNet-56                         & VGG-16                        & ResNet-18                 & ResNet-20      \\ 
                        & (94.77\%)                 & (92.12\%)                         & (92.95\%)                         & (93.65\%)                     & (76.67\%)                 &   (68.69\%)      \\\midrule
IMP                     &  87\% (94.77$\pm$0.10\%)  &\textbf{74}\% (92.15$\pm$0.15\%)   & \textbf{74}\% (92.99$\pm$0.12\%)  & 89\% (93.68$\pm$0.05\%)       & 87\% (76.91$\pm$0.19\%)   & \xmark       \\ % Grasp ResNet56 104 min
OMP                     & 49\% (94.80$\pm$0.10\%)    & \xmark                            & \xmark                            & 20\% (93.79$\pm$0.06\%)       & 74\% (76.99$\pm$0.07\%)   & \xmark         \\
\grasp                  & \xmark                    & \xmark                            & 36\% (93.07$\pm$0.34\%)           & \xmark                        & \xmark                    & \xmark         \\
{\hydra}                & \xmark                    & \xmark                            & \xmark                            & 87\% (93.73$\pm$0.03\%)       & \xmark                    & 20\% (68.94$\pm$0.17\%)  \\
{\biprune}              & \textbf{89}\% (94.79$\pm$0.15\%)   & 67\% (92.14$\pm$0.15\%)  & \textbf{74}\% (93.13$\pm$0.04\%)  & \textbf{93}\% (93.75$\pm$0.15\%)&  \textbf{89}\% (76.69$\pm$0.18\%)  & \textbf{49}\% (68.78$\pm$0.10\%)\\ \midrule
\bottomrule[1pt]
\end{tabular}%
}
\end{table}


\begin{figure}[htb]
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-10_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-10_ResNet20s.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-100_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-100_ResNet20s.pdf} \\
    
\end{tabular}}
\caption{\footnotesize{Filter pruning trajectory given by test accuracy  (\%) vs. pruning ratio (\%). 
   The visual presentation setting is  the same as Fig.\,\ref{fig: unstructured_performance_cifar}. We observe that {\biprune}   identifies winning tickets of structured pruning in certain sparsity regimes.
    }}
\vspace*{-3mm}
\label{fig: structured_performance_cifar}
\end{figure}


\underline{Fig.\,\ref{fig: unstructured_performance_cifar}} shows the \textit{unstructured pruning trajectory} (given by test accuracy vs. sparsity ratio) of {\biprune} and baseline methods   in $8$ model-dataset setups.  For comparison, we also present the performance of the original dense model. 
As we can see, the proposed   {\biprune} approach finds the best winning tickets  (in terms of the highest accuracy) compared to the baselines across  all the pruning setups. Note that a winning ticket refers to a sparse model with test accuracy that is at least as good as the dense model (see the marked green dash line). Among the baseline methods, IMP is the  pruning method  most competitive to ours. However, the improvement brought by {\biprune}  is significant with respect to the variance of IMP, except the $60\% $-$80\%$ sparsity regime in (CIFAR-10, ResNet-20). In the case of (CIFAR-100, ResNet-20)  where IMP can not find any winning tickets (as confirmed by\,\cite{ma2021sanity}),
{\biprune} still manages to find winning tickets with around $0.6\%$ improvement over the dense model.
\YY{We only show {\biprune} and IMP performance on ImageNet due to the computational resource constraints.} 
In \underline{Tab.\,\ref{tab: sparsest_wt}},
we   summarize the sparest  winning tickets along the pruning trajectory identified by different pruning methods.  As we can see, 
{\biprune} can identify the winning tickets with higher sparsity levels than the other methods, except the case of (CIFAR-10, ResNet-20). 
We also refer readers to Appendix\,\ref{app: add_results} for more experimental results to justify the high quality of winning tickets identified by {\biprune}.


%\paragraph{Structured Pruning}
\underline{Fig.\,\ref{fig: structured_performance_cifar}} demonstrates the \textit{structured pruning trajectory}  on the CIFAR-10/100 datasets.
Here we focus on filter pruning, where filter is regarded as a masking unit in \eqref{eq: prob_bi_level}. We refer readers to Appendix\,\ref{app: add_results} for  channel-wise pruning results. \YY{The other experimental results, without further mentioning, belong to the unstructured pruning regime.} 
% Due to the page limit, we only report the results of the filter-wise pruning in the main paper and please refer to Appendix\,\ref{app: add_results} for channel-wise pruning. 
%Fig.\,\ref{fig: structured_performance_cifar} shows the performance overview of structured pruning on CIFAR-10/100. 
In comparison with    Fig.\,\ref{fig: unstructured_performance_cifar}, Fig.\,\ref{fig: structured_performance_cifar} shows that it becomes much more difficult to find winning tickets of high-accuracy and high-sparsity in the structured pruning regime, and the  gap among different pruning methods decreases. This is not surprising since
filter pruning imposes much stricter pruning structure constraints than irregular weight pruning. However, {\biprune} still outperforms all the other baselines. Most important, it can identify clear winning tickets in the low sparse regime even when IMP fails. 

% As structured pruning is a more challenging setting\cite{chen2022coarsening}, all the methods drop more quickly than its unstructured counterparts. Nevertheless, {\biprune} still manages to find winning tickets in most settings. In general, {\biprune} consistently outperforms IMP and OMP in the low-sparsity regime, while the gap becomes less significant when sparsity ratio $p\% > 60\%$. As the only difference between structured and unstructured {\biprune} implementation lies in the threshold operation, the time consumption of Fig.\,\ref{fig: unstructured_performance_cifar}
%  and Fig.\,\ref{fig: structured_performance_cifar} are very similar.


%\begin{wrapfigure}{r}{50mm}
\begin{figure}[htb]
%\vspace*{-8mm}
\centerline{
\includegraphics[width=.3\textwidth,height=!]{figure/time_comparison_cifar10_resnet18.pdf}
}
%\vspace*{-3mm}
\caption{\footnotesize{Time consumption comparison on CIFAR-10 with ResNet-18 to different pruning ratio $p$. 
% The sparsest winning tickets (WT) of {\biprune} and IMP are marked in red star. 
% {\biprune} achieves sparser winning tickets (89\% v.s. 87\% and using $7\times$ less time than IMP.
% \SL{[update it. log-y scale!!!]}
% which are with 83\% sparsity. IMP achieves similar performance (see Fig.\,\ref{fig: unstructured_performance_cifar}).to {\biprune} but spends 7 times more training time.
}}
\label{fig: time_compare_res18c10}
%\vspace*{-15mm}
%\end{wrapfigure}
\end{figure}

\paragraph{{\biprune} is computationally efficient.}
% \SL{[Please use another table to highlight computation efficiency]}
% \begin{wraptable}{r}{.52\columnwidth}
\begin{table}[htb]
\vspace*{0mm}
\centering
\caption{\footnotesize{Computation complexities of different pruning methods on (CIFAR-10, ResNet-18). The training epoch numbers of pruning/retraining  baselines are consistent with their official settings  or the latest benchmark implementations. All the evaluations are based on a single Tesla-V100 GPU. \SL{Consider to put in appendix.}}}
\label{tab: efficiency}
\resizebox{.7\columnwidth}{!}{%
\begin{tabular}{c|cccc|c}
\toprule[1pt]
\midrule
\multicolumn{5}{c|}{{Runtime v.s. targeted sparsity}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Training epoch \# \end{tabular}} \\
\multicolumn{1}{c|}{Method $\backslash$ Sparsity} &
  \multicolumn{1}{c|}{$20\%$} &
  \multicolumn{1}{c|}{$59\%$} &
  \multicolumn{1}{c|}{$83.2\%$} &
  $95.6\%$ &
   \\ \midrule
\multicolumn{1}{c|}{IMP} &
  \multicolumn{1}{c|}{69 min} &
  \multicolumn{1}{c|}{276 min} &
  \multicolumn{1}{c|}{621 min} &
  966 min &
  160 epoch retrain \\ \midrule
\grasp &
  \multicolumn{4}{c|}{89 min} &
  200 epoch retrain \\ \midrule
OMP &
  \multicolumn{4}{c|}{69 min} &
  160 epoch retrain \\ \midrule
\hydra &
  \multicolumn{4}{c|}{115 min} &
  \begin{tabular}[c]{@{}c@{}}100 epoch prune\\ 100 epoch retrain\end{tabular} \\ \midrule
\biprune &
  \multicolumn{4}{c|}{86 min} &
  100 epoch         \\ \midrule
\bottomrule[1pt]
\end{tabular}%
}
%\vspace*{-5mm}
\end{table}
% \end{wraptable}
%We demonstrate the high efficiency of {\biprune} in Tab.\,\ref{tab: sparsest_wt}, Fig.\,\ref{fig: time_compare_res18c10}.  
In our experiments, another \textbf{key observation} is that 
{\biprune} yields sparsity-agnostic runtime complexity while IMP leads to runtime exponential to the targeted sparsity.
\underline{Fig.\,\ref{fig: time_compare_res18c10}} shows the computation cost of different pruning methods versus different pruning ratios on (CIFAR-10, ResNet-18). 
For example, {\biprune} takes 86 minutes (mins) to find the sparsest winning ticket (with $89\%$ sparsity ratio in Tab.\,\ref{tab: sparsest_wt}). This yields
$7\times$ less runtime than IMP, which consumes $620$ mins to find a comparable winning ticket with $87\%$ sparsity. 
Compared to the optimization-based pruning baseline {\hydra}, {\biprune} is also more efficient as it  does not rely on the extra post-optimization model retraining; see Tab.\,\ref{tab: efficiency} for a detailed summary of runtime and training epoch numbers requested by different pruning methods. 
Further, {\biprune} takes about {1.25 $\times$} more computation time   than {\grasp} and OMP, however, the latter methods lead to poorer pruning accuracy, \textit{e.g.}, justified by the failure cases of finding winning tickets  in  Tab.\,\ref{tab: sparsest_wt}, Fig.\,\ref{fig: unstructured_performance_cifar}, and Fig.\,\ref{fig: structured_performance_cifar}.
% \SL{[Refer to appendix for more results or details?]}

\paragraph{Rewinding effect on {\biprune}.} 
Another advantage of {\biprune} is that it is \textit{not} sensitive   to  model rewinding. 
Recall that 
rewinding is a strategy used in LTH \cite{frankle2019stabilizing} to determine what model initialization should be used for re-training a pruned sparse model. As shown in \cite{ma2021sanity}, an IMP-identified winning ticket could be sensitive to the choice of a rewinding point.
\underline{Fig.\,\ref{fig: rewind_study}} shows the test accuracy of the {\biprune}-pruned model       when it is retrained at different rewinding epochs, where `N/A' in the x-axis represents the case of no retraining (and thus no rewinding).
As we can see, a carefully-tuned rewinding scheme does not lead to a significant improvement over {\biprune} without retraining. This suggests that the subnetworks found by {\biprune} are already of high quality, and justifies the improved computation efficiency of   {\biprune} over {\hydra} (that requires post-optimization model retraining), as shown in Fig.\,\ref{fig: time_compare_res18c10}. %We stress that {\biprune}
%We highlight that all of our experiments results 



% In what follows, we show that the performance of {biprune} is sensitive to neither post-optimization retraining nor the rewinding epoch, which in contrast plays an indispensable and sensitive role in the success of IMP\,\cite{frankle2019stabilizing}.
% Fig.\,\ref{fig: rewind_study} demonstrates the test accuracy of the sparse model found by {\biprune} when further retrained with different rewinding epochs. For comparison, we also present the performance of the sparse model without retraining, which is denoted as "N/A" in the x-axis. As can be seen, rewinding and retraining in general do not bring significant improvement over the retrain-free setting, indicating the subnetworks found by {\biprune} are already of high quality. Considering that all of our baselines require retraining to further boost the performance after the mask is found (see Tab.\,\ref{tab: efficiency}), our method thus spares the time-consuming retraining and further improves the efficiency. We stress that we study four sparsity ratios from different sparse levels to make sure the conclusion is consistent.

%\begin{wrapfigure}{r}{47mm}
\begin{figure}[htb]
%\vspace*{-2mm}
\centerline{
\includegraphics[width=45mm]{figure/Diff_Init_on_CIFAR-10_ResNet20s.pdf}
}
\caption{\footnotesize{The sensitivity of {\biprune} to  rewinding epochs on (CIFAR-10, ResNet-20). Each curve represents a certain sparsity level and   "N/A" in the x-asis indicates  {\biprune} without retraining.
% \SL{Please add dense model and please remove $95.6\%$.}
}}
\label{fig: rewind_study}
\vspace*{-5mm}
%\end{wrapfigure}
\end{figure}

\paragraph{Sanity check of {\biprune} on specialized hyperparameters.} 

\begin{figure}[thb]
\centerline{
\begin{tabular}{cc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/Diff_K_on_CIFAR-10_ResNet20s.pdf} 
    &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/Diff_gamma_on_CIFAR-10_ResNet20s.pdf}  
    % \\
    % \footnotesize{(a)} 
    % & 
    % \footnotesize{(b)} 
    
\end{tabular}}
\caption{\footnotesize{The sensitivity of {\biprune}  to the lower-level step number $N$ (Left) and the lower-level regularization parameter $\gamma$ (Right) at different pruning ratios on (CIFAR-10, ResNet-20). 
% \SL{Update $NA$ to $\infty$ (easier to understand in this way).
% \SL{[Let us call pruning ratio since we use $p$. Please update sparsity ratio to pruning ratio for other figures.]}
% }
}}
\vspace*{-3mm}
\label{fig: ablation_study}
\end{figure}

In \underline{Fig.\ref{fig: ablation_study}}, we   show  the sensitivity of {\biprune} to   its specialized hyperparameters at lower-level optimization, including 
the SGD number ($N$) when  customizing \eqref{eq: theta_step}, and the regularization parameter $\gamma$ in \eqref{eq: prob_bi_level}.
%and the   learning rate $\alpha$.
We refer readers to Fig.\,\ref{fig: ablation_study_full} for a more extensive study.
\underline{Fig\,\ref{fig: ablation_study}(a)} shows the test accuracy of {\biprune}-pruned  models versus the choice of $N$ at different pruning ratios. As we can see, the calling of a larger number of SGD steps at lower-level optimization does not necessarily improve the overall performance of {\biprune}. This is because in {\biprune}, the \ref{eq: theta_step} is initialized by a pre-trained dense model which does not ask for aggressive weight updating. The best performance of {\biprune} is typically achieved at $N \leq 3$. We choose $N = 1$ throughout the experiments as it is computationally lightest. 
\underline{Fig\,\ref{fig: ablation_study}(b)} shows the performance of {\biprune} against the varying $\gamma$, where `$\infty$'  in the x-axis refers to the case of IG-excluded \eqref{eq: GD_bi_level} (by considering $\gamma \to \infty$ in \ref{eq: m_step}). As we can see, the choice of $\gamma \in \{ 0.5, 1\}$ yields the best pruning accuracy across all pruning ratios. If $\gamma$ is too small, then  the lack of strong convexity of lower-level optimization would hamper the convergence. 
If $\gamma$ is too large, then lower-level optimization would largely departs from the true model training objective and thus causes a performance drop. In addition, the accuracy loss encountered at   $\gamma = \infty$ also indicates the necessity of the IG enhancement in {\biprune}. 
% This is because: 1) a very small $\gamma$ does not introduce enough convexity to the lower-level objective and hurts the performance; 2) a too large regularization term intuitively deviates the true objective and also leads to performance degradation. Note that ${1}/{\gamma}$ serves as the coefficient of the IG-associated term in \eqref{eq: upper_update_final}. Thus, we further studied its contribution by manually removing the IG term in our default setting ($\gamma$=1.0), as denoted as "N/A" in the x-axis. Note this operation will make our BLO-based algorithm degrade to an alternating optimization method. 
% As can be seen, a performance drop of around $1\%$ can be spotted across different sparsity levels when compared to its IG-enhanced counterparts. Therefore, as discussed in Sec.\,\ref{bi-level prune methodology}, the IG-enhancement is necessary to good performance and can be achieved nearly for `free' thanks to the bi-linearity of the pruning variables.



%\SL{I stop here.}



% We evaluate the quality of winning tickets from the perspectives of sparsity and accuracy. In general, sparser winning tickets with better test accuracy are preferred. 
% Fig.\,\ref{fig: unstructured_performance_cifar} 
% % and Fig.\,\ref{fig: unstructured_performance_imagenet} 
% compares the performance of different methods in the unstructured pruning setting. Several observations can be drawn. Firstly, our method {\biprune} finds the winning tickets with the best test accuracy (marked by the green dashed line) across all the settings with no exceptions. 
% %\begin{wrapfigure}{r}{50mm}


% In some extreme cases, even IMP can not find any winning tickets (\emph{e.g.}, CIFAR-100 with ResNet-20, confirmed by\,\cite{ma2021sanity}), while {\biprune} still manages to find winning tickets with around $0.5\%$ improvement on the test accuracy. Secondly, as demonstrated in Tab.\,\ref{tab: sparsest_wt}, {\biprune} is able to find winning tickets with larger sparsity than other methods in most cases. Both observations suggest the quality of the sub-networks found by {\biprune} outperforms all the baselines. We compare {\biprune} with more heuristics-based init-pruning baselines in Appendix\,\ref{app: add_results}.


 

==> Deprecated_NO_USE/Version_Camera_08041600_Submission/Deprecated_NO_USE/Version_Camera_05161900/Sec3_SL.tex <==
In this section, we begin by providing a brief   background of neural  network pruning, including the predominant   iterative magnitude pruning (IMP) method and the 
associated lottery ticket hypothesis (LTH)
\cite{frankle2018lottery} to find high-quality subnetworks (known as `winning tickets') that--when trained in isolation--reach test accuracy comparable to or even better than the original dense network. 
However, the superior performance of IMP is accompanied with a prohibitive computation cost, as will be exemplified in Fig.\,\ref{fig: one_shot_results}. In  order to overcome the computational difficulty of IMP, we next introduce the  one-shot   pruning method and elaborate on its comparison with IMP. Spurred by the pros and cons of current pruning methods, we eventually state the problem to be studied in this paper. 
 

\paragraph{{Heuristics-based IMP.}}
The heuristics-based IMP is the  currently prevailing approach  to
identify the `winning ticket' in model pruning, so as to attain model sparsity without suffering  performance loss\,\cite{frankle2018lottery,Renda2020Comparing,frankle2020linear,blalock2020state,chen2020lottery,chen2021lottery}. 
For example, the current  state-of-the-art (SOTA) implementation of IMP in \cite{ma2021sanity} can lead to a pruned ResNet-20 on
% \SL{[This example  number needs to be   better aligned with the later figure, then you can cite it here.]}
CIFAR-10 with 74\% sparsity and $92.12\%$ test accuracy, {
which is comparable to the performance of the original dense model}; see Fig.\,\ref{fig: one_shot_results}. 
% For the larger-size {ResNet-18} model, IMP   can identify a sparser network with   {$95\%$ sparsity and $94.81\%$ test accuracy, yielding the $0.5\%$ improvement over the original dense model}; \SL{see Fig.\,xxx in Sec.\,xxx}.
The algorithm of IMP typically contains two key ingredients: \textbf{(i)} a \textit{temporally-evolved pruning schedule} (given by the growing model sparsity over pruning iterations), and \textbf{(ii)} the \textit{pruning-retraining learning mechanism} applied at each pruning round. 
% To be more specific, 
% IMP  repeatedly trains, prunes, and resets the network over multiple rounds (say $n$ rounds). 
For (i), supposing that there exist $n$ pruning rounds, each round  prunes $(p\%)^{\frac{1}{n}} $ of the model
weights that survive the previous round, where $p\%$ denotes the final pruning ratio to be achieved.
%This leads to a pruning mask $\mathbf m$ at each round. 
For (ii), 
the non-zero remaining weights at each pruning round are re-set to the  weights at initialization or at an early-training epoch \cite{Renda2020Comparing}, and   re-trained till convergence. 
In brief, IMP  repeatedly trains, prunes, and resets the network over multiple rounds. 

 

% A common example, the Lottery Ticket Hypothesis (LTH), can achieve comparable or even better performance with a sparsity of over $95\%$ in its state-of-the-art (SOTA) implementation\,\cite{ma2021SanityCheckLTH}. 
% In general, the heuristics-based IMP adopts a sparsifying-retraining paradigm which consists of multiple iterative cycles: \underline{\textit{(1)}} \textbf{training} dense model with several epochs; \underline{\textit{(2)}} \textbf{pruning} $p\%$ redundant model weights with certain heuristics-based criteria (\emph{e.g.} model weight magnitude) to obtain the new mask; \underline{\textit{(3)}} \textbf{fine-tuning} the sparse network with the found mask and rewound weights for accuracy recovery. 

\begin{wrapfigure}{r}{85mm}
\vspace*{-5mm}
\centerline{
\begin{tabular}{cc}
\hspace*{0mm}\includegraphics[width=.3\textwidth,height=!]{figure/performance_comparison.pdf}  
&\hspace*{-4mm}\includegraphics[width=.31\textwidth,height=!]{figure/time_comparison_long.pdf}
% \\
% \hspace*{2mm}\footnotesize{(a) Test accuracy vs. pruning ratio.} &   \footnotesize{(b) Runtime of pruning.}
\end{tabular}}
\vspace*{-2mm}
\caption{\footnotesize{
Illustration of the pros and cons of different pruning methods executed over (ResNet-20, CIFAR-10).
(a) Test accuracy vs. different pruning ratios: IMP significantly outperforms one-shot pruning methods (\textsc{OMP}\,\cite{frankle2018lottery}, \textsc{ProsPr}\,\cite{alizadeh2022prospect}, \textsc{Grasp}\,\cite{wang2020pick}, \textsc{Snip}\,\cite{lee2018snip}, \textsc{SynFlow}\,\cite{tanaka2020pruning}). (b) Computation time of pruning to different sparsity levels:  IMP becomes much more computational intensive when pruning is targeted for a higher sparsity level. 
%We highlight we adopt the SOTA implementation of OMP  following\,\cite{ma2021sanity} and other methods following their original settings.
% \SL{For (a): Update x-y axis and mark the $95\%$ or $99\%$ pruning point.}
% \SL{For (b): [X-axis: Pruning method, add the dense model training time.]}
% \SL{Illustration of  the pros and cons of different pruning methods executed over (ResNet-xxx, CIFAR-10).
% (a) Test accuracy against pruning ratio: IMP significantly outperforms one-shot pruning methods (OMP [refs], ....). (b) Computation time of pruning to different sparsity levels:  IMP becomes much more computational intensive when pruning is targeted for a higher sparsity level ($99\%$ vs. $60\%$).
% }
% Performance and efficiency comparison between IMP (LTH) and various one-shot pruning methods on CIFAR10 and ResNet20. One-shot methods save pruning time at the cost of significant performance drop compared to IMP (LTH).
% \SL{Why ResNet20? Not ResNet18?}
}}
  \label{fig: one_shot_results}
  \vspace*{-7mm}
\end{wrapfigure}

%\SL{[I stop here]}
Yet, the superior pruning accuracy   of IMP is at the cost of  computation efficiency. For ease of illustration, Fig.\,\ref{fig: one_shot_results} shows the example of pruning ResNet-20 over CIFAR-10 and demonstrates   the accuracy and the computation time of various pruning methods versus the growing sparsity ratio.
%and (b) the computation time of model pruning with different sparsity levels.
% \SL{For ease of illustration, Fig.\,\ref{fig: one_shot_results} shows a pruning example that unveils (a) the accuracy performance of various pruning methods versus the growing sparsity ratio, and (b) the computation time of model pruning with different sparsity levels.}
As we can see, IMP outperforms   the other pruning baselines and finds 
the sparsest winning ticket (marked by the red star in Fig.\,\ref{fig: one_shot_results}a) using $n = 6$ pruning rounds. 
However, this leads to $3\times$ more than the cost of training a dense model from scratch.
% \SL{the $95\%$-sparsity ResNet-18 model with $94.81\%$ test accuracy on CIFAR-10 takes $n = xxx$ pruning rounds. This leads to $xxx$-min runtime, which is $xxx$ times higher than training a dense model and $xxx$ times higher than pruning to the $60\%$  sparsity level.} 
%and thus hampers the pruning efficiency 
%
\iffalse
Although IMP-based pruning approaches have become the rising star sub-field in pruning, its current success largely sacrifices the pruning efficiency. Within each pruning cycle, the sparse structure is obtained by removing a small fixed pruning ratio (\emph{e.g.}, $20\%$ in LTH) of the \textbf{remaining weights} to make the final sparse model match the full performance of the dense model. Thus, the required pruning iterative numbers as well as their training time grow exponentially as the sparsity increases. For example, the SOTA implementation of LTH\,\cite{ma2021SanityCheckLTH} has to go through 22 pruning cycles to arrive at a sparsity of $99\%$. In such a case, the immense training time consumption has become one clear obstacle of IMP from scaling to large model architectures and datasets\,\cite{zhang2021efficient}.
\fi 
%
\paragraph{IMP vs. one-shot pruning.}
To reduce the computation cost of IMP, different kinds of `accelerated' pruning methods were developed  \cite{zhang2021efficient, frankle2018lottery, wang2020pick,lee2018snip,tanaka2020pruning, alizadeh2022prospect}; And many of them
  fall into the \textit{one-shot pruning} category: The network is directly pruned to the eventual target sparsity level  and retrained once. 
%: the network is trained once, p% of weights are pruned, and the surviving weights are reset.
% which refines the sparse mask directly to the given sparsity only one time. 
In particular, the one-shot magnitude pruning (OMP) has been served as an important baseline that  simplifies IMP directly \cite{frankle2018lottery}.
\textsc{OMP} obeys the pruning-retraining paradigm, but it  prunes the model to the target sparsity using only one pruning round. 
% \SL{Although some existing work\,\cite{ma2021SanityCheckLTH} observed that OMP and the other one-shot pruning methods (e.g., ProsPr\,\cite{alizadeh2022prospect}) could find winning tickets and achieve similar accuracy performance to IMP. However, this conclusion is model/dataset-specific. }
% Although some preliminary results showed that 
% existing work\,\cite{ma2021sanity}(\YH{cite TBD}) observed that OMP and the other one-shot pruning methods (e.g., \textsc{ProsPr}\,\cite{alizadeh2022prospect}) could find winning tickets and achieve similar accuracy performance to IMP at low sparsity levels. However, this conclusion is model/dataset-specific. 
However,  the promise of current one-shot pruning methods is dataset/model-specific \cite{ma2021sanity, su2020sanity_random_win} and mostly lie in the low-sparsity regime \cite{alizadeh2022prospect}.
As systematically studied in \cite{frankle2020pruning,ma2021sanity}, there exists a clear performance gap between one-shot pruning and IMP.
Fig.\,\ref{fig: one_shot_results} also justifies the above limitation.
% However, the degradation in accuracy of the one-shot methods is still significant compared to IMP (LTH), making them impractical to real world applications\,\cite{frankle2020pruning}.
As we can see, although one-shot pruning  is   computationally light (Fig.\,\ref{fig: one_shot_results}b), it suffers from an evident accuracy drop compared to IMP (Fig.\,\ref{fig: one_shot_results}a), especially at the large sparsity levels.
%For example, \textsc{OMP} and \textsc{ProsPr} \cite{alizadeh2022prospect}, the SOTA methods of one-shot pruning,   yield  over $2\%$ and $10\%$ accuracy drop compared to IMP at the $74\%$ and  $98\%$ sparsity level, respectively.
Thus,  there exists a strong demand for the algorithmic advancement of model pruning that can   enjoy the dual advantages of one-shot pruning and IMP.
%\textit{i.e.}, improve the tradeoff  between computation efficiency and pruning accuracy. 
% Even the SOTA one-shot pruning method \textsc{ProsPr}\,\cite{alizadeh2022prospect} also suffers from an accuracy drop of over $10\%$ compared to IMP when $99\%$ parameters are pruned.
% As demonstrated in Figure\,, all one-shot  
%\todo{I don't see 99\% sparsity level in Figure~\ref{fig: one_shot_results}. Do we mean 90\%?
%
%\YY{Solved.}}
%
%the observed accuracy-efficiency tradeoff
%the accuracy-efficiency tradeoff of one-shot pruning is based on the heuristics-based one-shot pruning 
%This efficiency-performance trade-off is primarily due to the heuristic nature, which is insufficient to find satisfactory masks with an extreme sparsity using the radical pruning ratio as OMP does.
%
\paragraph{Problem Statement.}
As described above, the existing  one-shot pruning methods do not suffice to close the performance gap with IMP. One possible root cause is its strong   dependence   on  the heuristics-based weight sparsification strategy. This leaves the question of  whether 
computation efficiency and pruning accuracy could be co-improved through a more rigorous and dedicated optimization-based approach. 
% a theoretically-grounded optimization-based approach can renovate one-shot pruning so as to improve the computation complexity of pruning while attaining the accuracy performance comparable to IMP.
% Based on the aforementioned dilemma between performance and pruning cycle number in heuristics-based pruning methods, we ask the following question:
Thus, we ask:  \textit{Beyond heuristics, how to establish the \textbf{optimization basis} of a successful pruning mechanism that can attain high pruning  accuracy (like IMP) as well as high   computation efficiency (like one-shot pruning)?}
% \begin{center}
%     \textit{Beyond heuristics, how to establish the \textbf{optimization basis} of a successful pruning mechanism that can close the gap between pruning accuracy (e.g., achieved by IMP) and computation efficiency (e.g., achieved by OMP)?}
% \end{center}


%\newpage 


==> Deprecated_NO_USE/Version_Camera_08041600_Submission/Deprecated_NO_USE/Version_Camera_05161900/Sec4_SL.tex <==
In this section, we   re-investigate the problem of model pruning through the lens of   bi-level optimization (BLO), and show that BLO  not only provides a natural interpretation of the pruning-retraining learning paradigm but also brings in additional   design flexibilities for model pruning.
Next, we establish  the algorithmic foundation of BLO-enabled model pruning (termed bi-level pruning or {\biprune}), extended from  the implicit gradient approach. Further, we     show that {\biprune} %is a special class of BLO problems and 
can be solved as easily as the first-order alternating optimization by taking advantages of the   bi-linear nature of the pruning variables. Lastly, we summarize the   {\biprune} algorithm and its   implementation details.  

% We will show the benefits as well as the mathematical challenges brought by the BLO formulation. Next, we point out that the bi-linearity of the pruning problem falls into a special class of the BLO and thus, can be solved as easily as the first-order alternating optimization. Finally, we propose {\biprune}, an efficient first-order BLO-based model weight pruning algorithm.

\paragraph{A BLO viewpoint on model pruning}
As described in Sec.\,\ref{sec: preliminary}, the pruning-retraining learning paradigm covers   two kinds of tasks: \ding{182} pruning  to determine the sparse pattern of model weights, and \ding{183} training remaining non-zero weights  to recover the model accuracy. 
In existing optimization-based pruning methods \cite{wen2016learning,zhang2018systematic,hoefler2021sparsity,wang2020proximal}, the tasks \ding{182}-\ding{183} are  achieved by merely  optimizing   model weights,   together with penalizing their sparsity-inducing norms, \textit{e.g.}, the $\ell_1$  and $\ell_2$ norms \cite{bach2012optimization}. Different from the above formulation, we propose to  separate optimization variables involved in the pruning tasks  \ding{182} and \ding{183}. This leads to    the (binary) pruning mask variable $\mask \in \{ 0, 1\}^n$ and the model weight variable $\btheta \in \mathbb R^n$, respectively. Here $n$ denotes the total number of model parameters. 
Accordingly, the pruned model is given by $(\mathbf m \odot  \btheta)$, where $\odot$ denotes the element-wise multiplication. As will be evident later, this  \textit{variable disentanglement} enables us to 
explicitly depict the co-evolving of pruning and retraining through BLO, and    helps us to    customize  the pruning task with high flexibility.
%so as to leverage more advanced optimization techniques to achieve a better pruning solution than heuristics-based search. 



% the model mask\,$\mask$ and the corresponding model weights\,$\btheta$. In the widely accepted sparsifying-retraining pruning paradigm, the masks $\mask$ are highly dependent on the model weights $\btheta$ as the magnitude of $\btheta$ serves as the pruning criterion. In the BLO formulation, $\mask$ and $\btheta$ are optimized independently using disparate variables. This \textit{disentanglement} gives the mask variables $\mask$ more flexibility to search better optima than the heuristics-based methods. More importantly, it facilitates us to interpret the sparsifying-retraining paradigm from a bi-level optimization viewpoint. 



In what follows, we elaborate on how BLO can be established to co-optimize the pruning mask $\mathbf m$  and the retrained sparse model weights $\boldsymbol \theta$. 
%Let $\ell$ denote the training loss and .
%Let $k$ denote the targeted sparsity number, determined by the pruning ratio $p = k/d$. 
Given the pruning ratio $p\%$, the sparsity constraint   is given by $\mathbf m \in  \mathcal{S} $, where $\mathcal S = \{ \mathbf m\,|\, \mathbf m \in \{ 0, 1\}^n, \mathbf  1^T \mathbf m \leq k \}$ and $k = p\% n$.
Our goal is to  prune the original   model \textit{directly} to the targeted sparse number $k$ (\textit{i.e.}, without calling for the IMP-like sparsity schedule as described in Sec.\,\ref{sec: preliminary}) and obtain the optimized sparse model $(\mathbf m \odot \btheta)$. To this end, we interpret the pruning task (\textit{i.e.}, \ding{182}) and the model retraining task (\textit{i.e.}, \ding{183}) as \textit{two optimization levels}, where the former is formulated as an \textit{upper-level} optimization problem, and it relies  on the optimizer of the \textit{lower-level}  retraining task. We then cast the model pruning problem as the following BLO problem (with \ding{183} being nested inside \ding{182}):
\todo{Mention structured pruning? For structured pruning, manipulate m with Kronecker and transfer the element-wise pruning unit to a structured one.

% \YY{In actual implementation, we use individual m for each $\theta$, but with specific structural patterns. I agree with Pari that we can mention such manipulation.}
}%

\vspace*{-6mm}
{\small{
\begin{align}
% \vspace*{-3mm}
\displaystyle
    \begin{array}{llll}
\displaystyle \minimize_{\mathbf \mask \in \mathcal{S}}         & \underbrace{\ell(\mask \odot {\btheta}^*(\mask))}_\text{ \ding{182}: Pruning task}; 
& \quad 
  \st &  \underbrace{\displaystyle {\btheta}^*(\mask) = \argmin_{\btheta \in \mathbb{R}^n} \overbrace{ \ell(\mask\odot \btheta) + \frac{\gamma}{2} \|\btheta\|_2^2}^\text{$\Def g(\mask, \btheta)$}}_\text{\ding{183}: Sparsity-fixed model retraining},
    \end{array}
    \label{eq: prob_bi_level}
\end{align}
}}%
where $\ell$ denotes the model training loss (\textit{e.g.}, cross entropy), 
$\mathbf m$ and $\btheta$ are the upper-level and lower-level optimization variables respectively, 
${\btheta}^*(\mask)$ signifies the lower-level solution by minimizing the objective function $g$ given the pruning mask $\mathbf m$, 
and $\gamma > 0$ is a regularization parameter introduced to strongly convexify the lower-level optimization so as to stabilize the gradient flow from   $\btheta^*(\mathbf m)$ to $\mathbf m$ and thus the   convergence of BLO \cite{shaham2015understanding,hong2020two}.
%As will be evident later, the introduction of $\lambda$
In a sharp contrast to existing single-level optimization-based model pruning methods \cite{wen2016learning,zhang2018systematic,hoefler2021sparsity,wang2020proximal}, the BLO formulation \eqref{eq: prob_bi_level} brings in  \underline{two advantages}. 

\underline{First}, BLO has flexibility to use   {mismatched} pruning and retraining objectives at the upper and   lower optimization levels, respectively. This flexibility exists  for customizing not only the regularized lower-level   objective function in \eqref{eq: prob_bi_level}
but also optimization algorithm per level. To be more specific, one can  update the upper-level pruning mask $\mask$ using a data batch (called $\mathcal B_2$) distinct from the one (called $\mathcal B_1$) used for  obtaining the lower-level solution ${\btheta}^*(\mask)$. The resulting BLO procedure can then mimic the idea of  meta learning to improve model generalization \cite{deng2021meta}, where the lower-level problem fine-tunes $\btheta$ using $\mathcal B_1$, and the upper-level problem validates the generalization of the sparsity-aware finetuned model $(\mathbf m \odot \boldsymbol \theta^* (\mathbf m))$ using $\mathcal B_2$.
%By doing so, the idea of meta learning (to improve model generalization)  can be infused into  model   


\underline{Second}, BLO enables us to explicitly model and optimize the coupling  between the retained model weights $\btheta^*(\mathbf m)$ and the   pruning mask $\mathbf m$ through the implicit gradient (IG)-based optimization routine. Here IG refers to  the gradient of the lower-level solution $\btheta^*(\mathbf m)$ with respect to (w.r.t.) the upper-level variable $\mathbf m$, and its derivation  calls the implicit function theory \cite{gould2016differentiating}.
The use of     IG makes our proposed BLO-oriented pruning \eqref{eq: prob_bi_level} significantly different from the greedy alternating minimization  \cite{csiszar1984information} that learns the upper-level and lower-level variables independently (\textit{i.e.}, minimizes one variable by fixing the other). We refer readers to the following  section for the detailed  IG theory.
 We will also show in Sec.\,\ref{sec: exp} that
 %assisted by the theoretically-grounded  BLO, 
 the pruning strategy acquired from \eqref{eq: prob_bi_level} can   outperform IMP in many pruning scenarios but is much more efficient in computation as it does not call for the scheduler of iterative pruning   ratios. 
 
% A sparse model (\emph{a.k.a.} a pruned model) is defined as $f(\mask \odot \btheta)$, namely the element-wise product of a dense network $f(\btheta, \cdot)$ and a binary mask $\mathbf m$. The pruning mask $\mask \in {\{0, 1\}}^d$ has the same shape as the model parameter $\btheta$ and localizes the non-zero weights with a certain sparsity ratio $p$, where $d={\|\btheta\|_0}$ demotes the dimension of the model parameter. 
% A pruning algorithm aims to find the sub-network of the given model architecture with a certain sparse level while maintaining the performance of the pruned model at a high level. 
% The pruning problem can be readily reformulated to a hierarchical optimization problem, where the model parameter $\mask$ and the mask $\btheta$ are jointly optimized. This nested structure presents a standard bi-level optimization (BLO) formulation, which is given by% 
% {
% \small
% \begin{align}
% % \vspace*{-3mm}
% \displaystyle
%     \begin{array}{ll}
% \displaystyle \minimize_{\mathbf \mask\in \mathbb \{0, 1\}^{d}}         & f(\mask, {\btheta}^*(\mask)) 
% \\
%   \st &  \displaystyle {\btheta}^*(\mask) = \argmin_{\btheta \in \mathbb{R}^d}  g(\mask, \btheta) + \frac{\gamma}{2} \|\btheta\|_2^2,
%     \end{array}
%     \label{eq: prob_bi_level}
% \end{align}
% }%

% where $f$ and $g$ denote the upper-level and the lower-level objective functions, and $\gamma > 0$ is a quadratic regularization parameter. 
% In the BLO formulation, the upper-level problem aims to find the pruning mask based on the given model parameter $\btheta$, while the lower-level problem retrains the model parameter with the fixed sparse mask. 
% The reasons for introducing the quadratic regularization term $\frac{\gamma}{2} \|\btheta\|_2^2$ are two-fold. First, it stabilizes the lower level problem via regularization. Second, it enforces the strong convexity of the lower-level problem. A different regularizer might be adopted in different use cases. 
% % For example, in implicit MAML\,\cite{rajeswaran2019meta} used $\| \mathbf y - \mathbf x\|_2^2$ as the regularizer. 
% For example, implicit MAML\,\cite{rajeswaran2019meta} used the $\ell_2$ regularizer to stablize the parameter update. 
% Such a strongly convex regularization term is also common in the BLO analysis \cite{shaham2015understanding} to stabilize the alternative optimization convergence of BLO.

% The BLO interpretation of model pruning provides multiple advantages in contrast to the conventional sparsity promoting optimization based methods ($\btheta$-only):

% \ding{172} Formulation-wise: the nested structure of \eqref{eq: prob_bi_level} allows for \emph{different} objective functions in different levels. This flexibility further enables us to use mismatched data batches for mask finding and model training, which has been verified to be very beneficial for improving the model generalization\,\cite{deng2021meta}.

% \ding{173} Optimization-wise: the BLO formulation is uniquely suited for characterizing structure of the pruning-retraining paradigm. Different from the single-level optimization problem, BLO will use a specialized optimization routine.

% \ding{174} Compared to IMP, BLO directly optimizes the mask $\mask$ to any given sparsity in one sole pruning cycle. There is no need to adopt a small pruning ratio and achieve the large sparsity in multiple pruning cycles. This characteristic resembles one-shot pruning methods and accounts for the \textit{sparsity-agnostic} computational costs of the BLO-based pruning method.

\paragraph{Optimization foundation of {\biprune}.}
The key optimization challenge of solving the {\biprune} problem \eqref{eq: prob_bi_level} lies in the computation of IG (implicit gradient). Prior to developing an effective solution, we first elaborate on the \textit{IG  challenge}, the unique characteristic of BLO. In the context of gradient descent, the gradient of the   objective function in  \eqref{eq: prob_bi_level} yields

\vspace*{-5mm}
{
\small{
\begin{align}
\displaystyle
    \underbrace{\frac{d\ell(\mask \odot \btheta^*(\mask))}{d\mask}}_\text{Gradient of objective} = \nabla_{\mask} \ell(\mask \odot {\btheta}^*(\mask)) + \underbrace{
    \frac{{d ( {\btheta}^*(\mask)^{\top} )
    }
    %^{\top}
    }{d \mask}}_{\text{{IG}}} \nabla_{\btheta}\ell (\mask \odot \btheta^*(\mask)),
    \label{eq: GD_bi_level}
\end{align}}}%
where $\nabla_{\mask}$ and $\nabla_{\btheta}$  denote the \textit{partial derivatives} of the bi-variate function $\ell(\mask, \boldsymbol \theta)$  w.r.t. the variable $\mask$ and $\btheta$ respectively, 
$d \btheta^\top / d \mask  \in \mathbb R^{n \times n} $ denotes the vector-wise \textit{full derivative},  
and for ease of notation, we will omit
the transpose $\top$ when the context is clear.
In \eqref{eq: GD_bi_level}, the IG challenge refers to the demand for   computing gradients of  the implicit function $\btheta^*(\mask) = \argmin_{\btheta} g(\mask, \btheta)$ w.r.t. $\mask$, where recall from \eqref{eq: prob_bi_level}  that $ g(\mask, \btheta) \Def  \ell(\mask\odot \btheta) + \frac{\gamma}{2} \|\btheta\|_2^2 $.
\iffalse
To circumvent this difficulty, the conventional method is  \textit{gradient unrolling} that   approximates the lower-level solution $\btheta^*(\mask)$ using a single or a few unrolled gradient descent steps, \textit{e.g.}, 
$\btheta^*(\mask) \approx \btheta - \alpha \nabla_{\btheta} g(\mask, \btheta)$. However, this only gives a rough estimate of the lower-level solution and  lacks   theoretical rigorousness \cite{hong2020two}. Meanwhile, even in this over-simplified scenario, it is not difficult to see that the computation of   IG
%, \textit{i.e.}, $ \frac{{d {\btheta}^*(\mask)}^{\top}}{d \mask}$,  
relies on the computation of   second-order partial derivatives.
\fi 

%Different from gradient unrolling,
Next,
we derive the IG formula following the more rigorous implicit function theory \cite{gould2016differentiating,hong2020two,rajeswaran2019meta}.
%, where the stationary condition of the lower-level optimization in \eqref{eq: GD_bi_level} is treated as  a differentiable explicit   function
Based on the fact that the   $\btheta^*(\mask)$ is satisfied with the stationary condition of the lower-level objective function in \eqref{eq: GD_bi_level},  it is not difficult to obtain that 

\vspace*{-5mm}
{\small
\begin{align}
% & \displaystyle
%     %{\frac{d\btheta^*(\mask)}{d\mask}}^{\top} (\nabla_{\btheta \btheta} g(\mask, \btheta) + \gamma \mathbf{I}) + \nabla_{\mask\btheta} g(\mask, \btheta)%
%     \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) + \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%     \nabla^2_{\btheta} \ell(\mask \odot \btheta^*)
%   + \gamma \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%   = \mathbf 0; \nonumber \\
%  \Longrightarrow  &
\displaystyle  \frac{d\btheta^*(\mask)}{d\mask} %^{\top} 
 =  -   \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) [ \nabla^2_{\btheta } \ell(\mask \odot \btheta^*) + \gamma \mathbf I ]^{-1},
 \label{eq: exact_IG}
\end{align}
}%
where   $\nabla_{\mask \btheta}^2 \ell $ and $\nabla_{\btheta \btheta}^2 \ell $ denote the second-order partial derivatives of $\ell$ respectively, and $(\cdot)^{-1}$ denotes the matrix inversion operation. We refer readers to Appendix\,\ref{eq: app_IG} for the full derivation of \eqref{eq: exact_IG}.


% we   obtain 

% \vspace*{-6mm}
% {
% \small
% \begin{align}
% \displaystyle
%   %  \frac{d g(\mask, \btheta^*(m)))}{
%   %  d\btheta}
%   \nabla_{\btheta} g(\mathbf m, \btheta^* )
%     = \nabla_{\btheta} \ell(\mask \odot \btheta^* ) + \gamma \btheta^*  = \mathbf 0.
%     \label{eq: stationary}
% \end{align}
% }%
% where for ease of notation, we omit the dependence of $\btheta^*(\mask)$ w.r.t. $\mathbf m$.
% We   then take    derivative of the second equality of \eqref{eq: stationary} w.r.t. $\mask$ by using the implicit 
% function theory. This leads to \todo{\YH{Put Eq. 3-4 in the appendix or merge them into one proof? }}
% % $
% % {\frac{d\btheta^*(\mask)}{d\mask}}^{\top} (\nabla_{\btheta \btheta} g(\mask, \btheta) + \gamma \mathbf{I}) + \nabla_{\mask\btheta} g(\mask, \btheta) = \mathbf  0
% % $

% \vspace*{-5mm}
% {\small
% \begin{align}
% & \displaystyle
%     %{\frac{d\btheta^*(\mask)}{d\mask}}^{\top} (\nabla_{\btheta \btheta} g(\mask, \btheta) + \gamma \mathbf{I}) + \nabla_{\mask\btheta} g(\mask, \btheta)%
%     \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) + \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%     \nabla^2_{\btheta} \ell(\mask \odot \btheta^*)
%   + \gamma \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%   = \mathbf 0; \nonumber \\
%  \Longrightarrow  &
%  \frac{d\btheta^*(\mask)}{d\mask} %^{\top} 
%  =  -   \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) [ \nabla^2_{\btheta } \ell(\mask \odot \btheta^*) + \gamma \mathbf I ]^{-1}.
%  \label{eq: exact_IG}
% \end{align}
% }%
% where $\nabla_{\mask \btheta} \ell $ and $\nabla_{\btheta \btheta} \ell $ are the second-order partial derivatives of the bivariate function $\ell$, and $(\cdot)^{-1}$ denotes the matrix inversion operation.

Yet, the exact   IG formula \eqref{eq: exact_IG} remains difficult in calculation due to the presence of    matrix   inversion and   second-order partial derivatives.
\todo{$\gamma$ is critical in this derivation. Without $\gamma$, and with the $\nabla^2_{\btheta} = 0$ assumption, this does not go through. How do we best motivate the introduction of $\gamma$ in (1) since standard pruning setups and schemes dont introduce such regularization term?}
To  simplify it, 
we impose the Hessian-free assumption, 
$ \nabla^2_{\btheta} \ell = \mathbf 0$, which  is mild in general; For example,   the decision boundaries of neural networks with ReLU activations are piece-wise linear in  a tropical hyper-surface \cite{alfarra2020decision}, and this assumption 
%is   necessary as  computing the Hessian matrix w.r.t.   model parameters $\btheta$ would be practically infeasible, and it
has been widely used in meta learning \cite{finn2017model}. Given $ \nabla^2_{\btheta } \ell = \mathbf 0$,  the matrix inversion in \eqref{eq: exact_IG} can   be then mitigated, leading to the IG formula

\vspace*{-5mm}
{\small
\begin{align}
    \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
    =  -  \frac{1}{\gamma} \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ).
    \label{eq: IG_simplify}
\end{align}
}%

At the first glance, the computation of the simplified IG   \eqref{eq: IG_simplify} still requires the mixed (second-order) partial derivative $\nabla^2_{\mask \btheta} \ell$. However, {\biprune} is a special class of BLO problems with bi-linear variables 
$(\mask \odot \btheta)$. Based on this bi-linearity, we can prove that  IG  in \eqref{eq: IG_simplify} can be \textit{analytically} expressed using only \textit{first-order} derivatives; see the following theorem. 

% \begin{tcolorbox}[colback=black!5!white,colframe=white!20!black]
\begin{myprop}
\label{thr: ig}
Assuming $\nabla^2_{ \btheta} \ell = 0$, the implicit gradient \eqref{eq: IG_simplify} is then given by

\vspace*{-5mm}
{\small
\begin{align}
\displaystyle
\frac{d\btheta^*(\mask)}{d\mask} %^{\top} 
% =  -  \frac{1}{\gamma} \nabla_{{\mask} {\btheta}} \ell ({\mask} \odot {\btheta}^*) 
= -  \frac{1}{\gamma} \mathrm{diag}( \nabla_{\mathbf z} \ell(\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right.);
% := -\frac{1}{\gamma} \mathrm{diag}(\mathbf{A}).
\label{eq: IG_final}
\end{align}
}%
% The rationale behind Hessian-free assumption is that commonly used ReLU-based neural network tends to form a piece-wise linear decision boundary \emph{w.r.t.} the model parameter $\btheta$. This has been theoretically proved by \,\cite{alfarra2020decision}. Empirical results \cite{finn2017model} also suggest that the absence of the second-order derivative hardly harms the performance of the BLO algorithm. 
Further, the   gradient of the  objective function given by \eqref{eq: GD_bi_level} becomes

{\vspace*{-3mm}
{
\small
\begin{align}
\displaystyle
    \frac{d \ell(\mask \odot \btheta^*)}{d \mask} = ( \btheta^* 
    - 
    \frac{1}{\gamma} \mask \odot \gradzsimple) \odot \gradzsimple,
    \label{eq: upper_update_final}
\end{align}}}%
where for ease of notation    {$\gradzsimple$} signifies {$\gradz$}, and recall that $\odot$ denotes the element-wise multiplication.
\end{myprop}
%\end{tcolorbox}
\textbf{Proof}: Using chain-rule, we can obtain that

\vspace*{-4mm}
{\small
\begin{align}
&    \nabla_{\btheta}\ell(\mask \odot \btheta^*) = %\nabla_{\btheta^*} (\mask \odot \btheta^*)^\top
\mathrm{diag}(\mathbf m)
\gradzsimple = \mask \odot \gradzsimple;
    \label{eq: chainrule_theta} \\
\text{similarly,   } & \nabla_\mask \ell(\mask \odot \btheta^*) 
    % = \nabla_\mask (\mask \odot \btheta^*)^\top \gradzsimple 
    % = \mathrm{diag}(\btheta^*) \gradzsimple 
    = \mathrm{diag}(\btheta^*) \gradzsimple 
    = \btheta^* \odot \gradzsimple \label{eq: chainrule_mask}
\end{align}
}%%
where $\mathrm{diag}(\cdot)$ represents a diagonal matrix with $\cdot$ being the main diagonal vector.
% Similarly, we also have $\nabla_{\btheta^*}\ell(\mask \odot \btheta^*) = \mask \odot \gradzsimple$. 
% For simplicity, we denote $\gradz$ as $\gradzsimple$. 
Further, we can convert \eqref{eq: IG_simplify} to

\vspace*{-4mm}
{
\small
\begin{align}
\displaystyle
    \nabla^2_{{\mask} {\btheta}} \ell({\mask}  \odot {\btheta^*}) 
    % & = \nabla_{{\mask}} \left [ \mathrm{diag}({\mask}) {\gradzsimple} \right ] \\
    & \overset{\eqref{eq: chainrule_theta}}{=} \nabla_{{\mask}} \left [ {\mask} \odot  \nabla_{\mathbf z} \ell(\mathbf z) \right ]
    \nonumber \overset{\text{chain rule}}{=} 
    \mathrm{diag}( {\gradzsimple}) 
    + 
    \mathrm{diag}({\mask}) [ \nabla_{{\mask}} ( \nabla_{\mathbf z} \ell(\mathbf z) ) ]
    % \mask \odot 
    % [\btheta^* \odot \nabla_{\mathbf z \mathbf z} \ell (\mathbf z) 
    % \left |_{\mathbf z = {\mask} \odot {\btheta^*}} \right. 
     \nonumber \\
    & \overset{\eqref{eq: chainrule_mask}}{=}  \mathrm{diag}( {\gradzsimple}) 
    + 
    \mathrm{diag}({\mask}) [ \mathrm{diag}(\btheta^*) \nabla^2_{\mathbf z } \ell(\mathbf z) ] = \mathrm{diag}(\gradzsimple) ,\label{eq: ezBiP}
 \end{align}}%
where the last equality holds due to the Hessian-free assumption. With \eqref{eq: ezBiP} and \eqref{eq: IG_simplify} we can prove \eqref{eq: IG_final}.
% of $\nabla_{\btheta \btheta} \ell = \mathbf 0$.

Next, substituting the IG \eqref{eq: IG_final}  to the upper-level gradient \eqref{eq: GD_bi_level}, we  obtain that

\vspace*{-3mm}
{
\small
\begin{align}
\displaystyle
     \frac{d \ell(\mask \odot \btheta^*)}{d \mask} 
    & \,\,\,\,=\nabla_{\mask}\ell({\mask} \odot {\btheta}^*) - 
    {\frac{1}{\gamma}
    \gradzsimple
    % \mathbf{A}
    \odot \nabla_{{\btheta}} \ell({\mask} \odot {\btheta^*})
    } \nonumber \\
    &
    \underset{ }{\overset{\eqref{eq: chainrule_theta}, \eqref{eq: chainrule_mask}}{=}}  \btheta^* \odot \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right.
    - \frac{1}{\gamma} \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right. 
    \odot
    ( \mask \odot \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right. 
    ) 
    %\nonumber \\
   % & \,\,\,\,
    =  (\btheta^* - \frac{1}{\gamma} \mask \odot \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right.
    ) \odot \gradzsimple, \nonumber
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right. 
   % \label{eq: upper_final_proof}
\end{align}
}%
which leads to \eqref{eq: upper_update_final}. 
The proof is now complete. \hfill $\square$ 
\todo{Do we have any empirical evidence that shows that using \eqref{eq: upper_update_final} is better than using \eqref{eq: chainrule_mask}? That would be good to highlight advantage of BLO and IG. 

\YY{Pari means the significance of the extra term brought by IG.} }

The key insight drawn from Prop.\,\ref{thr: ig} is that the bi-linearity of pruning variables (\textit{i.e.}, $\mask \odot \boldsymbol \theta^*$) makes the  IG-involved gradient \eqref{eq: GD_bi_level} easily computed, and the   computational complexity is almost same as that of computing the first-order gradient $\nabla_{\mathbf z} \ell (\mathbf z)$ just once, as supported by   \eqref{eq: upper_update_final}.
%\todo{Pari: computational complexity corollary}
 
\begin{mycor}
Given $\mask \in \{0, 1\}^n, \btheta \in \mathbb R^n$ and that the computation of the gradient $\nabla_{\mathbf z} \ell (\mathbf z) \in \mathbb R^n$ takes $O(n)$ time, the computation of the loss gradient~\eqref{eq: GD_bi_level} with respect to the mask $\mask$ of the objective~\eqref{eq: prob_bi_level} using \eqref{eq: upper_update_final} in Proposition~\ref{thr: ig} takes $O(n)$ time.
\end{mycor}
% Thus, we can prove \eqref{eq: upper_update_final}. As \eqref{eq: upper_update_final} suggests, the upper-level gradient update only involves one backward-propagation and thus, the bi-level pruning can be solved as easily as a first-order alternating optimization problem.

%\SL{[I stop here.]}
\paragraph{{\biprune} algorithm and implementation.}
%Assisted by Prop.\,\ref{thr: ig}, 
We will next 
formalize the {\biprune} algorithm 
%solve the {\biprune} problem \eqref{eq: prob_bi_level} 
based on Prop.\,\ref{thr: ig} and the alternating gradient descent method \cite{hong2020two}. At iteration $t$, there exist two main steps.

\todo{\YY{Hi Pari, feel free to elaborate on the algorithm with the way that you think is the best}}

\ding{72} \textit{Lower-level SGD for model retraining}: 
Given $\mask^{(t-1)}$, $\btheta^{(t-1)}$, and 
$\mathbf z^{(t-1)} \Def \mask^{(t-1)} \odot \btheta^{(t-1)}$, we update $\btheta^{(t)}$ by applying SGD (stochastic gradient descent) to the lower-level problem of \eqref{eq: prob_bi_level},%


\vspace*{-5mm}
{\small 
\begin{align}
    \btheta^{(t)} & = \btheta^{(t-1)} - \alpha \nabla_{\btheta} g(\mask^{(t-1)}, \btheta^{(t-1)})  \nonumber \\
   &  \hspace*{-5mm}
   \overset{%\eqref{eq: stationary}, 
   \eqref{eq: chainrule_theta}}{=}
    \btheta^{(t-1)} - \alpha [ \mask^{(t-1)} \odot 
    \nabla_{\mathbf z} \ell(\mathbf z )\left | \right._{\mathbf z = \mathbf z^{t-1}} + \gamma \btheta^{(t-1)} ],
    %\nabla_{\btheta} g(\mask^{(t-1)}, \btheta^{(t-1)}) 
    \tag{$\btheta$-step}
    \label{eq: theta_step}
\end{align}}%
where $\alpha > 0$ is the lower-level   learning rate.

\ding{72} \textit{Upper-level PGD for pruning}: Given $\mask^{(t-1)}$, $ \btheta^{(t)}$, and $\mathbf z^{(t+1/2)} \Def \mask^{(t-1)} \odot \btheta^{(t)}$, we update   $\mask$ using   PGD (projected gradient descent) along the IG-enhanced descent direction \eqref{eq: GD_bi_level},%

\vspace*{-5mm}
{\small
\begin{align}
    \mask^{(t)} = & \mathcal P_{\mathcal S} \left [ 
    \mask^{(t-1)}  - \beta  \frac{d \ell(\mask \odot \btheta^{(t)})}{d \mask} \left | \right._{\mask =     \mask^{(t-1)} }
    \right ] \nonumber \\
\overset{\eqref{eq: upper_update_final}}{=}    
    &\mathcal P_{\mathcal S} \left [ 
    \mask^{(t-1)}  - \beta  \left ( \btheta^{(t)} - 
    \frac{1}{\gamma} \mask^{(t-1)} \odot \gradzsimple \left | \right._{\mathbf z = \mathbf z^{(t+1/2)}} \right ) \odot \gradzsimple  \left | \right._{\mathbf z = \mathbf z^{(t+1/2)}}
    \right ],
    \tag{$\mask$-step}
    \label{eq: m_step}
\end{align}}%
where $\beta > 0$ is the upper-level learning rate, and $\mathcal P_{\mathcal S}(\cdot)$ denotes the Euclidean projection   onto the constraint set $\mathcal S$ given by
$\mathcal S = \{ \mathbf m\,|\, \mathbf m \in \{ 0, 1\}^n, \mathbf  1^T \mathbf m \leq k \}$ in \eqref{eq: prob_bi_level} and is achieved by the top-$k$ hard-thresholding operation as will be detailed later.  

In {\biprune}, the \eqref{eq: theta_step} and \eqref{eq: m_step} steps execute iteratively till convergence. In practice, we find that {\biprune} converges very well; see Fig.\,\ref{fig: convergence} for an ablation study.
It is also worth noting that both \eqref{eq: theta_step} and \eqref{eq: m_step} steps only require the first-order information $\nabla_{\mathbf z} \ell (\mathbf z)$, demonstrating that the {\biprune} algorithm can be conducted as efficiently as first-order optimization. 
We present more implementation details of {\biprune}   below.


\ding{70} \textit{Discrete optimization over $\mask$:} We follow the  {`convex relaxation + hard thresholding'} mechanism used in \cite{sehwag2020hydra,ramanujan2020sHiddenSubnetwork}.
Specifically, we relax the binary masking variables   to continuous masking   scores $\mathbf m \in [\mathbf 0, \mathbf 1]$. We then acquire  loss gradients at  the backward pass based on the relaxed  $\mathbf m$. At the forward pass, we project it  onto the discrete constraint set $\mathcal S$ using the hard thresholding operator, where   its top $k$ elements  are set by  $1$s and the others by $0$s. 
%At  to tn he backward pass for grationadient calculation, we 

\ding{70} \textit{Data batch selection for lower-level and upper-level optimization:} We adopt different data batches (with the same batch size) when implementing \eqref{eq: theta_step} and \eqref{eq: m_step}. This is one BLO's advantage of, which owns the flexibility to customize the lower-level and upper-level optimization problems. And the use of diverse data batches  is beneficial to model generalization as shown in \cite{deng2021meta}. 
 
\ding{70} \textit{Hyperparameter tuning:} As described in \eqref{eq: theta_step}-\eqref{eq: m_step},  {\biprune} needs to set two learning rates $\alpha$ and $\beta$ for lower-level and upper-level optimization, respectively. We choose $\alpha = 0.01$ and $\beta = 0.1$ in all experiments, where we adopt the mask learning rate $\beta$ from Hydra\,\cite{sehwag2020hydra} and set a smaller lower-level learning rate $\alpha$, as $\btheta$ is initialized by a pre-trained dense model. We show ablation study on $\alpha$ in Fig.\,\ref{fig: ablation_study}(c).
% The more aggressive lower-level optimization is typically suggested by the convergence of BLO \cite{hong2020two}. 
BLO also brings in the low-level convexification parameter $\gamma $. We set $\gamma = 1.0 $ in   experiments and refer readers to {Fig.\,\ref{fig: ablation_study}(b)} for a sanity check. 

\ding{70} \textit{One-shot vs. multi-step SGD:}
In  \eqref{eq: theta_step}, the   one-step SGD is used and helps reduce the computation overhead. In practice, we also find that the one-step SGD is sufficient:  The use of multi-step SGD in {\biprune} does not yield much significant improvement over the one-step version; see {Fig.\,\ref{fig: ablation_study}(a)}.
%computation-friendly. 

\ding{70} \textit{Extension to structured pruning:}
We formulate and solve the {\biprune} problem in the context of unstructured (element-wise)  weight pruning. However, if define the pruning mask $\mask$ corresponding to model's structure units  (\textit{e.g.}, filters), then it is easy to apply {\biprune} to structured weight pruning; see Fig.\,\ref{fig: structured_performance_cifar} and Fig.\,\ref{fig: structured_performance_cifar_appendix} for empirical results.

\iffalse
Next we give some implementation remarks on our algorithm. We adopt the commonly used Cross-Entropy loss as our upper- and lower-level loss functions. To circumvent the difficulty from discrete optimization for binary mask $\mask$, we adopt the widely accepted 
\textbf{soft score + hard threshold} paradigm to deal with $\mask$. We first loosen the binary constraint of $\mask$ from $\{0, 1\}^n$ to $\mathbb R^{n}$ as the `mask score'. After each step, for any given sparsity ratio $p\%$, we update the true binary mask by setting the top $1-p\%$ elements with the highest score to $1$ and the rest to $0$. We emphasize the {\biprune} can be applied to the structured pruning setting simply by changing the threshold operation by wipe out the parameter patterns (\emph{e.g.}, the convolutional kernel) with the lowest score $\ell_2$ norms. In practice, we use different batches $\mathcal{B}_\alpha$ and $\mathcal{B}_\beta$ for upper- and lower-level updates for better generalization ability. {In practice, we will show that the performance of {\biprune} is not sensitive to the lower level step number $K$ in Sec\,\ref{sec: exp}. Thus, unless otherwise specified, we report the results with $K=1$.}
\todo{Can we discuss $\mask_t$ update more formally like $\mask_{t+1} \gets P_\mathcal{S} (\mask_t - \beta (7))$?}
\fi 
% For initialization, the model parameter $\btheta_0$ are initialized with \textit{Kaiming Normal}\,\cite{he2015delving} and 

\iffalse
The mask scores $\mask_0$ are scaled proportionate to the model weights\,\cite{sehwag2020hydra} and the initial binary mask $\mask$ is initialized \emph{w.r.t.} the score initialization $\mask_0$. We use separate learning rates for upper and lower-level problem namely $0.1$ for sparse mask and $0.01$ for model parameter. We further set the lower-level problem regularization coefficient to $0.1$.  We will show in Sec.\,\ref{sec: exp} these hyper-parameter choices are consistently used in all settings and are easy to tune.
\fi 
% In our algorithm, we choose the upper- and lower-level objective as the commonly used model training loss function $\ltr$, such as Cross-Entropy loss. 
% Our algorithm is shown in Algorithm\,\ref{alg: BiP}. 
% In our implementation, we adopt the \textbf{soft score + hard threshold} paradigm to train the discrete variable $\mask$. We first loosen the binary constraint of $\mask$ from $\{0, 1\}^d$ to $\mathbb R^{d}$ as the `mask score'. After each step, for any given sparsity ratio $p\%$, we update the true binary mask $\mathbf{z}^*$ by setting the top $1-p\%$ elements with the highest score to $1$ and the rest to $0$ (denoted as threshold operation $\mathcal{T}_{\{0,1\}^d}$ in \eqref{eq: threshold}). We emphasize the {\biprune} can be applied to the structured pruning setting simply by changing the threshold operation by wipe out the parameter patterns (\emph{e.g.}, the convolutional kernel) with the lowest score $\ell_2$ norms.

% We use separate learning rates for upper and lower-level problem namely $0.1$ for sparse mask and $0.01$ for model parameter. We further set the lower-level problem regularization coefficient to $0.1$.  We will show in Sec.\,\ref{sec: exp} these hyper-parameter choices are consistently used in all settings and are easy to tune.
% For initialization, 
% the model parameter $\btheta_0$ are initialized with \textit{Kaiming Normal}\,\cite{he2015delving} and the mask scores $\mask_0$ are scaled proportionate to the model weights\,\cite{sehwag2020hydra}. 
% The initial binary mask $\mathbf{z}^*$ is initialized \emph{w.r.t.} $\mask_0$. 

% \newpage 


==> Deprecated_NO_USE/Version_Camera_08041600_Submission/Deprecated_NO_USE/Version_Camera_05161900/exp_SL.tex <==
In this section, we present extensive experiment results to show the effectiveness of {\biprune}  
%in both accuracy and   efficiency
across multiple model architectures,  various datasets, and different pruning setups. Compared to IMP, one-shot pruning, and optimization-based pruning baselines, 
we find that {\biprune} leads to better winning tickets in most cases and is computationally as efficient as one-shot pruning. 

\subsection{Experiment Setup}
\paragraph{Datasets and models.}
Following the pruning benchmark in \cite{ma2021sanity}, 
we consider 4 datasets including CIFAR-10\,\cite{krizhevsky2009learning}, CIFAR-100\,\cite{krizhevsky2009learning}, Tiny-ImageNet\,\cite{le2015tiny}, ImageNet\,\cite{deng2009imagenet}, and 5
architecture types  including  ResNet-20/56/18/50
% \SL{[do we really need RN here?]}
and VGG-16 \cite{he2016deep,simonyan2014very}. 
%ResNet\,\cite{he2016deep}, VGG\,\cite{simonyan2014very}\} for evaluation. 
Tab.\,\ref{table: impl_details} summarizes these dataset and model information and setups.  

% For more details on the dataset-model architecture combination, please refer to Table\,\ref{table: impl_details}.
% We summarize our detailed training setups and hyper-parameter selections in Table\,\ref{table: impl_details}. For both unstructured and structured pruning, we adopt two architecture series ResNet\,\cite{he2016deep} and VGG\,\cite{simonyan2014very} for four representative datasets, namely \emph{i.e.,} CIFAR-10\,\cite{krizhevsky2009learning}, CIFAR-100\,\cite{krizhevsky2009learning}, Tiny-ImageNet\,\cite{le2015tiny}, and ImageNet\,\cite{deng2009imagenet}. 



\paragraph{Baselines,  training, and evaluation.}
When comparing with {\biprune}, we mainly focus on 4 state-of-the-art (SOTA) pruning methods, \ding{172} IMP \cite{frankle2018lottery}, \ding{173} OMP \cite{frankle2018lottery},
% \SL{[refs; be consistent with earlier sections]}
 \ding{174} {\grasp} \cite{wang2019picking} (a one-shot pruning method by analyzing gradient flow at initialization), and \ding{175} {\hydra} \cite{sehwag2020hydra} (an optimization-based pruning method that optimizes masking scores). It is worth noting that there exist various implementations of IMP, \textit{e.g.}, specified by different learning rate and model initialization `rewinding' strategies \cite{Renda2020Comparing}. To make a fair comparison, we follow the recent IMP benchmark in \cite{ma2021sanity}, which can find the best winning tickets over current heuristics-based pruning baselines.
We also remark that {\hydra} is originally proposed for improving adversarial robustness of a pruned model, but it can be easily customized for standard pruning when setting the adversary's strength as $0$ \cite{sehwag2020hydra}. We choose {\hydra} as a baseline because it can be regarded as a specification of {\biprune}, given by a single-level sparse mask optimization task together with post-optimization weight re-training. 
When implementing {\biprune}, unless specified otherwise, we use the $1$-step SGD in \eqref{eq: theta_step}, and set the learning rates $(\alpha, \beta)$ and the lower-level regularization parameter $\gamma$ as described in the previous section. When implementing baselines, we follow their official code repository setups.
We evaluate the performance of {\biprune} and the above baselines mainly from two perspectives:14
(1) the test accuracy of the obtained sub-network, and (2) the runtime of pruning to reach the desired sparsity. 
We refer readers to Tab.\,\ref{tab: training_details}, Appendix\,\ref{app: training} for more training and evaluation details, such as training epochs, learning rate schedulers, and so forth. 

% In unstructured pruning settings, we compare {\biprune} with various heuristics-based and optimization-based baselines, including IMP\,\cite{frankle2019stabilizing}, OMP, \grasp\,\cite{wang2019picking}, and \hydra\,\cite{sehwag2020hydra}. To make a fair comparison, we adopt the recommended training settings from their papers and we adopt the SOTA implementation following\,\cite{ma2021sanity} for IMP and OMP. {\hydra} is an optimization-based baseline framework, which is originally designed for robust pruning, but can be customized to standard pruning as mentioned in its paper\,\cite{sehwag2020hydra}. 
%For complete and detailed training details please refer to Appendix\,\ref{app: training}.

% \begin{wrapfigure}{r}{85mm}
% \vspace*{-5mm}
% \centerline{
% \begin{tabular}{cc}
% \hspace*{0mm}\includegraphics[width=.3\textwidth,height=!]{figure/Global_Pruning_on_TinyImageNet_ResNet18.pdf}  
% &\hspace*{-6mm}\includegraphics[width=.3\textwidth,height=!]{figure/Global_Pruning_on_ImageNet_ResNet18.pdf}
% \\
% \hspace*{2mm}\footnotesize{(a) Tiny-ImageNet with ResNet-18} &   \footnotesize{(b) ImageNet with ResNet-50}
% \end{tabular}}
% % \vspace*{-2mm}
% \caption{\footnotesize{
% Unstructured pruning test accuracy (\%) v.s. sparsity (\%) on Tiny-ImageNet and ImageNet. Other settings remain the same as Fig.\,\ref{fig: unstructured_performance_cifar}.
% % Models are pruned up to $90\%$ following\,\cite{ma2021sanity}. 
% \YH{ImageNet is still incomplete.}}}
%   \label{fig: unstructured_performance_imagenet}
% %   \vspace*{-4mm}
% \end{wrapfigure}


% We consider two different structured pruning settings with different pruning granularity of a convolutional layer,  termed filter-wise and channel-wise pruning. In general, the parameters of a convolutional layer have a shape of [$c_{\text{out}}$, $c_{\text{in}}$, w, h], which denote the output channel number, input channel number, kernel width and kernel height respectively.
% The filter-wise pruning\,\cite{chen2022coarsening} remove the model 
% parameters following a basic pattern of [$c_{\text{in}}$, w, h] while the channel-wise following [$c_{\text{out}}$, w, h]. The sparsity ratio of each layer is kept the same as the target sparsity $p\%$. Please refer to Fig.\,\ref{fig: illustration} for illustration on the two settings.
% We choose the OMP and IMP as our baselines in both structured pruning settings. Due to the page limit, we only report the results of filter-wise pruning in the main paper and include the channel-wise in Appendix\,\ref{app: add_results}, while the both settings lead to consistent conclusions.


% \paragraph{Evaluation Setups.}
% We mainly evaluate the performance of {\biprune} and the other baselines from two perspectives. 
% %As our method is dedicated to achieve high pruning accuracy (like IMP) with less computational burden (like OMP), we
% particularly pay attention to the following two metrics:
% % to the quality of the sparse networks and the pruning efficiency.
% % evaluate the quality of the found sparse network (see \ding{182}-\ding{183}) and the pruning efficiency (see \ding{184}) when evaluating a method. In particular, we pay attention to the following metrics: 
% (1) the test accuracy of the obtained sub-network, and (2) the runtime of pruning to reach the desired sparsity. 

%  (How good?) the quality of the sub-networks: besides the test accuracy of the target sparsity, we also study the best winning tickets and the sparsest winning tickets that can be found by each method across different sparsities. The former reveals the maximum potential of a pruning method to improve the test accuracy over the dense model. The latter depicts how sparse the method can go without losing any accuracy.
% % : the improvement on the test accuracy of the best winning ticket compared to dense model. \ding{183} (How sparse?) the sparsest winning ticket: winning ticket with the largest sparsity found by each method 
% \ding{183} (How fast?) pruning efficiency: this includes the required time to reach the given sparsity as well as to find the best/sparsest winning tickets.
% % reach the given sparsity as well as 
% % this includes the time spent for finding the sparsest winning ticket and for the whole pruning process. For structured pruning in particular, we also compare the inference efficiency (FLOPs) of the found sparse networks.




\subsection{Experiment Results}

\paragraph{{\biprune}   identifies high-accuracy winning tickets.} 
In what follows, we peer into the quality of winning tickets identified by {\biprune}.
%\textit{pruning trajectory} (given by test accuracy vs. pruning ratio) of {\biprune} and baseline methods.
\textit{Two  key observations} can be drawn from our experiment results: (1)  {\biprune}   finds winning tickets of higher accuracy and/or higher  sparsity than  the baselines in most cases (as shown in Fig.\,\ref{fig: unstructured_performance_cifar} and Tab.\,\ref{tab: sparsest_wt}; (2)  The superiority of {\biprune} holds for both unstructured pruning and structured pruning (as shown in Fig.\,\ref{fig: structured_performance_cifar} and Fig.\,\ref{fig: structured_performance_cifar_appendix}
% \SL{, and xxx}
). 


\begin{figure}
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_ResNet20.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_ResNet56s.pdf} &
    \hspace*{-5mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_VGG16.pdf} \\
    
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-100_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-100_ResNet20s.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_TinyImageNet_ResNet18.pdf} &
    \hspace*{-5mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_ImageNet_ResNet50.pdf}
\end{tabular}}
\caption{\footnotesize{Unstructured pruning trajectory given by test accuracy (\%) vs. sparsity (\%) on various dataset-model pairs.
%with ResNet-18/20/56 and VGG-16.
The proposed \textcolor{Green}{\biprune} is compared with \textcolor{blue}{\hydra}\,\cite{sehwag2020hydra}, \textcolor{orange}{IMP}\,\cite{ma2021sanity}, \textcolor{ompcolor}{OMP}\,\cite{ma2021sanity}, \textcolor{Purple}{\grasp}\,\cite{wang2019picking}. And the performance of   dense model and that of the best winning ticket  are marked using   dashed lines in each plot. 
%the mean (solid line) and variance (shaded area) of accuracies over \SL{xxx} random trials are reported for each pruning method 
    The solid line and shaded area of each pruning method represent  the mean and variance of test accuracies over 3 independent trials. We observe that
    {\biprune}  consistently outperforms the other baselines.
}}
\label{fig: unstructured_performance_cifar}
\end{figure}



% \begin{table}[htb]
% \centering
% \caption{\footnotesize{The sparsest winning tickets found by different methods at different data-model setups. In each cell, $p\%$ ($t$ min) represents the sparsity as well as the time consumption to find the sparsest winning ticket. {\xmark} signifies that no winning ticket  is found  by a   pruning method. Given the data-model setup (\textit{i.e.}, per column),
% the sparsest winning ticket is highlighted in \textbf{bold}.
% \SL{[remove computation time from this table?]
% \SL{[wrap table?]}
% \SL{$aa, +bb$}
% }
% }}
% \label{tab: sparsest_wt}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{c|cccccc}
% \toprule[1pt]
% \midrule
% \multirow{2}{*}{Method} & \multicolumn{4}{c}{CIFAR-10}                               & \multicolumn{2}{c}{CIFAR-100} \\
%                         & ResNet-18    & ResNet-20    & ResNet-56    & VGG-16        & ResNet-18    & ResNet-20      \\ \midrule
% IMP        &  87\% (620 min) &\textbf{74}\% (200 min) & \textbf{74}\% (462 min) & 89\% (501 min) &  87\% (620 min) & \xmark       \\ % Grasp ResNet56 104 min
% OMP                     & 49\% (69 min) & \xmark & \xmark & 20\% (50 min) & 74\% (69 min)       & \xmark         \\
% \grasp                  & \xmark & \xmark & 36\% (104 min) & \xmark & \xmark       & \xmark         \\
% {\hydra}                & \xmark       & \xmark       & 20\% (188 min) & 87\% (108 min)  & \xmark       & 20\% (86 min)   \\
% {\biprune} & \textbf{89}\% (86 min)  & 67\% (65 min)  & \textbf{74}\% (179 min)  & \textbf{93}\% (118 min) &  \textbf{89}\% (86 min) & \textbf{49}\% (65 min) \\ \midrule
% \bottomrule[1pt]
% \end{tabular}%
% }
% \end{table}

% \begin{table}[htb]
% \centering
% \caption{\footnotesize{The sparsest winning tickets found by different methods at different data-model setups. \YY{Winning tickets refer to the sparse models with close performance to the dense ones.} In each cell, $p\%$ ($acc \pm std \%$) represents the sparsity as well as the test accuracy. The test accuracy of dense models can be found in the header. {\xmark} signifies that no winning ticket  is found  by a   pruning method. Given the data-model setup (\textit{i.e.}, per column),
% the sparsest winning ticket is highlighted in \textbf{bold}.
% % \SL{[remove computation time from this table?]
% % \SL{[wrap table?]}
% % \SL{$aa, +bb$}
% % \YY{Dense +-}
% % }
% \YY{test accuracy and std}
% }}
% \label{tab: sparsest_wt}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{c|cccccc}
% \toprule[1pt]
% \midrule
% \multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10}                               & \multicolumn{2}{c}{CIFAR-100} \\
%                         & ResNet-18    & ResNet-20    & ResNet-56    & VGG-16        & ResNet-18    & ResNet-20      \\ 
%                         & (94.77\%)      & (92.12\%)        & (92.95\%)       & (93.65\%)   & (76.67\%)   &   (68.69\%)      \\\midrule
% IMP        &  87\% (0.01\%$\uparrow$) &\textbf{74}\% (0.03\%$\uparrow$) & \textbf{74}\% (0.04\%$\uparrow$) & 89\% (0.03\%$\uparrow$) &  87\% (0.24\%$\uparrow$) & \xmark       \\ % Grasp ResNet56 104 min
% OMP                     & 49\% (0.03\%$\uparrow$) & \xmark & \xmark & 20\% (0.14\%$\uparrow$)  & 74\% (0.32\%$\uparrow$)    & \xmark         \\
% \grasp                  & \xmark & \xmark & 36\% (0.12\%$\uparrow$)& \xmark & \xmark       & \xmark         \\
% {\hydra}                & \xmark       & \xmark       & \xmark  & 87\% (0.08\%$\uparrow$)  & \xmark       & 20\% (0.25\%$\uparrow$)  \\
% {\biprune} & \textbf{89}\% (0.02\%$\uparrow$) & 67\% (0.02\%$\uparrow$) & \textbf{74}\% (0.18\%$\uparrow$) & \textbf{93}\% (0.1\%$\uparrow$) &  \textbf{89}\% (0.02\%$\uparrow$)  & \textbf{49}\% (0.09\%$\uparrow$)\\ \midrule
% \bottomrule[1pt]
% \end{tabular}%
% }
% \end{table}


\begin{table}[htb]
\centering
\caption{\footnotesize{The sparsest winning tickets found by different methods at different data-model setups. \YY{Winning tickets refer to the sparse models with average test accuracy no less than the dense ones.} In each cell, $p\%$ (acc$\pm$std\%) represents the sparsity as well as the test accuracy. The test accuracy of dense models can be found in the header. {\xmark} signifies that no winning ticket  is found  by a   pruning method. Given the data-model setup (\textit{i.e.}, per column),
the sparsest winning ticket is highlighted in \textbf{bold}.
% \SL{[remove computation time from this table?]
% \SL{[wrap table?]}
% \SL{$aa, +bb$}
% \YY{Dense +-}
% }
\YY{test accuracy and std}
}}
\label{tab: sparsest_wt}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{c|cccccc}
\toprule[1pt]
\midrule
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10}                               & \multicolumn{2}{c}{CIFAR-100} \\
                        & ResNet-18                 & ResNet-20                         & ResNet-56                         & VGG-16                        & ResNet-18                 & ResNet-20      \\ 
                        & (94.77\%)                 & (92.12\%)                         & (92.95\%)                         & (93.65\%)                     & (76.67\%)                 &   (68.69\%)      \\\midrule
IMP                     &  87\% (94.77$\pm$0.10\%)  &\textbf{74}\% (92.15$\pm$0.15\%)   & \textbf{74}\% (92.99$\pm$0.12\%)  & 89\% (93.68$\pm$0.05\%)       & 87\% (76.91$\pm$0.19\%)   & \xmark       \\ % Grasp ResNet56 104 min
OMP                     & 49\% (94.80$\pm$0.10\%)    & \xmark                            & \xmark                            & 20\% (93.79$\pm$0.06\%)       & 74\% (76.99$\pm$0.07\%)   & \xmark         \\
\grasp                  & \xmark                    & \xmark                            & 36\% (93.07$\pm$0.34\%)           & \xmark                        & \xmark                    & \xmark         \\
{\hydra}                & \xmark                    & \xmark                            & \xmark                            & 87\% (93.73$\pm$0.03\%)       & \xmark                    & 20\% (68.94$\pm$0.17\%)  \\
{\biprune}              & \textbf{89}\% (94.79$\pm$0.15\%)   & 67\% (92.14$\pm$0.15\%)  & \textbf{74}\% (93.13$\pm$0.04\%)  & \textbf{93}\% (93.75$\pm$0.15\%)&  \textbf{89}\% (76.69$\pm$0.18\%)  & \textbf{49}\% (68.78$\pm$0.10\%)\\ \midrule
\bottomrule[1pt]
\end{tabular}%
}
\end{table}


\begin{figure}[htb]
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-10_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-10_ResNet20s.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-100_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-100_ResNet20s.pdf} \\
    
\end{tabular}}
\caption{\footnotesize{Filter pruning trajectory given by test accuracy  (\%) vs. pruning ratio (\%). 
   The visual presentation setting is  the same as Fig.\,\ref{fig: unstructured_performance_cifar}. We observe that {\biprune}   identifies winning tickets of structured pruning in certain sparsity regimes.
    }}
\vspace*{-3mm}
\label{fig: structured_performance_cifar}
\end{figure}


\underline{Fig.\,\ref{fig: unstructured_performance_cifar}} shows the \textit{unstructured pruning trajectory} (given by test accuracy vs. sparsity ratio) of {\biprune} and baseline methods   in $8$ model-dataset setups.  For comparison, we also present the performance of the original dense model. 
As we can see, the proposed   {\biprune} approach finds the best winning tickets  (in terms of the highest accuracy) compared to the baselines across  all the pruning setups. Note that a winning ticket refers to a sparse model with test accuracy that is at least as good as the dense model (see the marked green dash line). Among the baseline methods, IMP is the  pruning method  most competitive to ours. However, the improvement brought by {\biprune}  is significant with respect to the variance of IMP, except the $60\% $-$80\%$ sparsity regime in (CIFAR-10, ResNet-20). In the case of (CIFAR-100, ResNet-20)  where IMP can not find any winning tickets (as confirmed by\,\cite{ma2021sanity}),
{\biprune} still manages to find winning tickets with around $0.6\%$ improvement over the dense model.
\YY{We only show {\biprune} and IMP performance on ImageNet due to the computational resource constraints.} 
In \underline{Tab.\,\ref{tab: sparsest_wt}},
we   summarize the sparest  winning tickets along the pruning trajectory identified by different pruning methods.  As we can see, 
{\biprune} can identify the winning tickets with higher sparsity levels than the other methods, except the case of (CIFAR-10, ResNet-20). 
We also refer readers to Appendix\,\ref{app: add_results} for more experimental results to justify the high quality of winning tickets identified by {\biprune}.


%\paragraph{Structured Pruning}
\underline{Fig.\,\ref{fig: structured_performance_cifar}} demonstrates the \textit{structured pruning trajectory}  on the CIFAR-10/100 datasets.
Here we focus on filter pruning, where filter is regarded as a masking unit in \eqref{eq: prob_bi_level}. We refer readers to Appendix\,\ref{app: add_results} for  channel-wise pruning results. \YY{The other experimental results, without further mentioning, belong to the unstructured pruning regime.} 
% Due to the page limit, we only report the results of the filter-wise pruning in the main paper and please refer to Appendix\,\ref{app: add_results} for channel-wise pruning. 
%Fig.\,\ref{fig: structured_performance_cifar} shows the performance overview of structured pruning on CIFAR-10/100. 
In comparison with    Fig.\,\ref{fig: unstructured_performance_cifar}, Fig.\,\ref{fig: structured_performance_cifar} shows that it becomes much more difficult to find winning tickets of high-accuracy and high-sparsity in the structured pruning regime, and the  gap among different pruning methods decreases. This is not surprising since
filter pruning imposes much stricter pruning structure constraints than irregular weight pruning. However, {\biprune} still outperforms all the other baselines. Most important, it can identify clear winning tickets in the low sparse regime even when IMP fails. 

% As structured pruning is a more challenging setting\cite{chen2022coarsening}, all the methods drop more quickly than its unstructured counterparts. Nevertheless, {\biprune} still manages to find winning tickets in most settings. In general, {\biprune} consistently outperforms IMP and OMP in the low-sparsity regime, while the gap becomes less significant when sparsity ratio $p\% > 60\%$. As the only difference between structured and unstructured {\biprune} implementation lies in the threshold operation, the time consumption of Fig.\,\ref{fig: unstructured_performance_cifar}
%  and Fig.\,\ref{fig: structured_performance_cifar} are very similar.


%\begin{wrapfigure}{r}{50mm}
\begin{figure}[htb]
%\vspace*{-8mm}
\centerline{
\includegraphics[width=.3\textwidth,height=!]{figure/time_comparison_cifar10_resnet18.pdf}
}
%\vspace*{-3mm}
\caption{\footnotesize{Time consumption comparison on CIFAR-10 with ResNet-18 to different pruning ratio $p$. 
% The sparsest winning tickets (WT) of {\biprune} and IMP are marked in red star. 
% {\biprune} achieves sparser winning tickets (89\% v.s. 87\% and using $7\times$ less time than IMP.
% \SL{[update it. log-y scale!!!]}
% which are with 83\% sparsity. IMP achieves similar performance (see Fig.\,\ref{fig: unstructured_performance_cifar}).to {\biprune} but spends 7 times more training time.
}}
\label{fig: time_compare_res18c10}
%\vspace*{-15mm}
%\end{wrapfigure}
\end{figure}

\paragraph{{\biprune} is computationally efficient.}
% \SL{[Please use another table to highlight computation efficiency]}
% \begin{wraptable}{r}{.52\columnwidth}
\begin{table}[htb]
\vspace*{0mm}
\centering
\caption{\footnotesize{Computation complexities of different pruning methods on (CIFAR-10, ResNet-18). The training epoch numbers of pruning/retraining  baselines are consistent with their official settings  or the latest benchmark implementations. All the evaluations are based on a single Tesla-V100 GPU. \SL{Consider to put in appendix.}}}
\label{tab: efficiency}
\resizebox{.7\columnwidth}{!}{%
\begin{tabular}{c|cccc|c}
\toprule[1pt]
\midrule
\multicolumn{5}{c|}{{Runtime v.s. targeted sparsity}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Training epoch \# \end{tabular}} \\
\multicolumn{1}{c|}{Method $\backslash$ Sparsity} &
  \multicolumn{1}{c|}{$20\%$} &
  \multicolumn{1}{c|}{$59\%$} &
  \multicolumn{1}{c|}{$83.2\%$} &
  $95.6\%$ &
   \\ \midrule
\multicolumn{1}{c|}{IMP} &
  \multicolumn{1}{c|}{69 min} &
  \multicolumn{1}{c|}{276 min} &
  \multicolumn{1}{c|}{621 min} &
  966 min &
  160 epoch retrain \\ \midrule
\grasp &
  \multicolumn{4}{c|}{89 min} &
  200 epoch retrain \\ \midrule
OMP &
  \multicolumn{4}{c|}{69 min} &
  160 epoch retrain \\ \midrule
\hydra &
  \multicolumn{4}{c|}{115 min} &
  \begin{tabular}[c]{@{}c@{}}100 epoch prune\\ 100 epoch retrain\end{tabular} \\ \midrule
\biprune &
  \multicolumn{4}{c|}{86 min} &
  100 epoch         \\ \midrule
\bottomrule[1pt]
\end{tabular}%
}
%\vspace*{-5mm}
\end{table}
% \end{wraptable}
%We demonstrate the high efficiency of {\biprune} in Tab.\,\ref{tab: sparsest_wt}, Fig.\,\ref{fig: time_compare_res18c10}.  
In our experiments, another \textbf{key observation} is that 
{\biprune} yields sparsity-agnostic runtime complexity while IMP leads to runtime exponential to the targeted sparsity.
\underline{Fig.\,\ref{fig: time_compare_res18c10}} shows the computation cost of different pruning methods versus different pruning ratios on (CIFAR-10, ResNet-18). 
For example, {\biprune} takes 86 minutes (mins) to find the sparsest winning ticket (with $89\%$ sparsity ratio in Tab.\,\ref{tab: sparsest_wt}). This yields
$7\times$ less runtime than IMP, which consumes $620$ mins to find a comparable winning ticket with $87\%$ sparsity. 
Compared to the optimization-based pruning baseline {\hydra}, {\biprune} is also more efficient as it  does not rely on the extra post-optimization model retraining; see Tab.\,\ref{tab: efficiency} for a detailed summary of runtime and training epoch numbers requested by different pruning methods. 
Further, {\biprune} takes about {1.25 $\times$} more computation time   than {\grasp} and OMP, however, the latter methods lead to poorer pruning accuracy, \textit{e.g.}, justified by the failure cases of finding winning tickets  in  Tab.\,\ref{tab: sparsest_wt}, Fig.\,\ref{fig: unstructured_performance_cifar}, and Fig.\,\ref{fig: structured_performance_cifar}.
% \SL{[Refer to appendix for more results or details?]}

\paragraph{Rewinding effect on {\biprune}.} 
Another advantage of {\biprune} is that it is \textit{not} sensitive   to  model rewinding. 
Recall that 
rewinding is a strategy used in LTH \cite{frankle2019stabilizing} to determine what model initialization should be used for re-training a pruned sparse model. As shown in \cite{ma2021sanity}, an IMP-identified winning ticket could be sensitive to the choice of a rewinding point.
\underline{Fig.\,\ref{fig: rewind_study}} shows the test accuracy of the {\biprune}-pruned model       when it is retrained at different rewinding epochs, where `N/A' in the x-axis represents the case of no retraining (and thus no rewinding).
As we can see, a carefully-tuned rewinding scheme does not lead to a significant improvement over {\biprune} without retraining. This suggests that the subnetworks found by {\biprune} are already of high quality, and justifies the improved computation efficiency of   {\biprune} over {\hydra} (that requires post-optimization model retraining), as shown in Fig.\,\ref{fig: time_compare_res18c10}. %We stress that {\biprune}
%We highlight that all of our experiments results 



% In what follows, we show that the performance of {biprune} is sensitive to neither post-optimization retraining nor the rewinding epoch, which in contrast plays an indispensable and sensitive role in the success of IMP\,\cite{frankle2019stabilizing}.
% Fig.\,\ref{fig: rewind_study} demonstrates the test accuracy of the sparse model found by {\biprune} when further retrained with different rewinding epochs. For comparison, we also present the performance of the sparse model without retraining, which is denoted as "N/A" in the x-axis. As can be seen, rewinding and retraining in general do not bring significant improvement over the retrain-free setting, indicating the subnetworks found by {\biprune} are already of high quality. Considering that all of our baselines require retraining to further boost the performance after the mask is found (see Tab.\,\ref{tab: efficiency}), our method thus spares the time-consuming retraining and further improves the efficiency. We stress that we study four sparsity ratios from different sparse levels to make sure the conclusion is consistent.

%\begin{wrapfigure}{r}{47mm}
\begin{figure}[htb]
%\vspace*{-2mm}
\centerline{
\includegraphics[width=45mm]{figure/Diff_Init_on_CIFAR-10_ResNet20s.pdf}
}
\caption{\footnotesize{The sensitivity of {\biprune} to  rewinding epochs on (CIFAR-10, ResNet-20). Each curve represents a certain sparsity level and   "N/A" in the x-asis indicates  {\biprune} without retraining.
% \SL{Please add dense model and please remove $95.6\%$.}
}}
\label{fig: rewind_study}
\vspace*{-5mm}
%\end{wrapfigure}
\end{figure}

\paragraph{Sanity check of {\biprune} on specialized hyperparameters.} 

\begin{figure}[thb]
\centerline{
\begin{tabular}{cc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/Diff_K_on_CIFAR-10_ResNet20s.pdf} 
    &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/Diff_gamma_on_CIFAR-10_ResNet20s.pdf}  
    % \\
    % \footnotesize{(a)} 
    % & 
    % \footnotesize{(b)} 
    
\end{tabular}}
\caption{\footnotesize{The sensitivity of {\biprune}  to the lower-level step number $N$ (Left) and the lower-level regularization parameter $\gamma$ (Right) at different pruning ratios on (CIFAR-10, ResNet-20). 
% \SL{Update $NA$ to $\infty$ (easier to understand in this way).
% \SL{[Let us call pruning ratio since we use $p$. Please update sparsity ratio to pruning ratio for other figures.]}
% }
}}
\vspace*{-3mm}
\label{fig: ablation_study}
\end{figure}

In \underline{Fig.\ref{fig: ablation_study}}, we   show  the sensitivity of {\biprune} to   its specialized hyperparameters at lower-level optimization, including 
the SGD number ($N$) when  customizing \eqref{eq: theta_step}, and the regularization parameter $\gamma$ in \eqref{eq: prob_bi_level}.
%and the   learning rate $\alpha$.
We refer readers to Fig.\,\ref{fig: ablation_study_full} for a more extensive study.
\underline{Fig\,\ref{fig: ablation_study}(a)} shows the test accuracy of {\biprune}-pruned  models versus the choice of $N$ at different pruning ratios. As we can see, the calling of a larger number of SGD steps at lower-level optimization does not necessarily improve the overall performance of {\biprune}. This is because in {\biprune}, the \ref{eq: theta_step} is initialized by a pre-trained dense model which does not ask for aggressive weight updating. The best performance of {\biprune} is typically achieved at $N \leq 3$. We choose $N = 1$ throughout the experiments as it is computationally lightest. 
\underline{Fig\,\ref{fig: ablation_study}(b)} shows the performance of {\biprune} against the varying $\gamma$, where `$\infty$'  in the x-axis refers to the case of IG-excluded \eqref{eq: GD_bi_level} (by considering $\gamma \to \infty$ in \ref{eq: m_step}). As we can see, the choice of $\gamma \in \{ 0.5, 1\}$ yields the best pruning accuracy across all pruning ratios. If $\gamma$ is too small, then  the lack of strong convexity of lower-level optimization would hamper the convergence. 
If $\gamma$ is too large, then lower-level optimization would largely departs from the true model training objective and thus causes a performance drop. In addition, the accuracy loss encountered at   $\gamma = \infty$ also indicates the necessity of the IG enhancement in {\biprune}. 
% This is because: 1) a very small $\gamma$ does not introduce enough convexity to the lower-level objective and hurts the performance; 2) a too large regularization term intuitively deviates the true objective and also leads to performance degradation. Note that ${1}/{\gamma}$ serves as the coefficient of the IG-associated term in \eqref{eq: upper_update_final}. Thus, we further studied its contribution by manually removing the IG term in our default setting ($\gamma$=1.0), as denoted as "N/A" in the x-axis. Note this operation will make our BLO-based algorithm degrade to an alternating optimization method. 
% As can be seen, a performance drop of around $1\%$ can be spotted across different sparsity levels when compared to its IG-enhanced counterparts. Therefore, as discussed in Sec.\,\ref{bi-level prune methodology}, the IG-enhancement is necessary to good performance and can be achieved nearly for `free' thanks to the bi-linearity of the pruning variables.



%\SL{I stop here.}



% We evaluate the quality of winning tickets from the perspectives of sparsity and accuracy. In general, sparser winning tickets with better test accuracy are preferred. 
% Fig.\,\ref{fig: unstructured_performance_cifar} 
% % and Fig.\,\ref{fig: unstructured_performance_imagenet} 
% compares the performance of different methods in the unstructured pruning setting. Several observations can be drawn. Firstly, our method {\biprune} finds the winning tickets with the best test accuracy (marked by the green dashed line) across all the settings with no exceptions. 
% %\begin{wrapfigure}{r}{50mm}


% In some extreme cases, even IMP can not find any winning tickets (\emph{e.g.}, CIFAR-100 with ResNet-20, confirmed by\,\cite{ma2021sanity}), while {\biprune} still manages to find winning tickets with around $0.5\%$ improvement on the test accuracy. Secondly, as demonstrated in Tab.\,\ref{tab: sparsest_wt}, {\biprune} is able to find winning tickets with larger sparsity than other methods in most cases. Both observations suggest the quality of the sub-networks found by {\biprune} outperforms all the baselines. We compare {\biprune} with more heuristics-based init-pruning baselines in Appendix\,\ref{app: add_results}.


 

==> Deprecated_NO_USE/Version_Camera_08041600_Submission/Sec1_Old.tex <==
\section{Introduction (1 page)}

% \paragraph{Contributions.}
% Discuss the importance and the development of DNN pruning

% \fakepara{the DNN prevails and pruning is necessary}
Deep neural networks (DNNs) have dramatically revolutionized the state-of-the-art performance in various fields\,\cite{krizhevsky2012imagenet, brown2020language}. As a key to increase the generalization of the DNNs\,\cite{bartlett2021deep}, the over-parameterized structures also bring its own problem. The millions or even billions of parameters not only increase computational costs during inference, but also raise great challenges for deployment on the resource-limited devices\,\cite{han2015deep}. Thus, the model pruning techniques has become the research hot spot recent years to remove redundant parameters and reduce the model size\,\cite{han2015deep, blalock2020state}.
\SL{[Add more song han's work.]}
% Deep neural networks (DNNs) have boosted their performances in many areas, \emph{e.g.,} computer vision and natural language processing \cite{krizhevsky2012imagenet, brown2020language}. However, DNNs of increasingly large sizes, despite their generalization brought by the over-parameterization \cite{bartlett2021deep}, hinder themselves from being deployed on computational resource-limited devices \cite{han2015deep}. Therefore, pruning is proposed and has become one effective method to remove redundant parameters as for improving the inference efficiency and the storage of large DNNs \cite{han2015deep, blalock2020state}.

% \fakepara{LTH is the predominant one while too computationally expensive.}
Among numerous studies on model pruning algorithms\,\cite{lecun1989optimal, ren2018admmnn,  ramanujan2020sHiddenSubnetwork}, the heuristics-based Iterative Magnitude Pruning (IMP) is the current dominant approach to achieve model sparsity 
\SL{without suffering performance loss, as suggested and empirically justified by the Lottery Ticket Hypothesis (LTH) \cite{frankle2018lottery,Renda2020Comparing,frankle2020linear,blalock2020state,chen2020lottery,chen2021lottery}.}
% \SL{and it is justified by} the Lottery Ticket Hypothesis (LTH) serves as one of the most well-known approaches to attain sparse sub-networks without suffering performance loss. 
LTH hypothesizes the existence of a sub-network (the so-called `winning ticket'), when trained from the scratch, can match the performance of the full model. The core idea of LTH lies in repetitively calling the pruning-retraining cycle and prunes a small ratio of the remaining parameters at each round. However, the achieved winning ticket is often at the cost of \SL{much} more computations than training a dense model from scratch, which hinders its scalability towards large dataset and large model architectures. 
\todo{Is LTH an algorithm or a hypothesis that motivates algorithms like IMP? \SL{IMP is defined prior to LTH. LTH is a hypothesis to state that IMP works and can find winning tickets and suggests a formal and refined IMP pipeline to surely find these winning tickets justified by experiments.}}
To improve the efficiency of IMP, numerous heuristics-based one-shot pruning methods\,\cite{lee2018snip, frankle2018lottery,ma2021sanity,  wang2020pick, tanaka2020pruning, alizadeh2022prospect}, \emph{e.g.}, one-shot magnitude pruning (OMP), have been proposed, which directly prunes the model to the target sparsity and achieves significant speedup compared to IMP. However, all the current one-shot methods   encountered \SL{evident} performance drop, leading to small odds to find winning tickets\,\cite{ma2021sanity}.
\todo{substantiate with citations or support otherwise}

% Among numerous studies on designing model pruning algorithms \cite{lecun1989optimal, ren2018admmnn,  ramanujan2020sHiddenSubnetwork}, a rising representative study focuses on obtaining sparse subnetworks out of dense unpruned models \cite{frankle2018lottery, ma2021sanity}. It is claimed that a dense, randomly-initialized neural network contains a subnetwork (so-called "winning ticket") that can match the test accuracy of the original network after training with the same algorithm.

% IMP is the SOTA way to figure out the sparse model
% The heuristics-based iterative magnitude pruning (IMP) is one of the most promising methods to identify the "winning ticket" in model pruning \cite{ma2021sanity}. However, its repetitive training and rewinding procedures make it time-consuming and prevent it from large dataset and architecture schemes. There are also heuristics-based one-shot pruning methods \cite{ma2021sanity, frankle2018lottery, wang2020pick, lee2018snip, tanaka2020pruning, alizadeh2022prospect} that deliver efficient sparsification solutions but can hardly find winning tickets as IMP does. 

% \fakepara{current optimization-based pruning methods save time but are weak. is fundamental improvement possible?}
Another research direction is 
the optimization-based pruning methods \cite{sehwag2020hydra, ramanujan2020sHiddenSubnetwork, lee2020layer, csordas2020neural, ren2018admmnn}, which still follow the pruning-retraining paradigm and adopt sparsity regularization\,\cite{liu2019admm, wang2020neural}  or parameterized masking\,\cite{csordas2020neural, ramanujan2020sHiddenSubnetwork, sehwag2020hydra} to promote sparsity. However, current optimization-based pruning methods still suffer from a non-negligible performance gap from IMP and can hardly find the winning tickets.
\todo{substantiate with citations or support otherwise}
This motivates us to rethink the fundamentals of this research direction: can we advance the optimization basis of the optimization-based pruning and achieve comparable or even better performance than IMP?
% are then motivated to find sub-networks with better performance more efficiently. 
% These methods adopt the pruning-retraining paradigm either by the method of sparsity regularization \cite{liu2019admm, wang2020neural}  or parameterized masking \cite{csordas2020neural, ramanujan2020sHiddenSubnetwork, sehwag2020hydra}. However, they can not find winning tickets but only result in sub-networks with close performance to the dense ones. This motivates us to rethink this direction: is there any missing point that stops us from reaching the winning ticket from the optimization view?

% There are also some one-shot, init-pruned methods but can not achieve as good performance as IMP does. \textsc{OMP}\,\cite{frankle2018lottery}, \textsc{ProsPr}\,\cite{alizadeh2022prospect}, \textsc{Grasp}\,\cite{wang2020pick}, \textsc{Snip}\,\cite{lee2018snip}, \textsc{SynFlow}\,\cite{tanaka2020pruning}

% There are also optimization-based pruning, Hydra to achieve robustness, hidden network to only achieve better performance than OMP. Are there any missing points for optimization-based methods? We should rethink.

% \fakepara{BLO is good framework but algorithm is too complicated.}

\begin{wrapfigure}{r}{60mm}
\vspace*{-4mm}
\centerline{
\includegraphics[width=58mm]{figure/main_compare.pdf}
}
\caption{\footnotesize{
A performance snapshot of the proposed {\biprune} method vs. the IMP baseline and the original dense model across three pruned ResNet models (ResNet-20, ResNet-56, and ResNet-18) with 74\% sparsity on CIFAR-10. The marker size indicates the model size (\textit{i.e.}, the remaining model parameters). And the uni-color   region corresponds to the same model type used by different pruning methods.
% of test accuracy of pruned models (with 74\% sparsity) and 
% CIFAR-10 test accuracy and training time of three different network architectures by {\biprune} and IMP at the sparsity ratio of 74\%.
% % compared to dense models. 
% The size of markers indicates model parameter counts.
}}
\label{fig: intro}
\vspace*{-4mm}
\end{wrapfigure}


To tackle the above challenge, we revisit the pruning problem from a fresh and novel viewpoint of bi-level optimization (BLO). 
In the new formulation, we show that BLO provides a technically-grounded optimization basis for an efficient implementation of the pruning-retraining learning paradigm. 
% In the new formulation, the pruning and retraining tasks are cast as the upper- and lower-level problem with disentangled variables and objectives. 



To the best of our knowledge, this is the first work making a rigorous connection between pruning and BLO. Technically, we propose a novel \textbf{bi}-level optimization-enabled \textbf{p}runing method (termed {\biprune}).  We further show {\biprune} takes advantage of the bi-linearity of the pruning variables and avoids the computationally intensive nature of the common BLO methods. More specifically, {\biprune} can be solved as easily as the first-order alternating optimization problem. Practically, extensive experiments demonstrate the superiority of the proposed {\biprune} in terms of accuracy, sparsity, and efficiency. {\biprune} achieves the best winning tickets in all settings with only OMP-level time consumption. As Fig.\,\ref{fig: intro} shows, {\biprune} achieves winning tickets with 5$\times$ speedup compared to IMP on CIFAR-10 with ResNet-18 in the sparsity of 74\%.
\todo{MINOR: in fig~\ref{fig: intro} make axis labels, legend and arch name larger}

% Inspired from studies that apply parameterized masks to search better sub-networks, we propose the first study into bi-level optimization based pruning ({\biprune}), separating the mask searching and the model weight tuning. Such disentanglement indicates the flexibility to use mismatched pruning and retraining objectives. On the other hand, the bi-level architecture enables the coupling between model weights and pruning masks through the implicit gradient-based routine.

% Hydra style; Layer-wise style; Chen Fan literature mentioned Bernoulli based masking; These studies inspired us to rethink optimization-based pruning from a bi-level point of view, which disentangles weights and masks naturally, and enjoys the benefits of the more accurate estimation of upper-level gradients. 

% \fakepara{Our technical summary on BLO with bi-linear nature.}

% However, BLO generally brings in extra computational costs, which may hinder the efficiency by optimization-based pruning. We will show in Sec.\,\ref{bi-level prune methodology} that, thanks to the bi-linearity of {\biprune} optimizes, the second-order derivative introduced by the implicit gradient can be solved as easily as the first-order derivative only alternative optimization. We further demonstrate that, with extensive experiments, BLO not only brings sparser and more accurate winning ticket, but also improves the efficiency of the whole process. As shown in Fig.\,\ref{fig: unstructured_performance_cifar}, our {\biprune} method consistently outperforms other methods in terms of accuracy, sparsity, and efficiency. 

% Thanks to the bi-linear formulation brought by the coupling of the masks and weights, we can come to the first-order derivative only form to solve the pruning-retraining pipeline. 



% Finally, we conclude experimental results on both structured and unstructured pruning with 5 model architectures and 4 popular datasets. We show that 



Our main contributions are listed as the following aspects:

\noindent $\bullet$ (Formulation-wise) We reformulate the model pruning problem as a bi-level optimization (BLO) problem. We show that the new formulation not only advances the optimization foundation of the pruning problem, but also provides a natural interpretation of the widely-accepted pruning-retraining paradigm. More importantly, the new formulation disentangles model pruning and retraining variables and provides more flexibility to design mismatched objectives at the upper and lower optimization levels.
% To our best knowledge, we are the first to rethink the optimization-based pruning from a bi-level point of view. We show that the bi-level optimization (BLO) not only inherits the spirit of the pruning-retraining paradigm but also brings in the design flexibility for model pruning.

\noindent $\bullet$ (Algorithmic-wise), we propose a new pruning algorithm {\biprune} based on our new BLO formulation and the implicit gradient theory. Different from the ordinary computationally intensive BLO methods, we theoretically show that {\biprune} can be solved as easily as the first-order optimization by taking advantage of the bi-linear nature of the pruning variables. 
% We propose the bi-level pruning (BiP) algorithm and prove that the implicit gradient (IG) term brought by the bi-level formulation can be solved with only first-order derivatives. The bi-linearity of the pruning problem optimizes allows simplification of the IG computation, accelerating the execution of {\biprune}.  

\noindent $\bullet$ (Experiment-wise) We conduct extensive experiments across 4 datasets (CIFAR-10/100, Tiny-ImageNet and ImageNet), 5 model architectures, and 2 pruning settings (unstructured and structured pruning). We show that {\biprune} combines the high accuracy of the predominant iterative magnitude pruning (IMP) and the high efficiency of the one-shot pruning schemes. Specifically, (i) {\biprune} achieves higher test accuracy than IMP and finds the best winning tickets in all settings. (ii) {\biprune} enjoys high pruning efficiency (comparable to one-shot pruning schemes), and achieves $2\sim7\times$ speedup over IMP for the same level of model accuracy and sparsity.
% We conduct extensive experiments to validate our method {\biprune} on diverse datasets (\emph{i.e.,} CIFAR-10/100, Tiny-ImageNet, and ImageNet) across multiple network architectures, including various ResNets and VGG. Specifically, our unstructural winning tickets achieve up to 2\% improvement over the unpruned dense models and 3-7$\times$ speedup compared to IMP for the same level of model accuracy and sparsity.


\clearpage

==> Deprecated_NO_USE/Version_Camera_08041600_Submission/Sec1_PR.tex <==
\vspace*{-2mm}
\section{Introduction }
\vspace*{-2mm}
% \SL{[Updated]}
%
Deep neural networks (DNNs) have dramatically improved the state-of-the-art in various fields~\citep{krizhevsky2012imagenet, brown2020language}. While over-parameterized structures are key to the improved generalization of DNNs~\citep{bartlett2021deep}, they create new problems -- the millions or even billions of parameters not only increase computational costs during inference, but also pose serious deployment challenges on resource-limited devices~\citep{han2015deep}. As a result, model pruning has seen a lot of research interest in recent years, focusing on reducing model sizes by removing (or pruning) redundant parameters~\citep{han2015deep, blalock2020state, han2015learning, he2018amc, mao2017exploring}.
% \SL{[Add more song han's work. \YY{Solved}]}

% \fakepara{LTH is the predominant one while too computationally expensive.}
Among various proposed model pruning algorithms\,\cite{blalock2020state,lecun1989optimal, ren2018admmnn, ramanujan2020sHiddenSubnetwork, frankle2018lottery, Renda2020Comparing, frankle2020linear, chen2020lottery, chen2021lottery,lee2018snip, ma2021sanity, wang2020pick,tanaka2020pruning, alizadeh2022prospect, sehwag2020hydra, lee2020layer,csordas2020neural},
the heuristics-based Iterative Magnitude Pruning (IMP) is the current dominant approach to achieving model sparsity without suffering performance loss, as suggested and empirically justified by the Lottery Ticket Hypothesis (LTH) \cite{frankle2018lottery}.
The LTH hypothesizes the existence of a sub-network (the so-called `winning ticket') when trained in isolation (\textit{e.g.}, from either a random initialization \cite{frankle2018lottery} or an early-rewinding point of dense model training \cite{frankle2020linear}),
%\todo{should we introduce ``rewinding'' here?\\ \YY{I use the word "trained in isolation" instead of "retrained from scratch" to try to include all rewinding and random intiialization scanarios}\\ PR: might need to think more -- I think rewinding \& random init (i.e. from scratch) are diff. init schemes, right? And for IMP, we try both to see which gives best performance, right? \\ \YY{Yes. I agree}}
can match the performance of the original dense model \cite{blalock2020state,frankle2018lottery,Renda2020Comparing,frankle2020linear,chen2020lottery,chen2021lottery}. The core idea of IMP is to iteratively prune and retrain the model while progressively pruning a small ratio of the remaining weights in each iteration, and continuing till the desired pruning ratio has been reached. While IMP often finds the winning ticket, it incurs the cost of repeated model retraining from scratch, making it prohibitively expensive for large datasets or large model architectures \cite{you2019drawing, zhang2021efficient}.
%
To improve the efficiency of model pruning, numerous heuristics-based one-shot pruning methods\,\cite{frankle2018lottery, lee2018snip, ma2021sanity, wang2020pick, tanaka2020pruning, alizadeh2022prospect}, \emph{e.g.}, one-shot magnitude pruning (OMP), have been proposed. These schemes directly prune the model to the target sparsity and are significantly more efficient than IMP. 
{Yet,  the promise of current one-shot pruning methods is dataset/model-specific~\cite{ma2021sanity, su2020sanity_random_win} and mostly lies in the low pruning ratio regime~\cite{alizadeh2022prospect}.
As systematically studied in~\cite{ma2021sanity, frankle2020pruning}, there exists a clear performance gap between one-shot pruning and IMP.}
%However, current one-shot methods often incur evident performance degradation, and could fail to find winning tickets\,\cite{ma2021sanity}.
%
% \fakepara{current optimization-based pruning methods save time but are weak. is fundamental improvement possible?}
As an alternative to heuristics-based schemes, optimization-based pruning methods~\cite{ren2018admmnn, ramanujan2020sHiddenSubnetwork,sehwag2020hydra, lee2020layer, csordas2020neural} still follow the pruning-retraining paradigm and adopt sparsity regularization\,\cite{liu2019admm, wang2020neural}  or parameterized masking\,\cite{ramanujan2020sHiddenSubnetwork, sehwag2020hydra, csordas2020neural} to prune models efficiently. However, these 
% optimization-based pruning 
methods do not always
%are unable to 
match the accuracy of IMP and  thus have not been widely used to find winning tickets\,
\cite{frankle2018lottery, lee2018snip, wang2020pick,tanaka2020pruning, alizadeh2022prospect, zhang2021efficient}.
{The empirical results showing that optimization underperforms heuristics} 
motivate us to revisit the algorithmic fundamentals of this research: Can we reformulate optimization-based pruning to match and improve over IMP in terms of model accuracy? 
%

\begin{wrapfigure}{r}{60mm}
\vspace*{-6mm}
\centerline{
\includegraphics[width=58mm]{figure/main_compare.pdf}
}
\vspace*{-4mm}
\caption{\footnotesize{
A performance snapshot of the proposed {\biprune} method vs. the IMP baseline and the original dense model across three pruned ResNet models (ResNet-20, ResNet-56, and ResNet-18) with 74\% sparsity on CIFAR-10. The marker size indicates the relative model size. The uni-color region corresponds to the same model type used by different pruning methods.
% of test accuracy of pruned models (with 74\% sparsity) and 
% CIFAR-10 test accuracy and training time of three different network architectures by {\biprune} and IMP at the sparsity ratio of 74\%.
% % compared to dense models. 
% The size of markers indicates model parameter counts.
}}
\label{fig: intro-c2}
\vspace*{-5mm}
\end{wrapfigure}
To this end, we put forth a novel perspective of model pruning as a bi-level optimization (BLO) problem. In this new formulation, we show that BLO provides a technically-grounded optimization basis for an efficient implementation of the pruning-retraining paradigm, the key algorithmic component used in IMP. 
%
To the best of our knowledge, we make the first rigorous connection between model pruning and BLO. Technically, we propose a novel \textbf{bi}-level optimization-enabled \textbf{p}runing method (termed {\biprune}).  We further show how {\biprune} takes advantage of the bi-linearity of the pruning problem to avoid the computational challenges of common BLO methods, and is as  efficient as any first-order alternating optimization scheme. Practically, we demonstrate the superiority of the proposed {\biprune} in terms of accuracy, sparsity, and  computation efficiency through extensive experiments. {\biprune} finds the best winning tickets nearly in all settings while taking time comparable to the one-shot OMP. In Fig.\,\ref{fig: intro-c2}, we present a snapshot of our empirical results for CIFAR-10 with 3 ResNet architectures at 74\% pruning ratio. In all cases, {\biprune}
% in 
(\textcolor{red}
{$\star$}) finds winning tickets, improving accuracy over the dense model (\textcolor{ForestGreen}{ $\bullet$}) and matching IMP (\textcolor{orange}{$\blacktriangle$}), while being upto 5$\times$ faster than IMP.


Our \textbf{contributions} can be summarized as follows:
%\todo{Maybe need to say why ``flexibility'' is helpful\\
%\YY{I am not sure how to elaborate on this. I added "mimic the meta learning" to state the meaning of choosing various objectives of different levels. But I am not sure whether such explanation is straight-forward.}\\
%PR: not sure it helps -- we suddenly mention meta-learning while focusing on pruning. need to think a bit more
%}

\noindent $\bullet$ (Formulation) We rethink the algorithmic foundation of model pruning through the lens of BLO (bi-level optimization). The new BLO-oriented formulation 
%advances the optimization foundation for the pruning problem, and
%provides
provides an optimization basis of  
%a natural justification for 
the widely-accepted pruning-retraining paradigm. Moreover, %the new formulation 
the formulation disentangles
 pruning and retraining variables, providing the flexibility to design the interface between pruning and retraining.
% use different objectives at different levels of the BLO, \emph{i.e.}, mimic the design of meta-learning. 

\noindent $\bullet$ (Algorithm) We propose the new bi-level pruning ({\biprune}) algorithm, which is built upon the aforementioned BLO formulation and the implicit gradient-based optimization theory. Unlike computationally intensive standard BLO solvers, we theoretically show that {\biprune} is as efficient as any first-order optimization by taking advantage of the bi-linear nature of the pruning variables. 
% We propose the bi-level pruning (BiP) algorithm and prove that the implicit gradient (IG) term brought by the bi-level formulation can be solved with only first-order derivatives. The bi-linearity of the pruning problem optimizes allows simplification of the IG computation, accelerating the execution of {\biprune}.  

\noindent $\bullet$ (Experiments) We conduct extensive experiments across 4 datasets (CIFAR-10/100, Tiny-ImageNet and ImageNet), 5 model architectures, and 2 pruning settings (unstructured and structured pruning). We show that {\biprune} enjoys the high accuracy of IMP and the high efficiency of the one-shot pruning schemes. 
Specifically, we show that (i)~{\biprune} achieves higher test accuracy than IMP and finds the best winning tickets nearly in all settings, and (ii)~{\biprune} is highly efficient (comparable to one-shot pruning schemes), achieving 2-7$\times$ speedup over IMP for the same level of model accuracy and sparsity. 
% \SL{[I removed the third point.]}

% and (iii)~{\biprune} is insensitive to specialized hyper-parameter choices, thus introduces no burden of BLO.
% \todo{do we want to say anything about insensitivity to specialized hyper-parameters or rewinding?\\ \YY{I agree. I try to highlight that BLO does not introduce new burden of the practical optimization.}\\ PR:insensitive is too strong since we depend a lot of $\gamma$ upto a point. I think the robustness to (i)~rewinding (critical HP in pruning literature) and (ii)~number of inner-loop steps (critical HP in BLO) is useful but we need to think about how we say it.  }

% We conduct extensive experiments to validate our method {\biprune} on diverse datasets (\emph{i.e.,} CIFAR-10/100, Tiny-ImageNet, and ImageNet) across multiple network architectures, including various ResNets and VGG. Specifically, our unstructural winning tickets achieve up to 2\% improvement over the unpruned dense models and 3-7$\times$ speedup compared to IMP for the same level of model accuracy and sparsity.



==> Deprecated_NO_USE/Version_Camera_08041600_Submission/Sec3_SL.tex <==
In this section, we begin by providing a brief   background of neural  network pruning, including the predominant   iterative magnitude pruning (IMP) method and the 
associated lottery ticket hypothesis (LTH)
\cite{frankle2018lottery} to find high-quality subnetworks (known as `winning tickets') that--when trained in isolation--reach test accuracy comparable to or even better than the original dense network. 
However, the superior performance of IMP is accompanied by a prohibitive computation cost, as will be exemplified in Fig.\,\ref{fig: one_shot_results}. In  order to overcome the computational difficulty of IMP, we next introduce the  one-shot pruning method and elaborate on its comparison with IMP. Spurred by the pros and cons of current pruning methods, we eventually state the problem to be studied in this paper. 
 

\paragraph{{Heuristics-based IMP.}}
The heuristics-based IMP is the  currently prevailing approach  to
identify the `winning ticket' in model pruning, so as to attain model sparsity without suffering  performance loss\,\cite{blalock2020state,frankle2018lottery,Renda2020Comparing,frankle2020linear,chen2020lottery,chen2021lottery}. 
For example, the current  state-of-the-art (SOTA) implementation of IMP in \cite{ma2021sanity} can lead to a pruned ResNet-20 on
% \SL{[This example  number needs to be   better aligned with the later figure, then you can cite it here.]}
CIFAR-10 with 74\% sparsity and $92.12\%$ test accuracy, {
which is comparable to the performance of the original dense model}; see Fig.\,\ref{fig: one_shot_results}. 
% For the larger-size {ResNet-18} model, IMP   can identify a sparser network with   {$95\%$ sparsity and $94.81\%$ test accuracy, yielding the $0.5\%$ improvement over the original dense model}; \SL{see Fig.\,xxx in Sec.\,xxx}.
The algorithm of IMP typically contains two key ingredients: \textbf{(i)} a \textit{temporally-evolved pruning schedule} (given by the growing model sparsity over pruning iterations), and \textbf{(ii)} the \textit{pruning-retraining learning mechanism} applied at each pruning round. 
% To be more specific, 
% IMP  repeatedly trains, prunes, and resets the network over multiple rounds (say $n$ rounds). 
For (i), supposing that there exist $n$ pruning rounds, each round  prunes $(p\%)^{\frac{1}{n}} $ of the model
weights that survive the previous round, where $p\%$ denotes the final pruning ratio to be achieved.
%This leads to a pruning mask $\mathbf m$ at each round. 
For (ii), 
the non-zero remaining weights at each pruning round are re-set to the  weights at initialization or at an early-training epoch \cite{Renda2020Comparing}, and   re-trained till convergence. 
In brief, IMP  repeatedly trains, prunes, and resets the network over multiple rounds. 

 

% A common example, the Lottery Ticket Hypothesis (LTH), can achieve comparable or even better performance with a sparsity of over $95\%$ in its state-of-the-art (SOTA) implementation\,\cite{ma2021SanityCheckLTH}. 
% In general, the heuristics-based IMP adopts a sparsifying-retraining paradigm which consists of multiple iterative cycles: \underline{\textit{(1)}} \textbf{training} dense model with several epochs; \underline{\textit{(2)}} \textbf{pruning} $p\%$ redundant model weights with certain heuristics-based criteria (\emph{e.g.} model weight magnitude) to obtain the new mask; \underline{\textit{(3)}} \textbf{fine-tuning} the sparse network with the found mask and rewound weights for accuracy recovery. 

\begin{wrapfigure}{r}{85mm}
\vspace*{-5mm}
\centerline{
\begin{tabular}{cc}
\hspace*{0mm}\includegraphics[width=.3\textwidth,height=!]{figure/performance_comparison.pdf}  
&\hspace*{-4mm}\includegraphics[width=.31\textwidth,height=!]{figure/time_comparison_long.pdf}
% \\
% \hspace*{2mm}\footnotesize{(a) Test accuracy vs. pruning ratio.} &   \footnotesize{(b) Runtime of pruning.}
\end{tabular}}
\vspace*{-2mm}
\caption{\footnotesize{
Illustration of the pros and cons of different pruning methods executed over (ResNet-20, CIFAR-10).
(a) Test accuracy vs. different pruning ratios: IMP significantly outperforms one-shot pruning methods (\textsc{OMP}\,\cite{frankle2018lottery}, \textsc{ProsPr}\,\cite{alizadeh2022prospect}, \textsc{Grasp}\,\cite{wang2020pick}, \textsc{Snip}\,\cite{lee2018snip}, \textsc{SynFlow}\,\cite{tanaka2020pruning}). (b) Computation time of pruning to different sparsity levels:  IMP becomes much more computational intensive when pruning is targeted for a higher sparsity level. 
%We highlight we adopt the SOTA implementation of OMP  following\,\cite{ma2021sanity} and other methods following their original settings.
% \SL{For (a): Update x-y axis and mark the $95\%$ or $99\%$ pruning point.}
% \SL{For (b): [X-axis: Pruning method, add the dense model training time.]}
% \SL{Illustration of  the pros and cons of different pruning methods executed over (ResNet-xxx, CIFAR-10).
% (a) Test accuracy against pruning ratio: IMP significantly outperforms one-shot pruning methods (OMP [refs], ....). (b) Computation time of pruning to different sparsity levels:  IMP becomes much more computational intensive when pruning is targeted for a higher sparsity level ($99\%$ vs. $60\%$).
% }
% Performance and efficiency comparison between IMP (LTH) and various one-shot pruning methods on CIFAR10 and ResNet20. One-shot methods save pruning time at the cost of significant performance drop compared to IMP (LTH).
% \SL{Why ResNet20? Not ResNet18?}
}}
  \label{fig: one_shot_results}
  \vspace*{-7mm}
\end{wrapfigure}

%\SL{[I stop here]}
Yet, the superior pruning accuracy   of IMP is at the cost of  computation efficiency. For ease of illustration, Fig.\,\ref{fig: one_shot_results} shows the example of pruning ResNet-20 over CIFAR-10 and demonstrates   the accuracy and the computation time of various pruning methods versus the growing sparsity ratio.
%and (b) the computation time of model pruning with different sparsity levels.
% \SL{For ease of illustration, Fig.\,\ref{fig: one_shot_results} shows a pruning example that unveils (a) the accuracy performance of various pruning methods versus the growing sparsity ratio, and (b) the computation time of model pruning with different sparsity levels.}
As we can see, IMP outperforms   the other pruning baselines and finds 
the sparsest winning ticket (marked by the red star in Fig.\,\ref{fig: one_shot_results}a) using $n = 6$ pruning rounds. 
However, this leads to $3\times$ more than the cost of training a dense model from scratch.
% \SL{the $95\%$-sparsity ResNet-18 model with $94.81\%$ test accuracy on CIFAR-10 takes $n = xxx$ pruning rounds. This leads to $xxx$-min runtime, which is $xxx$ times higher than training a dense model and $xxx$ times higher than pruning to the $60\%$  sparsity level.} 
%and thus hampers the pruning efficiency 
%
\iffalse
Although IMP-based pruning approaches have become the rising star sub-field in pruning, its current success largely sacrifices the pruning efficiency. Within each pruning cycle, the sparse structure is obtained by removing a small fixed pruning ratio (\emph{e.g.}, $20\%$ in LTH) of the \textbf{remaining weights} to make the final sparse model match the full performance of the dense model. Thus, the required pruning iterative numbers as well as their training time grow exponentially as the sparsity increases. For example, the SOTA implementation of LTH\,\cite{ma2021SanityCheckLTH} has to go through 22 pruning cycles to arrive at a sparsity of $99\%$. In such a case, the immense training time consumption has become one clear obstacle of IMP from scaling to large model architectures and datasets\,\cite{zhang2021efficient}.
\fi 
%
\paragraph{IMP vs. one-shot pruning.}
To reduce the computation cost of IMP, different kinds of `accelerated' pruning methods were developed \cite{frankle2018lottery,lee2018snip, wang2020pick,tanaka2020pruning, alizadeh2022prospect, zhang2021efficient}; And many of them
  fall into the \textit{one-shot pruning} category: The network is directly pruned to the eventual target sparsity level  and retrained once. 
%: the network is trained once, p% of weights are pruned, and the surviving weights are reset.
% which refines the sparse mask directly to the given sparsity only one time. 
In particular, the one-shot magnitude pruning (OMP) has served as an important baseline that  simplifies IMP directly \cite{frankle2018lottery}.
\textsc{OMP} obeys the pruning-retraining paradigm, but it  prunes the model to the target sparsity using only one pruning round. 
% \SL{Although some existing work\,\cite{ma2021SanityCheckLTH} observed that OMP and the other one-shot pruning methods (e.g., ProsPr\,\cite{alizadeh2022prospect}) could find winning tickets and achieve similar accuracy performance to IMP. However, this conclusion is model/dataset-specific. }
% Although some preliminary results showed that 
% existing work\,\cite{ma2021sanity}(\YH{cite TBD}) observed that OMP and the other one-shot pruning methods (e.g., \textsc{ProsPr}\,\cite{alizadeh2022prospect}) could find winning tickets and achieve similar accuracy performance to IMP at low sparsity levels. However, this conclusion is model/dataset-specific. 
However,  the promise of current one-shot pruning methods is dataset/model-specific \cite{ma2021sanity, su2020sanity_random_win} and mostly lie in the low-sparsity regime \cite{alizadeh2022prospect}.
As systematically studied in \cite{ma2021sanity, frankle2020pruning}, there exists a clear performance gap between one-shot pruning and IMP.
Fig.\,\ref{fig: one_shot_results} also justifies the above limitation.
% However, the degradation in accuracy of the one-shot methods is still significant compared to IMP (LTH), making them impractical to real world applications\,\cite{frankle2020pruning}.
As we can see, although one-shot pruning  is   computationally light (Fig.\,\ref{fig: one_shot_results}b), it suffers from an evident accuracy drop compared to IMP (Fig.\,\ref{fig: one_shot_results}a), especially at the large sparsity levels.
%For example, \textsc{OMP} and \textsc{ProsPr} \cite{alizadeh2022prospect}, the SOTA methods of one-shot pruning,   yield  over $2\%$ and $10\%$ accuracy drop compared to IMP at the $74\%$ and  $98\%$ sparsity level, respectively.
Thus,  there exists a strong demand for the algorithmic advancement of model pruning that can   enjoy the dual advantages of one-shot pruning and IMP.
%\textit{i.e.}, improve the tradeoff  between computation efficiency and pruning accuracy. 
% Even the SOTA one-shot pruning method \textsc{ProsPr}\,\cite{alizadeh2022prospect} also suffers from an accuracy drop of over $10\%$ compared to IMP when $99\%$ parameters are pruned.
% As demonstrated in Figure\,, all one-shot  
%\todo{I don't see 99\% sparsity level in Figure~\ref{fig: one_shot_results}. Do we mean 90\%?
%
%\YY{Solved.}}
%
%the observed accuracy-efficiency tradeoff
%the accuracy-efficiency tradeoff of one-shot pruning is based on the heuristics-based one-shot pruning 
%This efficiency-performance trade-off is primarily due to the heuristic nature, which is insufficient to find satisfactory masks with an extreme sparsity using the radical pruning ratio as OMP does.
%
\paragraph{Problem Statement.}
As described above, the existing  one-shot pruning methods do not suffice to close the performance gap with IMP. One possible root cause is its strong   dependence   on  the heuristics-based weight sparsification strategy. This leaves the question of  whether 
computation efficiency and pruning accuracy could be co-improved through a more rigorous and dedicated optimization-based approach. 
% a theoretically-grounded optimization-based approach can renovate one-shot pruning so as to improve the computation complexity of pruning while attaining the accuracy performance comparable to IMP.
% Based on the aforementioned dilemma between performance and pruning cycle number in heuristics-based pruning methods, we ask the following question:
Thus, we ask:  \textit{Beyond heuristics, how to establish the \textbf{optimization basis} of a successful pruning mechanism that can attain high pruning  accuracy (like IMP) as well as high   computation efficiency (like one-shot pruning)?}
% \begin{center}
%     \textit{Beyond heuristics, how to establish the \textbf{optimization basis} of a successful pruning mechanism that can close the gap between pruning accuracy (e.g., achieved by IMP) and computation efficiency (e.g., achieved by OMP)?}
% \end{center}


%\newpage 


==> Deprecated_NO_USE/Version_Camera_08041600_Submission/Sec4_SL.tex <==
In this section, we re-investigate the problem of model pruning through the lens of  BLO and develop the bi-level pruning (\biprune) algorithm.
%and show that BLO  not only provides a natural interpretation of the pruning-retraining learning paradigm but also brings in additional   design flexibilities for model pruning.
%Next, we 
%We establish  its algorithmic foundation of BLO-enabled model pruning (termed bi-level pruning or {\biprune}), extended from  the implicit gradient approach. Further, 
We  can theoretically    show that {\biprune} %is a special class of BLO problems and 
can be solved as easily as the first-order alternating optimization by taking advantage of the bi-linearity of pruning variables.
%Lastly, we summarize the   {\biprune} algorithm and its   implementation details.  

% We will show the benefits as well as the mathematical challenges brought by the BLO formulation. Next, we point out that the bi-linearity of the pruning problem falls into a special class of the BLO and thus, can be solved as easily as the first-order alternating optimization. Finally, we propose {\biprune}, an efficient first-order BLO-based model weight pruning algorithm.
\vspace*{-3mm}
\paragraph{A BLO viewpoint on model pruning}
As described in the previous section, the pruning-retraining learning paradigm covers two kinds of tasks: \ding{182} pruning  that determines the sparse pattern of model weights, and \ding{183} training remaining non-zero weights  to recover the model accuracy. 
In existing optimization-based pruning methods \cite{wen2016learning,zhang2018systematic,hoefler2021sparsity,wang2020proximal}, the tasks \ding{182}-\ding{183} are  typically achieved by optimizing model weights,   together with penalizing their sparsity-inducing norms, \textit{e.g.}, the $\ell_1$  and $\ell_2$ norms \cite{bach2012optimization}. Different from the above formulation, we propose to  separate optimization variables involved in the pruning tasks  \ding{182} and \ding{183}. This leads to the (binary) pruning mask variable $\mask \in \{ 0, 1\}^n$
and the model weight variable $\btheta \in \mathbb R^n$. Here $n$ denotes the total number of model parameters. 
Accordingly, the pruned model is given by $(\mathbf m \odot  \btheta)$, where $\odot$ denotes the element-wise multiplication. As will be evident later, this form of \textit{variable disentanglement} enables us to 
explicitly depict how the pruning and retraining process co-evolve, and helps customize  the pruning task with high flexibility.
%so as to leverage more advanced optimization techniques to achieve a better pruning solution than heuristics-based search. 



% the model mask\,$\mask$ and the corresponding model weights\,$\btheta$. In the widely accepted sparsifying-retraining pruning paradigm, the masks $\mask$ are highly dependent on the model weights $\btheta$ as the magnitude of $\btheta$ serves as the pruning criterion. In the BLO formulation, $\mask$ and $\btheta$ are optimized independently using disparate variables. This \textit{disentanglement} gives the mask variables $\mask$ more flexibility to search better optima than the heuristics-based methods. More importantly, it facilitates us to interpret the sparsifying-retraining paradigm from a bi-level optimization viewpoint. 



We next elaborate on how BLO can be established to co-optimize the pruning mask $\mathbf m$  and the retrained sparse model weights $\boldsymbol \theta$. 
%Let $\ell$ denote the training loss and .
%Let $k$ denote the targeted sparsity number, determined by the pruning ratio $p = k/d$. 
Given the pruning ratio $p\%$, the sparsity constraint   is given by $\mathbf m \in  \mathcal{S} $, where $\mathcal S = \{ \mathbf m\,|\, \mathbf m \in \{ 0, 1\}^n, \mathbf  1^T \mathbf m \leq k \}$ and $k = (1-p\%) n$.
Our goal is to  prune the original  model \textit{directly} to the targeted pruning ratio $p\%$ (\textit{i.e.}, without calling for the IMP-like sparsity schedule as described in Sec.\,\ref{sec: preliminary}) and obtain the optimized sparse model $(\mathbf m \odot \btheta)$. To this end, we interpret the pruning task (\textit{i.e.}, \ding{182}) and the model retraining task (\textit{i.e.}, \ding{183}) as \textit{two optimization levels}, where the former is formulated as an \textit{upper-level} optimization problem, and it relies  on the optimization of the \textit{lower-level}  retraining task. We thus cast the model pruning problem as the following BLO problem (with \ding{183} being nested inside \ding{182}):
%\todo{Mention structured pruning? For structured pruning, manipulate m with Kronecker and transfer the element-wise pruning unit to a structured one.
% \YY{In actual implementation, we use individual m for each $\theta$, but with specific structural patterns. I agree with Pari that we can mention such manipulation.}
%}%


{\small{
\vspace*{-6mm}
\begin{align}
% \vspace*{-3mm}
\displaystyle
    \begin{array}{llll}
\displaystyle \minimize_{\mathbf \mask \in \mathcal{S}}         & \underbrace{\ell(\mask \odot {\btheta}^*(\mask))}_\text{ \ding{182}: Pruning task}; 
& \quad 
  \st &  \underbrace{\displaystyle {\btheta}^*(\mask) = \argmin_{\btheta \in \mathbb{R}^n} \overbrace{ \ell(\mask\odot \btheta) + \frac{\gamma}{2} \|\btheta\|_2^2}^\text{$\Def g(\mask, \btheta)$}}_\text{\ding{183}: Sparsity-fixed model retraining},
    \end{array}
    \label{eq: prob_bi_level}
    \vspace*{-4mm}
\end{align}
}}%
where $\ell$ denotes the training loss (\textit{e.g.}, cross-entropy), 
$\mathbf m$ and $\btheta$ are the upper-level and lower-level optimization variables respectively, 
${\btheta}^*(\mask)$ signifies the lower-level solution obtained by minimizing the objective function $g$ given the pruning mask $\mask$, 
and $\gamma > 0$ is a regularization parameter introduced to convexify the lower-level optimization so as to stabilize the gradient flow from   $\btheta^*(\mathbf m)$ to $\mathbf m$ and thus the convergence of BLO \cite{hong2020two, shaham2015understanding}.
%As will be evident later, the introduction of $\lambda$
In a sharp contrast to existing single-level optimization-based model pruning methods \cite{wen2016learning,zhang2018systematic,hoefler2021sparsity,wang2020proximal}, the BLO formulation \eqref{eq: prob_bi_level} brings in  \underline{two advantages}. 

\underline{First}, BLO has the flexibility to use   {mismatched} pruning and retraining objectives at the upper and lower optimization levels, respectively. 
% {\color{red}[but in (1) we did not have the mismatch? shall we be specific as to which functions are different?]} 
% \YH{We do have mismatch as $\ell$ and $g$ are different.} 
{This flexibility allows us to regularize the lower-level training objective function  in \eqref{eq: prob_bi_level}  and customize the implemented optimization methods at both levels.}
% This flexibility allows us to customize not only the regularized lower-level   objective function in \eqref{eq: prob_bi_level}
% but also the optimization algorithm per level. 
To be more specific, one can  update the upper-level pruning mask $\mask$ using a data batch (called $\mathcal B_2$) distinct from the one (called $\mathcal B_1$) used for  obtaining the lower-level solution ${\btheta}^*(\mask)$. The resulting BLO procedure can then mimic the idea of  meta learning to improve model generalization \cite{deng2021meta}, where the lower-level problem fine-tunes $\btheta$ using $\mathcal B_1$, and the upper-level problem validates the generalization of the sparsity-aware finetuned model $(\mathbf m \odot \boldsymbol \theta^* (\mathbf m))$ using $\mathcal B_2$.
%By doing so, the idea of meta learning (to improve model generalization)  can be infused into  model   


\underline{Second}, BLO enables us to explicitly model and optimize the coupling  between the retrained model weights $\btheta^*(\mathbf m)$ and the pruning mask $\mathbf m$ through the implicit gradient (IG)-based optimization routine. Here IG refers to  the gradient of the lower-level solution $\btheta^*(\mathbf m)$ with respect to (w.r.t.) the upper-level variable $\mathbf m$, and its derivation  calls the implicit function theory \cite{gould2016differentiating}.
The use of     IG makes our proposed BLO-oriented pruning \eqref{eq: prob_bi_level} significantly different from the greedy alternating minimization  \cite{csiszar1984information} that learns the upper-level and lower-level variables independently (\textit{i.e.}, minimizes one variable by fixing the other). We refer readers to the following section for the detailed IG theory.
 We will also show in Sec.\,\ref{sec: exp} that
 the pruning strategy from \eqref{eq: prob_bi_level} can outperform IMP in many pruning scenarios but is much more efficient as it does not call for the scheduler of iterative pruning ratios. 
 
% A sparse model (\emph{a.k.a.} a pruned model) is defined as $f(\mask \odot \btheta)$, namely the element-wise product of a dense network $f(\btheta, \cdot)$ and a binary mask $\mathbf m$. The pruning mask $\mask \in {\{0, 1\}}^d$ has the same shape as the model parameter $\btheta$ and localizes the non-zero weights with a certain sparsity ratio $p$, where $d={\|\btheta\|_0}$ demotes the dimension of the model parameter. 
% A pruning algorithm aims to find the sub-network of the given model architecture with a certain sparse level while maintaining the performance of the pruned model at a high level. 
% The pruning problem can be readily reformulated to a hierarchical optimization problem, where the model parameter $\mask$ and the mask $\btheta$ are jointly optimized. This nested structure presents a standard bi-level optimization (BLO) formulation, which is given by% 
% {
% \small
% \begin{align}
% % \vspace*{-3mm}
% \displaystyle
%     \begin{array}{ll}
% \displaystyle \minimize_{\mathbf \mask\in \mathbb \{0, 1\}^{d}}         & f(\mask, {\btheta}^*(\mask)) 
% \\
%   \st &  \displaystyle {\btheta}^*(\mask) = \argmin_{\btheta \in \mathbb{R}^d}  g(\mask, \btheta) + \frac{\gamma}{2} \|\btheta\|_2^2,
%     \end{array}
%     \label{eq: prob_bi_level}
% \end{align}
% }%

% where $f$ and $g$ denote the upper-level and the lower-level objective functions, and $\gamma > 0$ is a quadratic regularization parameter. 
% In the BLO formulation, the upper-level problem aims to find the pruning mask based on the given model parameter $\btheta$, while the lower-level problem retrains the model parameter with the fixed sparse mask. 
% The reasons for introducing the quadratic regularization term $\frac{\gamma}{2} \|\btheta\|_2^2$ are two-fold. First, it stabilizes the lower level problem via regularization. Second, it enforces the strong convexity of the lower-level problem. A different regularizer might be adopted in different use cases. 
% % For example, in implicit MAML\,\cite{rajeswaran2019meta} used $\| \mathbf y - \mathbf x\|_2^2$ as the regularizer. 
% For example, implicit MAML\,\cite{rajeswaran2019meta} used the $\ell_2$ regularizer to stablize the parameter update. 
% Such a strongly convex regularization term is also common in the BLO analysis \cite{shaham2015understanding} to stabilize the alternative optimization convergence of BLO.

% The BLO interpretation of model pruning provides multiple advantages in contrast to the conventional sparsity promoting optimization based methods ($\btheta$-only):

% \ding{172} Formulation-wise: the nested structure of \eqref{eq: prob_bi_level} allows for \emph{different} objective functions in different levels. This flexibility further enables us to use mismatched data batches for mask finding and model training, which has been verified to be very beneficial for improving the model generalization\,\cite{deng2021meta}.

% \ding{173} Optimization-wise: the BLO formulation is uniquely suited for characterizing structure of the pruning-retraining paradigm. Different from the single-level optimization problem, BLO will use a specialized optimization routine.

% \ding{174} Compared to IMP, BLO directly optimizes the mask $\mask$ to any given sparsity in one sole pruning cycle. There is no need to adopt a small pruning ratio and achieve the large sparsity in multiple pruning cycles. This characteristic resembles one-shot pruning methods and accounts for the \textit{sparsity-agnostic} computational costs of the BLO-based pruning method.
\vspace*{-0.1in}
\paragraph{Optimization foundation of {\biprune}.}
The key optimization challenge of solving the {\biprune} problem \eqref{eq: prob_bi_level} lies in the computation of IG (implicit gradient). Prior to developing an effective solution, we first elaborate on the \textit{IG  challenge}, the unique characteristic of BLO. In the context of gradient descent, the gradient of the   objective function in  \eqref{eq: prob_bi_level} yields

\vspace*{-5mm}
{
\small{
\begin{align}
\displaystyle
    \underbrace{\frac{d\ell(\mask \odot \btheta^*(\mask))}{d\mask}}_\text{Gradient of objective} = \nabla_{\mask} \ell(\mask \odot {\btheta}^*(\mask)) + \underbrace{
    \frac{{d ( {\btheta}^*(\mask)^{\top} )
    }
    %^{\top}
    }{d \mask}}_{\text{{IG}}} \nabla_{\btheta}\ell (\mask \odot \btheta^*(\mask)),
    \label{eq: GD_bi_level}
\end{align}}}%
where $\nabla_{\mask}$ and $\nabla_{\btheta}$  denote the \textit{partial derivatives} of the bi-variate function $\ell(\mask \odot \btheta)$  w.r.t. the variable $\mask$ and $\btheta$ respectively, 
$d \btheta^\top / d \mask  \in \mathbb R^{n \times n} $ denotes the vector-wise \textit{full derivative},  
and for ease of notation, we will omit
the transpose $\top$ when the context is clear.
In \eqref{eq: GD_bi_level}, the IG challenge refers to the demand for   computing the full gradient of  the implicit function $\btheta^*(\mask) = \argmin_{\btheta} g(\mask, \btheta)$ w.r.t. $\mask$, where recall from \eqref{eq: prob_bi_level}  that $ g(\mask, \btheta) \Def  \ell(\mask\odot \btheta) + \frac{\gamma}{2} \|\btheta\|_2^2 $.
\iffalse
To circumvent this difficulty, the conventional method is  \textit{gradient unrolling} that   approximates the lower-level solution $\btheta^*(\mask)$ using a single or a few unrolled gradient descent steps, \textit{e.g.}, 
$\btheta^*(\mask) \approx \btheta - \alpha \nabla_{\btheta} g(\mask, \btheta)$. However, this only gives a rough estimate of the lower-level solution and  lacks theoretical rigorousness \cite{hong2020two}. Meanwhile, even in this over-simplified scenario, it is not difficult to see that the computation of   IG
%, \textit{i.e.}, $ \frac{{d {\btheta}^*(\mask)}^{\top}}{d \mask}$,  
relies on the computation of second-order partial derivatives.
\fi 

%Different from gradient unrolling,
Next,
we derive the IG formula following the %more 
rigorous 
implicit function theory \cite{gould2016differentiating,hong2020two,rajeswaran2019meta}.
%, where the stationary condition of the lower-level optimization in \eqref{eq: GD_bi_level} is treated as  a differentiable explicit   function
Based on the fact that $\btheta^*(\mask)$ satisfies the stationarity condition for the lower-level objective function in \eqref{eq: GD_bi_level},  it is not difficult to obtain that  (see derivation in  Appendix\,\ref{eq: app_IG})

\vspace*{-5mm}
{\small
\begin{align}
% & \displaystyle
%     %{\frac{d\btheta^*(\mask)}{d\mask}}^{\top} (\nabla_{\btheta \btheta} g(\mask, \btheta) + \gamma \mathbf{I}) + \nabla_{\mask\btheta} g(\mask, \btheta)%
%     \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) + \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%     \nabla^2_{\btheta} \ell(\mask \odot \btheta^*)
%   + \gamma \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%   = \mathbf 0; \nonumber \\
%  \Longrightarrow  &
\displaystyle  \frac{d\btheta^*(\mask)}{d\mask} %^{\top} 
 =  -   \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) [ \nabla^2_{\btheta } \ell(\mask \odot \btheta^*) + \gamma \mathbf I ]^{-1},
 \label{eq: exact_IG}
\end{align}
}%
where   $\nabla_{\mask \btheta}^2 \ell $ and $\nabla_{\btheta}^2 \ell $ denote the second-order partial derivatives of $\ell$ respectively, and $(\cdot)^{-1}$ denotes the matrix inversion operation. 
%We refer readers to Appendix\,\ref{eq: app_IG} for the full derivation of \eqref{eq: exact_IG}.


% we   obtain 

% \vspace*{-6mm}
% {
% \small
% \begin{align}
% \displaystyle
%   %  \frac{d g(\mask, \btheta^*(m)))}{
%   %  d\btheta}
%   \nabla_{\btheta} g(\mathbf m, \btheta^* )
%     = \nabla_{\btheta} \ell(\mask \odot \btheta^* ) + \gamma \btheta^*  = \mathbf 0.
%     \label{eq: stationary}
% \end{align}
% }%
% where for ease of notation, we omit the dependence of $\btheta^*(\mask)$ w.r.t. $\mathbf m$.
% We   then take    derivative of the second equality of \eqref{eq: stationary} w.r.t. $\mask$ by using the implicit 
% function theory. This leads to \todo{\YH{Put Eq. 3-4 in the appendix or merge them into one proof? }}
% % $
% % {\frac{d\btheta^*(\mask)}{d\mask}}^{\top} (\nabla_{\btheta \btheta} g(\mask, \btheta) + \gamma \mathbf{I}) + \nabla_{\mask\btheta} g(\mask, \btheta) = \mathbf  0
% % $

% \vspace*{-5mm}
% {\small
% \begin{align}
% & \displaystyle
%     %{\frac{d\btheta^*(\mask)}{d\mask}}^{\top} (\nabla_{\btheta \btheta} g(\mask, \btheta) + \gamma \mathbf{I}) + \nabla_{\mask\btheta} g(\mask, \btheta)%
%     \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) + \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%     \nabla^2_{\btheta} \ell(\mask \odot \btheta^*)
%   + \gamma \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
%   = \mathbf 0; \nonumber \\
%  \Longrightarrow  &
%  \frac{d\btheta^*(\mask)}{d\mask} %^{\top} 
%  =  -   \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ) [ \nabla^2_{\btheta } \ell(\mask \odot \btheta^*) + \gamma \mathbf I ]^{-1}.
%  \label{eq: exact_IG}
% \end{align}
% }%
% where $\nabla_{\mask \btheta} \ell $ and $\nabla_{\btheta \btheta} \ell $ are the second-order partial derivatives of the bivariate function $\ell$, and $(\cdot)^{-1}$ denotes the matrix inversion operation.

Yet, the exact   IG formula \eqref{eq: exact_IG} remains difficult to calculate due to the presence of matrix inversion and second-order partial derivatives.
% \todo{$\gamma$ is critical in this derivation. Without $\gamma$, and with the $\nabla^2_{\btheta} = 0$ assumption, this does not go through. How do we best motivate the introduction of $\gamma$ in (1) since standard pruning setups and schemes dont introduce such regularization term?}
To  simplify it, 
we impose the Hessian-free assumption, 
$ \nabla^2_{\btheta} \ell = \mathbf 0$, which  is mild in general; For example,   the decision boundaries of neural networks with ReLU activations are piece-wise linear in  a tropical hyper-surface \cite{alfarra2020decision}, and this assumption 
%is   necessary as  computing the Hessian matrix w.r.t.   model parameters $\btheta$ would be practically infeasible, and it
has been widely used in BLO-involved applications such as meta learning \cite{finn2017model} and adversarial learning \cite{zhang2021bat}. Given $ \nabla^2_{\btheta } \ell = \mathbf 0$,  the matrix inversion in \eqref{eq: exact_IG} can   be then mitigated, leading to the IG formula

\vspace*{-5mm}
{\small
\begin{align}
    \frac{d\btheta^*(\mask)}{d\mask} %^{\top}
    =  -  \frac{1}{\gamma} \nabla^2_{\mask \btheta} \ell (\mask \odot \btheta^* ).
    \label{eq: IG_simplify}
\end{align}
\vspace*{-3mm}
}%

At the first glance, the computation of the simplified IG   \eqref{eq: IG_simplify} still requires the mixed (second-order) partial derivative $\nabla^2_{\mask \btheta} \ell$. However, {\biprune} is a special class of BLO problems with bi-linear variables 
$(\mask \odot \btheta)$. Based on this bi-linearity, we can prove that  IG  in \eqref{eq: IG_simplify} can be \textit{analytically} expressed using only \textit{first-order} derivatives; see the following theorem. 

% \begin{tcolorbox}[colback=black!5!white,colframe=white!20!black]
\begin{myprop}
\label{thr: ig}
Assuming $\nabla^2_{ \btheta} \ell = 0$ and defining {$\gradzsimple \Def \gradz$}, the implicit gradient \eqref{eq: IG_simplify} is then given by

\vspace*{-5mm}
{\small
\begin{align}
\displaystyle
\frac{d\btheta^*(\mask)}{d\mask} %^{\top} 
% =  -  \frac{1}{\gamma} \nabla_{{\mask} {\btheta}} \ell ({\mask} \odot {\btheta}^*) 
= -  \frac{1}{\gamma} \mathrm{diag}( \nabla_{\mathbf z} \ell(\mathbf z)
%\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right.
);
% := -\frac{1}{\gamma} \mathrm{diag}(\mathbf{A}).
\label{eq: IG_final}
\end{align}
}%
% The rationale behind Hessian-free assumption is that commonly used ReLU-based neural network tends to form a piece-wise linear decision boundary \emph{w.r.t.} the model parameter $\btheta$. This has been theoretically proved by \,\cite{alfarra2020decision}. Empirical results \cite{finn2017model} also suggest that the absence of the second-order derivative hardly harms the performance of the BLO algorithm. 
Further, the   gradient of the  objective function given by \eqref{eq: GD_bi_level} becomes

{\vspace*{-5mm}
{
\small
\begin{align}
\displaystyle
    \frac{d \ell(\mask \odot \btheta^*)}{d \mask} = ( \btheta^* 
    - 
    \frac{1}{\gamma} \mask \odot \gradzsimple) \odot \gradzsimple,
    \label{eq: upper_update_final}
\end{align}}}%
where
%for ease of notation    {$\gradzsimple$} signifies {$\gradz$}, 
% {\color{red}[I think this does not simplify too much, why not just directly write this in (6)?][at the beginning of the proof we can use this simplification.]} 
%and 
$\odot$ denotes the element-wise multiplication.
\end{myprop}
%\end{tcolorbox}
\textbf{Proof}: Using chain-rule, we can obtain that

\vspace*{-6mm}
{\small
\begin{align}
&    \nabla_{\btheta}\ell(\mask \odot \btheta^*) = %\nabla_{\btheta^*} (\mask \odot \btheta^*)^\top
\mathrm{diag}(\mathbf m)
\gradzsimple = \mask \odot \gradzsimple;
    \label{eq: chainrule_theta} \\
\text{similarly,   } & \nabla_\mask \ell(\mask \odot \btheta^*) 
    % = \nabla_\mask (\mask \odot \btheta^*)^\top \gradzsimple 
    % = \mathrm{diag}(\btheta^*) \gradzsimple 
    = \mathrm{diag}(\btheta^*) \gradzsimple 
    = \btheta^* \odot \gradzsimple \label{eq: chainrule_mask}
\end{align}
}%%
where $\mathrm{diag}(\cdot)$ represents a diagonal matrix with $\cdot$ being the main diagonal vector.
% Similarly, we also have $\nabla_{\btheta^*}\ell(\mask \odot \btheta^*) = \mask \odot \gradzsimple$. 
% For simplicity, we denote $\gradz$ as $\gradzsimple$. 
Further, we can convert \eqref{eq: IG_simplify} to

\vspace*{-6mm}
{
\small
\begin{align}
\displaystyle
    \nabla^2_{{\mask} {\btheta}} \ell({\mask}  \odot {\btheta^*}) 
    % & = \nabla_{{\mask}} \left [ \mathrm{diag}({\mask}) {\gradzsimple} \right ] \\
    & \overset{\eqref{eq: chainrule_theta}}{=} \nabla_{{\mask}} \left [ {\mask} \odot  \nabla_{\mathbf z} \ell(\mathbf z) \right ]
    \nonumber \overset{\text{chain rule}}{=} 
    \mathrm{diag}( {\gradzsimple}) 
    + 
    \mathrm{diag}({\mask}) [ \nabla_{{\mask}} ( \nabla_{\mathbf z} \ell(\mathbf z) ) ]
    % \mask \odot 
    % [\btheta^* \odot \nabla_{\mathbf z \mathbf z} \ell (\mathbf z) 
    % \left |_{\mathbf z = {\mask} \odot {\btheta^*}} \right. 
     \nonumber \\
    & \overset{\eqref{eq: chainrule_mask}}{=}  \mathrm{diag}( {\gradzsimple}) 
    + 
    \mathrm{diag}({\mask}) [ \mathrm{diag}(\btheta^*) \nabla^2_{\mathbf z } \ell(\mathbf z) ] = \mathrm{diag}(\gradzsimple) ,\label{eq: ezBiP}
 \end{align}}%
where the last equality holds due to the Hessian-free assumption. With \eqref{eq: ezBiP} and \eqref{eq: IG_simplify} we can prove \eqref{eq: IG_final}.
% of $\nabla_{\btheta \btheta} \ell = \mathbf 0$.

Next, substituting the IG \eqref{eq: IG_final}  to the upper-level gradient \eqref{eq: GD_bi_level}, we  obtain that

\vspace*{-3.9mm}
{
\small
\begin{align}
\displaystyle
     \frac{d \ell(\mask \odot \btheta^*)}{d \mask} 
    & \,\,\,\,=\nabla_{\mask}\ell({\mask} \odot {\btheta}^*) - 
    {\frac{1}{\gamma}
    \gradzsimple
    % \mathbf{A}
    \odot \nabla_{{\btheta}} \ell({\mask} \odot {\btheta^*})
    } \nonumber \\
    &
    \underset{ }{\overset{\eqref{eq: chainrule_theta}, \eqref{eq: chainrule_mask}}{=}}  \btheta^* \odot \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right.
    - \frac{1}{\gamma} \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right. 
    \odot
    ( \mask \odot \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right. 
    ) 
    %\nonumber \\
   % & \,\,\,\,
    =  (\btheta^* - \frac{1}{\gamma} \mask \odot \gradzsimple
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right.
    ) \odot \gradzsimple, \nonumber
    % \nabla_{\mathbf z} \ell (\mathbf z)\left |_{\mathbf z = {\mask} \odot {\btheta}^*} \right. 
   % \label{eq: upper_final_proof}
\end{align}
}%
which leads to \eqref{eq: upper_update_final}. 
The proof is now complete. \hfill $\square$ 
% \todo{Do we have any empirical evidence that shows that using \eqref{eq: upper_update_final} is better than using \eqref{eq: chainrule_mask}? That would be good to highlight advantage of BLO and IG. \YY{Pari means the significance of the extra term brought by IG.} }

The key insight drawn from Prop.\,\ref{thr: ig} is that the bi-linearity of pruning variables (\textit{i.e.}, $\mask \odot \boldsymbol \theta^*$) makes the  IG-involved gradient \eqref{eq: GD_bi_level} easily solvable, and the   computational complexity is almost the same as that of computing the first-order gradient $\nabla_{\mathbf z} \ell (\mathbf z)$ just once, as supported by   \eqref{eq: upper_update_final} 
% (\YH{see Corollary\,\ref{col: efficiency}}).  {\red[shall we comment somewhere that, even with this simplification, the gradient computation is still different than the existing approaches, and where is potentially the key terms?]} 
%\todo{Pari: computational complexity corollary}

% {\red[shall we make some comments about this corollary? seems a bit abrupt at this point.]}
% \begin{mycor}
% \label{col: efficiency}
% Given $\mask \in \{0, 1\}^n, \btheta \in \mathbb R^n$ and that the computation of the gradient $\nabla_{\mathbf z} \ell (\mathbf z) \in \mathbb R^n$ takes $O(n)$ time, the computation of the loss gradient~\eqref{eq: GD_bi_level} with respect to the mask $\mask$ of the objective~\eqref{eq: prob_bi_level} using \eqref{eq: upper_update_final} in Proposition~\ref{thr: ig} also takes $O(n)$ time.
% \end{mycor}
% Thus, we can prove \eqref{eq: upper_update_final}. As \eqref{eq: upper_update_final} suggests, the upper-level gradient update only involves one backward-propagation and thus, the bi-level pruning can be solved as easily as a first-order alternating optimization problem.

\vspace*{-0.1in}
\paragraph{{\biprune} algorithm and implementation.}
We next 
formalize the {\biprune} algorithm 
%solve the {\biprune} problem \eqref{eq: prob_bi_level} 
based on Prop.\,\ref{thr: ig} and the alternating gradient descent  based BLO solver~\cite{hong2020two}. At iteration $t$, there are two main steps.

\ding{72} \textit{Lower-level SGD for model retraining}: 
Given $\mask^{(t-1)}$, $\btheta^{(t-1)}$, and 
$
\mathbf z^{(t-1)} 
% \btheta_{\mask^{(t)}}^{(t)} 
\Def \mask^{(t-1)} \odot \btheta^{(t-1)}$, we update $\btheta^{(t)}$ by randomly selecting a data batch with the learning rate $\alpha$ and applying SGD (stochastic gradient descent) to the lower-level problem of \eqref{eq: prob_bi_level},%


\vspace*{-5mm}
{\small 
\begin{align}
    \btheta^{(t)} & = \btheta^{(t-1)} - \alpha \nabla_{\btheta} g(\mask^{(t-1)}, \btheta^{(t-1)})  
    % \nonumber 
%   &  \hspace*{-5mm}
   \overset{%\eqref{eq: stationary}, 
   \eqref{eq: chainrule_theta}}{=}
    \btheta^{(t-1)} - \alpha [ \mask^{(t-1)} \odot 
    \nabla_{\mathbf z} \ell(\mathbf z )\left | \right._{\mathbf z = \mathbf z^{(t-1)}} + \gamma \btheta^{(t-1)} ],
    %\nabla_{\btheta} g(\mask^{(t-1)}, \btheta^{(t-1)}) 
    \tag{$\btheta$-step}
    \label{eq: theta_step}
\end{align}}%
% where $\alpha > 0$ is the lower-level   learning rate. 
% {\red[where is the stochasticity coming from? cannot quite see it in the above expression. be a bit more specific.]\YH{I introduced the data batch here.} [also if we use $\nabla_z \ell(z)$ a lot in the paper, maybe consider define it formally in the paper somewhere, instead of defining it in the statement of the thereom.]} \YH{I agree, and a better notation to describe the `masked model parameter'. Maybe something like $\btheta_{\mask}^{(t-1)}$ will be more self-contained. At the beginning, $\mathbf z$ is nothing but an arbitrary choice. }

\ding{72} \textit{Upper-level {SPGD} for pruning}: Given $\mask^{(t-1)}$, $ \btheta^{(t)}$, and $\mathbf z^{(t+1/2)} \Def \mask^{(t-1)} \odot \btheta^{(t)}$, we update   $\mask$ using SPGD (stochastic projected gradient descent) along the IG-enhanced descent direction \eqref{eq: GD_bi_level},%

\vspace*{-5mm}
{\small
\begin{align}
    \mask^{(t)} = & \mathcal P_{\mathcal S} \left [ 
    \mask^{(t-1)}  - \beta  \frac{d \ell(\mask \odot \btheta^{(t)})}{d \mask} \left | \right._{\mask =     \mask^{(t-1)} }
    \right ] \nonumber \\
\overset{\eqref{eq: upper_update_final}}{=}    
    &\mathcal P_{\mathcal S} \left [ 
    \mask^{(t-1)}  - \beta  \left ( \btheta^{(t)} - 
    \frac{1}{\gamma} \mask^{(t-1)} \odot \gradzsimple \left | \right._{\mathbf z = \mathbf z^{(t+1/2)}} \right ) \odot \gradzsimple  \left | \right._{\mathbf z = \mathbf z^{(t+1/2)}}
    \right ],
    \tag{$\mask$-step}
    \label{eq: m_step}
    \vspace{-7mm}
\end{align}}%
where $\beta > 0$ is the upper-level learning rate, and $\mathcal P_{\mathcal S}(\cdot)$ denotes the Euclidean projection   onto the constraint set $\mathcal S$ given by
$\mathcal S = \{ \mathbf m\,|\, \mathbf m \in \{ 0, 1\}^n, \mathbf  1^T \mathbf m \leq k \}$ in \eqref{eq: prob_bi_level} and is achieved by the top-$k$ hard-thresholding operation as will be detailed later.  
% {\red[so if the lower level also uses data batches, is it also an SGD instead of GD? probably need some more elaboration.]} \YH{This is stochastic as well and I think we omit `S' for ease of notation, like the one used in Adversarial Training? This need @Sijia to double check.}

In {\biprune}, the \eqref{eq: theta_step} and \eqref{eq: m_step} steps execute iteratively. In practice, we find that {\biprune} converges very well; see Fig.\,\ref{fig: convergence} for an ablation study.
It is also worth noting that both \eqref{eq: theta_step} and \eqref{eq: m_step} only require the first-order information $\nabla_{\mathbf z} \ell (\mathbf z)$, 
% {\red[theta-step is SGD right? so does not need full gradient.]} \YY{Yes, this is correct.} 
demonstrating that   {\biprune}   can be conducted as efficiently as first-order optimization. 
We present more implementation details of {\biprune}   below and {refer readers to  Appendix\,\ref{app: algorithm}  for a detailed algorithm description}.


\ding{70} \textit{Discrete optimization over $\mask$:} We follow the  {`convex relaxation + hard thresholding'} mechanism used in \cite{ramanujan2020sHiddenSubnetwork,sehwag2020hydra}.
Specifically, we relax the binary masking variables   to continuous masking   scores $\mathbf m \in [\mathbf 0, \mathbf 1]$. We then acquire  loss gradients at  the backward pass based on the relaxed  $\mathbf m$. At the forward pass, we project it  onto the discrete constraint set $\mathcal S$ using the hard thresholding operator, where   the top $k$ elements  are set to $1$s and the others to $0$s. See Appendix\,\ref{app: algorithm} for more discussion.
% \SL{[@Pari, if you want, you could talk about the implementation of $\tilde{m}$  here.]}
% \todo{I think we can just say ``see detailed discussion'' in appendix and have the $\widetilde \mask$ version there. I already have it there but it is commented out right now}
%At  to tn he backward pass for grationadient calculation, we 

\ding{70} \textit{Data batch selection for lower-level and upper-level optimization:} We adopt different data batches (with the same batch size) when implementing \eqref{eq: theta_step} and \eqref{eq: m_step}. This is one of the advantages of the BLO formulation, which enables the flexibility to customize the lower-level and upper-level problems. The use of diverse data batches  is beneficial to generalization as shown in \cite{deng2021meta}. 
% {\red[are data batches changing all the time? or they are fixed at the beginning, and then for the fixed data batch, the theta-step select mini-batches to do sgd?]} \YH{Each m-step and theta-step select a random data batch at each step and nothing is fixed. Both m-step and theta-step are stochasticity-based.}
 
\ding{70} \textit{Hyperparameter tuning:} As described in \eqref{eq: theta_step}-\eqref{eq: m_step},  {\biprune} needs to set two learning rates $\alpha$ and $\beta$ for lower-level and upper-level optimization, respectively. We choose $\alpha = 0.01$ and $\beta = 0.1$ in all experiments, where we adopt the mask learning rate $\beta$ from Hydra\,\cite{sehwag2020hydra} and set a smaller lower-level learning rate $\alpha$, as $\btheta$ is initialized by a pre-trained dense model. We show ablation study on $\alpha$ in Fig.\,\ref{fig: ablation_study}(c).
% The more aggressive lower-level optimization is typically suggested by the convergence of BLO \cite{hong2020two}. 
BLO also brings in the low-level convexification parameter $\gamma $. We set $\gamma = 1.0 $ in   experiments and refer readers to {Fig.\,\ref{fig: ablation_study}(b)} for a sanity check. 

\ding{70} \textit{One-step vs. multi-step SGD:}
In  \eqref{eq: theta_step}, the   one-step SGD is used and helps reduce the computation overhead. In practice, we also find that the one-step SGD is sufficient:  The use of multi-step SGD in {\biprune} does not yield much significant improvement over the one-step version; see {Fig.\,\ref{fig: ablation_study}(a)}.
%computation-friendly. 

\ding{70} \textit{Extension to structured pruning:}
We formulate and solve the {\biprune} problem in the context of unstructured (element-wise)  weight pruning. However, if define the pruning mask $\mask$ \emph{w.r.t.} model's structural units  (\textit{e.g.}, filters), then it is easy to apply {\biprune} to structured weight pruning; see Fig.\,\ref{fig: structured_performance_cifar} and Fig.\,\ref{fig: structured_performance_cifar_appendix} for empirical results.



\iffalse
Next we give some implementation remarks on our algorithm. We adopt the commonly used Cross-Entropy loss as our upper- and lower-level loss functions. To circumvent the difficulty from discrete optimization for binary mask $\mask$, we adopt the widely accepted 
\textbf{soft score + hard threshold} paradigm to deal with $\mask$. We first loosen the binary constraint of $\mask$ from $\{0, 1\}^n$ to $\mathbb R^{n}$ as the `mask score'. After each step, for any given sparsity ratio $p\%$, we update the true binary mask by setting the top $1-p\%$ elements with the highest score to $1$ and the rest to $0$. We emphasize the {\biprune} can be applied to the structured pruning setting simply by changing the threshold operation by wipe out the parameter patterns (\emph{e.g.}, the convolutional kernel) with the lowest score $\ell_2$ norms. In practice, we use different batches $\mathcal{B}_\alpha$ and $\mathcal{B}_\beta$ for upper- and lower-level updates for better generalization ability. {In practice, we will show that the performance of {\biprune} is not sensitive to the lower level step number $K$ in Sec\,\ref{sec: exp}. Thus, unless otherwise specified, we report the results with $K=1$.}
\todo{Can we discuss $\mask_t$ update more formally like $\mask_{t+1} \gets P_\mathcal{S} (\mask_t - \beta (7))$?}
\fi 
% For initialization, the model parameter $\btheta_0$ are initialized with \textit{Kaiming Normal}\,\cite{he2015delving} and 

\iffalse
The mask scores $\mask_0$ are scaled proportionate to the model weights\,\cite{sehwag2020hydra} and the initial binary mask $\mask$ is initialized \emph{w.r.t.} the score initialization $\mask_0$. We use separate learning rates for upper and lower-level problems namely $0.1$ for sparse mask and $0.01$ for the model parameter. We further set the lower-level problem regularization coefficient to $0.1$.  We will show in Sec.\,\ref{sec: exp} that these hyper-parameter choices are consistently used in all settings and are easy to tune.
\fi 
% In our algorithm, we choose the upper- and lower-level objective as the commonly used model training loss function $\ltr$, such as Cross-Entropy loss. 
% Our algorithm is shown in Algorithm\,\ref{alg: BiP}. 
% In our implementation, we adopt the \textbf{soft score + hard threshold} paradigm to train the discrete variable $\mask$. We first loosen the binary constraint of $\mask$ from $\{0, 1\}^d$ to $\mathbb R^{d}$ as the `mask score'. After each step, for any given sparsity ratio $p\%$, we update the true binary mask $\mathbf{z}^*$ by setting the top $1-p\%$ elements with the highest score to $1$ and the rest to $0$ (denoted as threshold operation $\mathcal{T}_{\{0,1\}^d}$ in \eqref{eq: threshold}). We emphasize the {\biprune} can be applied to the structured pruning setting simply by changing the threshold operation by wipe out the parameter patterns (\emph{e.g.}, the convolutional kernel) with the lowest score $\ell_2$ norms.

% We use separate learning rates for upper and lower-level problem namely $0.1$ for sparse mask and $0.01$ for model parameter. We further set the lower-level problem regularization coefficient to $0.1$.  We will show in Sec.\,\ref{sec: exp} these hyper-parameter choices are consistently used in all settings and are easy to tune.
% For initialization, 
% the model parameter $\btheta_0$ are initialized with \textit{Kaiming Normal}\,\cite{he2015delving} and the mask scores $\mask_0$ are scaled proportionate to the model weights\,\cite{sehwag2020hydra}. 
% The initial binary mask $\mathbf{z}^*$ is initialized \emph{w.r.t.} $\mask_0$. 

% \newpage 


==> Deprecated_NO_USE/Version_Camera_08041600_Submission/combine_23_Yuguang.tex <==
\vspace*{-2mm}
\section{Related Work and Open Question}
\label{sec: preliminary}
%
\vspace*{-0.1in}
\paragraph{Neural network pruning.}
As neural networks become deeper and more sophisticated,
%and over-parameterized,
model pruning technology has gained increasing attention over the last decade since pruned models are necessary for the deployment of deep networks in practical applications~\cite{han2015deep, denil2013overparamterized_and_redundancy}. 
With the goal of finding highly-sparse {\em and} highly-accurate subnetworks from original dense models, 
%Based on different regimes to find the sparse model mask, 
a variety of pruning methods have been developed such as    heuristics-based pruning \cite{frankle2018lottery,lee2018snip, wang2020pick,tanaka2020pruning, alizadeh2022prospect, zhang2021efficient} and  optimization-based pruning \cite{ramanujan2020sHiddenSubnetwork, sehwag2020hydra, lee2020layer, csordas2020neural}.
The former identifies redundant model weights by leveraging heuristics-based metrics such as weight magnitudes~\cite{han2015learning,frankle2018lottery,frankle2020linear,chen2021lottery, ma2021sanity, janowsky1989pruning,  frankle2020pruning}, gradient magnitudes~\cite{lee2018snip, wang2020pick, tanaka2020pruning, mozer1989skeletonization}, and Hessian statistics~\cite{molchanov2019importance, yao2020pyhessian, lecun1990optimal, hassibi1993second, molchanov2016pruning}.% and low-rank matrix factorization~\cite{chee2021pruning, swaminathan2020sparse, idelbayev2020low}
%\todo{Low-rank MF is not reall a ``heuristics-based metric'' like the other previous quantities. A diff. way to say this? \SL{Removed it.}}
%  \SL{[add grasp, SynFlow, snip?? do they belong to?]}
%  Taylor coefficients~\cite{molchanov2016pruning} \SL{[I did not understand Taylor coefficients. Please be more specific and preciser.]}.
The latter is typically built on: 1)~sparsity-promoting optimization \cite{ren2018admmnn, wang2020neural, liu2017learning,he2017channel,zhou2016less,louizos2017learning},
%  \SL{[add admm pruning from Yanzhi's group; no need to cite optimization literature]},
 where model weights are trained by penalizing their sparsity-inducing norms, such as \RV{$\ell_0$ norm to encourage weights to be exactly zero}, $\ell_1$ norm for irregular weight pruning, and $\ell_2$ norm for structured pruning; 2)~parameterized masking \cite{ramanujan2020sHiddenSubnetwork, sehwag2020hydra, guo2021gdp, liberis2021differentiable, kusupati2020soft, xue2021rethinking, zhou2021effective}, where model weight scores are optimized to filter the most important weights and achieve better performance. 
 %or formulate the pruning problem to the constrained optimization problem\,\cite{boyd2011distributed,ouyang2013stochastic,ren2018admmnn,guo2021gdp, sehwag2020hydra}.
 
\noindent \textbf{Iterative vs. one-shot pruning, and motivation.}
%\todo{would {\bf Iterative vs one-shot pruning} be a better paragraph title? \\ \YY{Agree. Solved.}} 
Existing schemes can be further categorized into one-shot or iterative pruning based on the pruning schedule employed for achieving the targeted model sparsity.
% Heuristics-based pruning methods can be further categorized into the one-shot and iterative pruning methods, based on whether the found sparse mask is one-time generated or approached through multiple pruning cycles.
Among the iterative schemes, the IMP (Iterative Magnitude Pruning scheme) \cite{frankle2018lottery, chen2020lottery, gale2019state, pmlr-v139-zhang21c, chen2020lottery2, yu2019playing, chen2021gans, ma2021good, gan2021playing, chen2021unified, kalibhat2021winning, chen2021ultra} has played a significant role in identifying high-quality sub-networks or `winning tickets', as postulated by 
%, which is capable of achieving extreme sparsity without losing performance by iteratively update the mask with increasing sparsity. As one successful sub-field of IMP,
LTH  (Lottery Ticket Hypothesis)  \cite{Renda2020Comparing,frankle2020linear}.
%, which unveils the existence of `winning tickets', \textit{i.e.}, sub-networks that can be trained in isolation to reach or even succeed over the performance of the original dense model.
% managed to find sparse neural network, which can match the performance of the full model when trained from scratch (\emph{a.k.a.} the \textbf{winning ticket}). 
% Further explorations\,\cite{Renda2020Comparing,frankle2020linear} incorporates weight rewinding and managed to scale LTH to large networks and datasets. 
% Applications of LTH on plenty of fields other than image classification are also studied\,\cite{gale2019state,pmlr-v139-zhang21c,chen2020lottery,chen2020lottery2,yu2019playing,chen2021gans,ma2021good,gan2021playing,chen2021unified,kalibhat2021winning,chen2021gans,chen2021ultra}, (\emph{e.g.}, natural language processing\,\cite{gale2019state,chen2020lottery}).  
% However, it is computationally expensive to find winning tickets by IMP due to its iterative nature. 
% As a computation-efficient counterpart of IMP, One-shot Magnitude Pruning (OMP)\,\cite{frankle2018lottery} is developed, where a dense model is directly pruned to the targeted sparsity.  The other one-shot pruning methods such as pruning at initialization \cite{wang2020pick,lee2018snip,tanaka2020pruning,alizadeh2022prospect} further reduce the computation cost of pruning by avoiding the dense model training. Yet, it is worth noting that the gain of efficiency using one-shot pruning is accompanied by the loss of pruning accuracy, compared to iterative pruning.
%
% \paragraph{Put some preliminary here}
%
For example, the current  state-of-the-art (SOTA) implementation of IMP in \cite{ma2021sanity} can lead to a pruned ResNet-20 on
% \SL{[This example  number needs to be   better aligned with the later figure, then you can cite it here.]}
CIFAR-10 with 74\% sparsity and $92.12\%$ test accuracy, matching the performance of the original dense model (see \textcolor{red}{red $\star$} in Fig.\,\ref{fig: one_shot_results_merged}-{\bf Left}). 
% For the larger-size {ResNet-18} model, IMP   can identify a sparser network with   {$95\%$ sparsity and $94.81\%$ test accuracy, yielding the $0.5\%$ improvement over the original dense model}; \SL{see Fig.\,xxx in Sec.\,xxx}.
The IMP algorithm typically contains two key ingredients: \textbf{(i)}~a \textit{temporally-evolving pruning schedule} to progressively increase model sparsity over pruning iterations, and \textbf{(ii)}~the \textit{pruning-retraining learning mechanism} applied at each pruning iteration. 
% To be more specific, 
% IMP  repeatedly trains, prunes, and resets the network over multiple rounds (say $n$ rounds). 
With a target pruning ratio of $p\%$ with $T$ pruning
% \SL{[$n$ has been used for dimension later. I changed it to $T$.]}
iterations, an example pruning schedule in (i) could be as follows -- each iteration prunes $(p\%)^{\nicefrac{1}{T}}$ of the currently unpruned model
weights, progressively pruning fewer weights in each iteration.
%This leads to a pruning mask $\mathbf m$ at each round. 
For (ii), 
the unpruned weights in each pruning iteration are re-set to the  weights at initialization or at an early-training epoch \cite{Renda2020Comparing}, and   re-trained till convergence. 
In brief, IMP repeatedly prunes, resets, and trains the network over multiple iterations.
%
% A common example, the Lottery Ticket Hypothesis (LTH), can achieve comparable or even better performance with a sparsity of over $95\%$ in its state-of-the-art (SOTA) implementation\,\cite{ma2021SanityCheckLTH}. 
% In general, the heuristics-based IMP adopts a sparsifying-retraining paradigm which consists of multiple iterative cycles: \underline{\textit{(1)}} \textbf{training} dense model with several epochs; \underline{\textit{(2)}} \textbf{pruning} $p\%$ redundant model weights with certain heuristics-based criteria (\emph{e.g.} model weight magnitude) to obtain the new mask; \underline{\textit{(3)}} \textbf{fine-tuning} the sparse network with the found mask and rewound weights for accuracy recovery. 

\begin{wrapfigure}{r}{85mm}
\vspace*{-5mm}
\centerline{
\begin{tabular}{cc}
\hspace*{0mm}\includegraphics[width=.3\textwidth,height=!]{figure/performance_comparison.pdf}  
&\hspace*{-4mm}\includegraphics[width=.31\textwidth,height=!]{figure/time_comparison_long.pdf}
% \\
% \hspace*{2mm}\footnotesize{(a) Test accuracy vs. pruning ratio.} &   \footnotesize{(b) Runtime of pruning.}
\end{tabular}}
\vspace*{-3mm}
\caption{\footnotesize{
Illustration of the pros and cons of different pruning methods executed over (ResNet-20, CIFAR-10).
{\bf Left}: test accuracy vs. different pruning ratios of IMP and one-shot pruning methods (\textsc{OMP}\,\cite{frankle2018lottery}, \textsc{Grasp}\,\cite{wang2020pick}, \textsc{Snip}\,\cite{lee2018snip}, \textsc{SynFlow}\,\cite{tanaka2020pruning}). {\bf Right}: comparison of the computation time with different sparsity levels. 
%We highlight we adopt the SOTA implementation of OMP  following\,\cite{ma2021sanity} and other methods following their original settings.
% \SL{For (a): Update x-y axis and mark the $95\%$ or $99\%$ pruning point.}
% \SL{For (b): [X-axis: Pruning method, add the dense model training time.]}
% \SL{Illustration of  the pros and cons of different pruning methods executed over (ResNet-xxx, CIFAR-10).
% (a) Test accuracy against pruning ratio: IMP significantly outperforms one-shot pruning methods (OMP [refs], ....). (b) Computation time of pruning to different sparsity levels:  IMP becomes much more computational intensive when pruning is targeted for a higher sparsity level ($99\%$ vs. $60\%$).
% }
% Performance and efficiency comparison between IMP (LTH) and various one-shot pruning methods on CIFAR10 and ResNet20. One-shot methods save pruning time at the cost of significant performance drop compared to IMP (LTH).
}}
  \label{fig: one_shot_results_merged}
  \vspace*{-4mm}
\end{wrapfigure}
%
However, winning tickets found by IMP incur significant computational costs. The sparsest winning ticket found by IMP in Fig.~\ref{fig: one_shot_results_merged}-{\bf Left} (\textcolor{red}{red $\star$}) utilizes $T=6$  
pruning iterations. As shown in Fig.~\ref{fig: one_shot_results_merged}-{\bf Right}, this takes 3$\times$ more time than the original training of the dense model.
%\todo{In fig 3, one plot says "dense model", other one says "model pretrain". can we say "dense model" and "dense model" or "dense model train". What do you think will make things more consistent? \\ \YY{Dense Model. Fixed}}
%
%\SL{[I stop here]}
%Yet, the superior pruning accuracy   of IMP is at the cost of  computation efficiency. For ease of illustration, Fig.\,\ref{fig: one_shot_results_merged} shows the example of pruning ResNet-20 over CIFAR-10 and demonstrates   the accuracy and the computation time of various pruning methods versus the growing sparsity ratio.
%and (b) the computation time of model pruning with different sparsity levels.
% \SL{For ease of illustration, Fig.\,\ref{fig: one_shot_results} shows a pruning example that unveils (a) the accuracy performance of various pruning methods versus the growing sparsity ratio, and (b) the computation time of model pruning with different sparsity levels.}
%As we can see, IMP outperforms   the other pruning baselines and finds the sparsest winning ticket (marked by the red star in Fig.\,\ref{fig: one_shot_results_merged}a) using $n = 6$ pruning iterations. 
%However, this leads to $3\times$ more than the cost of training a dense model from scratch.
% \SL{the $95\%$-sparsity ResNet-18 model with $94.81\%$ test accuracy on CIFAR-10 takes $n = xxx$ pruning rounds. This leads to $xxx$-min runtime, which is $xxx$ times higher than training a dense model and $xxx$ times higher than pruning to the $60\%$  sparsity level.} 
%and thus hampers the pruning efficiency 
%
% \todo{Replace 3a/3b in text with 3(left)/3(right). \YH{Fixed}}
%
To avoid the computational cost of IMP, different kinds of `accelerated' pruning methods were developed  \cite{frankle2018lottery,lee2018snip, wang2020pick,tanaka2020pruning, alizadeh2022prospect, zhang2021efficient}, and many fall into the \textit{one-shot pruning} category: The network is directly pruned to the target sparsity  and retrained once. 
%: the network is trained once, p% of weights are pruned, and the surviving weights are reset.
% which refines the sparse mask directly to the given sparsity only one time. 
In particular, \textsc{OMP}  (one-shot magnitude pruning) is an important baseline that simplifies IMP~\cite{frankle2018lottery}.
It follows the pruning-retraining paradigm, but  prunes the model to the target ratio with a single pruning iteration. 
% \SL{Although some existing work\,\cite{ma2021SanityCheckLTH} observed that OMP and the other one-shot pruning methods (e.g., ProsPr\,\cite{alizadeh2022prospect}) could find winning tickets and achieve similar accuracy performance to IMP. However, this conclusion is model/dataset-specific. }
% Although some preliminary results showed that 
% existing work\,\cite{ma2021sanity}(\YH{cite TBD}) observed that OMP and the other one-shot pruning methods (e.g., \textsc{ProsPr}\,\cite{alizadeh2022prospect}) could find winning tickets and achieve similar accuracy performance to IMP at low sparsity levels. However, this conclusion is model/dataset-specific.
\iffalse
However,  the promise of current one-shot pruning methods is dataset/model-specific~\cite{ma2021sanity, su2020sanity_random_win} and mostly lies in the low pruning ratio regime~\cite{alizadeh2022prospect}.
As systematically studied in~\cite{ma2021sanity, frankle2020pruning}, there exists a performance gap between one-shot pruning and IMP.
\fi 
%Fig.\,\ref{fig: one_shot_results_merged} highlights the above limitation -- 
Although one-shot pruning schemes are computationally cheap (Fig.\,\ref{fig: one_shot_results_merged}-{\bf Right}), they incur a significant accuracy drop compared to IMP (Fig.\,\ref{fig: one_shot_results_merged}-{\bf Left}).
{Even if IMP is customized with a reduced number of training epochs  per pruning round, the pruning accuracy also drops largely (see Fig.\,\ref{fig: compare_IMP_OMP_GMP}).}
% \textcolor{red}{Besides, IMP also suffers from severe performance degradation, if its epoch numbers per pruning iteration is reduced to improve efficiency. (see Fig.\,\ref{fig: compare_IMP_OMP_GMP}).}
% with fewer epochs per pruning iteration also improves the computational efficiency but degrades the performance (see Fig.\,\ref{fig: compare_IMP_OMP_GMP}).}
%For example, \textsc{OMP} and \textsc{ProsPr} \cite{alizadeh2022prospect}, the SOTA methods of one-shot pruning,   yield  over $2\%$ and $10\%$ accuracy drop compared to IMP at the $74\%$ and  $98\%$ sparsity level, respectively.
Hence, there is a need for advanced model pruning techniques to find winning tickets like IMP, while being efficient like one-shot pruning.
%Thus,  there exists a strong demand for the algorithmic advancement of model pruning that can   enjoy the dual advantages of one-shot pruning and IMP.




% To improve the efficiency, various one-shot pruning methods such as One-shot Magnitude Pruning (OMP)\,\cite{frankle2018lottery} and prune-at-initialization\,\cite{wang2020pick,lee2018snip,tanaka2020pruning,alizadeh2022prospect} methods, propose to refine the model mask only one time and thus spare the cost of multiple retraining. Nevertheless, the current one-shot pruning methods still suffer from significant performance drop compared to IMP and hard find any winning tickets, making them impractical for real-world application\,\cite{frankle2020pruning}.
%\vspace*{-1mm}
Different from unstructured weight pruning described above,  structured pruning takes into consideration the sparse patterns of the model, such as filter and channel-wise pruning~\cite{he2017channel, guo2021gdp, li2016pruning, chen2022coarsening, niu2020patdnn, ma2020image, wang2022paca, van2020single}.
% \SL{[please cite more e.g., pattern-aware pruning from yanzhi's group]}.  
Structured pruning is desirable for deep model deployment in the presence of hardware constraints~\cite{han2015deep, denil2013overparamterized_and_redundancy}.
% \SL{[refs]}. 
However, compared to unstructured pruning, it is usually more challenging to maintain the performance and find structure-aware winning tickets~\cite{you2019drawing, zhang2021efficient}.
% \SL{[refs]}. 

%\paragraph{Problem Statement.}
\vspace*{-3mm}
\paragraph{Open question.}
As discussed above, 
{one-shot pruning methods are unable to match the predictive performance of IMP, and structure-aware winning tickets are hard to find. One possible cause is the requirement to prune in a single iteration or in a structure-constrained space mainly through   heuristics-based  strategies, while the best optimization foundation of model pruning is underdeveloped. Thus, we consider the following open question:} 
% one-shot pruning methods are unable to match the predictive performance of IMP, and struct winning tickets are hardly to find. One possible cause is the requirement to prune in a single iteration or in a structure-constrained space using heuristics-based  strategies. This raises the question of  whether 
% computational efficiency and pruned model accuracy could be simultaneously improved through a rigorous and dedicated optimization-based approach.
% a theoretically-grounded optimization-based approach can renovate one-shot pruning so as to improve the computation complexity of pruning while attaining the accuracy performance comparable to IMP.
% Based on the aforementioned dilemma between performance and pruning cycle number in heuristics-based pruning methods, we ask the following question:
%Specifically we consider the following open question:
%Thus, we ask:  \textit{Beyond heuristics, how to establish the \textbf{optimization basis} of a successful pruning mechanism that can attain high pruning  accuracy (like IMP) as well as high   computation efficiency (like one-shot pruning)?}
\begin{tcolorbox}
\vspace*{-2mm}
Is there an \textbf{optimization basis} for a successful pruning algorithm that can attain high pruned model accuracy (like IMP) {\em and} high computational efficiency (like one-shot pruning)?
\vspace*{-2mm}
\end{tcolorbox}
%
The model pruning problem has a natural hierarchical structure -- we need to find the best mask to prune model parameters, {\em and then}, given the mask, find the best model weights for the unpruned model parameters. Given this hierarchical structure, we believe that the {\em bi-level optimization (BLO)  framework} is one promising optimization basis for a successful pruning algorithm.
{We briefly review the BLO-related work below.}
% \begin{center}
%     \textit{Beyond heuristics, how to establish the \textbf{optimization basis} of a successful pruning mechanism that can close the gap between pruning accuracy (e.g., achieved by IMP) and computation efficiency (e.g., achieved by OMP)?}
% \end{center}
%
% Pruning methods can also be roughly categorized into the structured and unstructured pruning methods according to the regularity of the found sparse pattern. As most of the above mentioned pruning algorithms fall into the unstructured group, structured pruning is designed to remove the redundant weights with basic pruning units like filters, channels or other certain patterns of parameters\,\cite{he2017channel,li2016pruning,guo2021gdp,chen2022coarsening}. Such methods are usually more efficient and friendly for deployment on hardware, while suffering from major performance drops in most cases and have difficulty in find the winning tickets as the SOTA unstructured method (\emph{e.g.}, LTH) does.
%
% From the perspective of the , the pruning methods can be categorized into two classes: the unstructured\,\cite{han2015deep, frankle2018lottery,mostafa2019parameter, mocanu2018scalable,evci2020rigging} and the structured pruning\,\cite{hu2016network}. 
%
% Unstructured pruning, including global pruning \cite{frankle2018lottery, lecun1989optimal, hassibi1992second} and layer-wise pruning \cite{ sehwag2020hydra, ramanujan2020sHiddenSubnetwork}, is designed to remove the model parameters without any pattern constraints, \emph{e.g.}, filter-wise or group-wise\,\cite{chen2022coarsening}. 
% One of the most successful branches is called the Iterative Magnitude Pruning (IMP) method\,\cite{han2015deep,frankle2018lottery,chen2020lottery}, which iteratively prunes and retrains the model parameters with a certain pruning ratio until the network reaches a certain sparsity level. Although IMP works effectively in most cases, the high computational costs brought by its working pattern make it hard to scale to large networks and datasets. 
% Thus, to reduce the computational cost by IMP, some more efficient methods such as initial pruning, sub-sampling, and pre-training-based methods\,\cite{lee2018snip,wang2020pick,tanaka2020pruning,luo2020neural,zhang2021efficient,you2019drawing,chen2020lottery} were proposed as well.
%
% Another major direction is structured pruning, where the basic pruning unit becomes filters, channels, or certain patters of parameters\,\cite{he2017channel,li2016pruning,guo2021gdp,chen2022coarsening}. Such methods are usually more efficient and friendly for deployment on hardware, while suffering from major performance drops in most cases.
% Although most pruning methods work in a three-step pipeline, where a model goes through the process of pretraining, pruning and retraining\,\cite{han2015training, guo2016dynamic}, some methods were propose
%
% There is another categorization for pruning methods, including heuristic and optimization-based pruning. Most pruning methods fall into the heuristic category, which correlates the pruning mask to the magnitude, gradient, or the hessian\,\cite{han2015deep,frankle2018lottery,chen2020lottery,lecun1989optimal, hassibi1992second}, while some optimization-based pruning methods\,\cite{han2015learning} also demonstrate their effectiveness, \emph{e.g.}, HYDRA \cite{sehwag2020hydra} for robust pruning and STR \cite{kusupati2020soft_thres_learnable} for layer-wise sparsity.
%
%% 
%
%% 
% \SL{[I stop here. @Pari, if possible, please feel free to check the following. I will do it tonight as well.]}
% To bridge the gap between the one-shot pruning and IMP and explore the possibility of achieving winning tickets in structured pruning, we revisit pruning problem from the perspective of bi-level optimization. In our work, we for the first time propose an efficient first-order pruning framework through bi-level optimization for both structured and unstructured pruning. In particular, our proposed algorithm solves the bi-level pruning algorithm and achieves better performance in various settings than IMP with computational costs comparable to OMP.
% with the first-order computational costs
% Our algorithm keeps the training computational costs comparable to normal one-step alternative optimization based methods \cite{ramanujan2020sHiddenSubnetwork} while achieving the state-of-the-art performance in various pruning settings.
%
%
\vspace*{-0.1in}
\paragraph{Bi-level optimization (BLO).} BLO is a general hierarchical optimization framework, where the upper-level problem depends on the solution to the lower-level problem. Such a nested structure makes the BLO in its most generic form very difficult to solve, since it is hard to characterize the influence of the lower-level optimization on the upper-level problem. Various existing literature focuses on the design and analysis of algorithms for various special cases of BLO. Applications range from the classical approximate descent methods\,\cite{falk1995bilevel, vicente1994descent}, penalty-based methods\,\cite{white1993penalty, gould2016differentiating}, to recent BigSAM\,\cite{sabach2017first} and its extensions\,\cite{liu2020generic, li2020improved}. It is also studied in the area of stochastic algorithms\,\cite{ghadimi2018approximation, ji2020bilevel, hong2020two} and back-propagation based algorithms\,\cite{franceschi2017forward, grazzi2020iteration, shaban2019truncated}. BLO has also advanced adversarial training\,\cite{zhang2021bat}, meta-learning\,\cite{rajeswaran2019meta}, data poisoning attack generation\,\cite{huang2020metapoison}, neural architecture search\,\cite{liu2018darts} as well as reinforcement learning\,\cite{chen2019research}. 
However, to the best of our knowledge, the BLO framework  has not been {rigorously} considered for neural network pruning. 
\RV{We notice \cite{louizos2017learning} mentioned BLO in pruning while adopted alternating optimization instead.}
% \RV{Bi-level optimization has ever been mentioned in the pruning literature \cite{louizos2017learning}, but only alternating optimization is applied to perform training and pruning.} 
{We will show that model pruning yields a special class of BLO problems with bi-linear optimization variables. We will also theoretically  show that  this specialized BLO problem for model pruning can be  solved as efficiently as first-order optimization. This is in a sharp contrast to existing BLO applications  that rely on heuristics-based BLO solvers (\textit{e.g.}, gradient unrolling in meta learning \cite{rajeswaran2019meta} and neural architecture search \cite{liu2018darts}).}
%Our work, for the first time, advances the algorithmic foundation of neural network pruning through the lens of BLO.

% \section{Preliminaries and Motivation}
% \label{sec: preliminary}


% In this section, we begin by providing a brief   background of neural  network pruning, including the predominant   iterative magnitude pruning (IMP) method and the 
% associated lottery ticket hypothesis (LTH)
% \cite{frankle2018lottery} to find high-quality subnetworks (known as `winning tickets') that--when trained in isolation--reach test accuracy comparable to or even better than the original dense network. 
% However, the superior performance of IMP is accompanied with a prohibitive computation cost, as will be exemplified in Fig.\,\ref{fig: one_shot_results}. In  order to overcome the computational difficulty of IMP, we next introduce the  one-shot   pruning method and elaborate on its comparison with IMP. Spurred by the pros and cons of current pruning methods, we eventually state the problem to be studied in this paper. 
 

% \paragraph{{Heuristics-based IMP.}}
% The heuristics-based IMP is the  currently prevailing approach  to
% identify the `winning ticket' in model pruning, so as to attain model sparsity without suffering  performance loss\,\cite{frankle2018lottery,Renda2020Comparing,frankle2020linear,blalock2020state,chen2020lottery,chen2021lottery}. 

\iffalse
Although IMP-based pruning approaches have become the rising star sub-field in pruning, its current success largely sacrifices the pruning efficiency. Within each pruning cycle, the sparse structure is obtained by removing a small fixed pruning ratio (\emph{e.g.}, $20\%$ in LTH) of the \textbf{remaining weights} to make the final sparse model match the full performance of the dense model. Thus, the required pruning iterative numbers as well as their training time grow exponentially as the sparsity increases. For example, the SOTA implementation of LTH\,\cite{ma2021SanityCheckLTH} has to go through 22 pruning cycles to arrive at a sparsity of $99\%$. In such a case, the immense training time consumption has become one clear obstacle of IMP from scaling to large model architectures and datasets\,\cite{zhang2021efficient}.
\fi 
%

%\textit{i.e.}, improve the tradeoff  between computation efficiency and pruning accuracy. 
% Even the SOTA one-shot pruning method \textsc{ProsPr}\,\cite{alizadeh2022prospect} also suffers from an accuracy drop of over $10\%$ compared to IMP when $99\%$ parameters are pruned.
% As demonstrated in Figure\,, all one-shot  
%\todo{I don't see 99\% sparsity level in Figure~\ref{fig: one_shot_results}. Do we mean 90\%?
%
%\YY{Solved.}}
%
%the observed accuracy-efficiency tradeoff
%the accuracy-efficiency tradeoff of one-shot pruning is based on the heuristics-based one-shot pruning 
%This efficiency-performance trade-off is primarily due to the heuristic nature, which is insufficient to find satisfactory masks with an extreme sparsity using the radical pruning ratio as OMP does.
%

%\newpage 


% \paragraph{\SL{Heuristics-based IMP.}}
% The heuristics-based Iterative Magnitude Pruning (IMP) has been the predominant approach to obtain sparse neural networks. A common example, the Lottery Ticket Hypothesis (LTH), can achieve comparable or even better performance with a sparsity of over $95\%$ in its state-of-the-art (SOTA) implementation\,\cite{ma2021SanityCheckLTH}. 
% In general, the heuristics-based IMP adopts a sparsifying-retraining paradigm which consists of multiple iterative cycles: \underline{\textit{(1)}} \textbf{training} dense model with several epochs; \underline{\textit{(2)}} \textbf{pruning} $p\%$ redundant model weights with certain heuristics-based criteria (\emph{e.g.} model weight magnitude) to obtain the new mask; \underline{\textit{(3)}} \textbf{fine-tuning} the sparse network with the found mask and rewound weights for accuracy recovery. 
% \begin{wrapfigure}{r}{85mm}
% \vspace*{0mm}
% \centerline{
% \begin{tabular}{cc}
% \hspace*{0mm}\includegraphics[width=.3\textwidth,height=!]{figure/performance_comparison.png}  
% &\hspace*{-5mm} 
% \includegraphics[width=.32\textwidth,height=!]{figure/time_comparison.png}
% \vspace*{-0mm}
% \\
% \footnotesize{(a) Performance comparison.} &   \footnotesize{(b) Efficiency comparison.}
% \end{tabular}}
% \vspace*{-2mm}
% \caption{\footnotesize{Performance and efficiency comparison between IMP (LTH) and various one-shot pruning methods on CIFAR10 and ResNet20. One-shot methods save pruning time at the cost of significant performance drop compared to IMP (LTH).
% }}
%   \label{fig: one_shot_results}
%   \vspace*{-5mm}
% \end{wrapfigure}

% Although IMP-based pruning approaches have become the rising star sub-field in pruning, its current success largely sacrifices the pruning efficiency. Within each pruning cycle, the sparse structure is obtained by removing a small fixed pruning ratio (\emph{e.g.}, $20\%$ in LTH) of the \textbf{remaining weights} to make the final sparse model match the full performance of the dense model. Thus, the required pruning iterative numbers as well as their training time grow exponentially as the sparsity increases. For example, the SOTA implementation of LTH\,\cite{ma2021SanityCheckLTH} has to go through 22 pruning cycles to arrive at a sparsity of $99\%$. In such a case, the immense training time consumption has become one clear obstacle of IMP from scaling to large model architectures and datasets\,\cite{zhang2021efficient}.

% \paragraph{IMP versus OMP}
% To reduce the computation overhead of IMP, many efficient pruning methods are proposed in recent years\,\cite{zhang2021efficient, frankle2018lottery, wang2020pick,lee2018snip,tanaka2020pruning, alizadeh2022prospect} and most of them belong to the one-shot pruning category, which refines the sparse mask directly to the given sparsity only one time. 
% The one-shot magnitude pruning (OMP) serves as one important example.
% Inheriting the sparsifying-retraining paradigm, OMP prunes the model to the target sparsity with only one pruning cycle. However, the degradation in accuracy of the one-shot methods is still significant compared to IMP (LTH), making them impractical to real world applications\,\cite{frankle2020pruning}.
% As shown in Figure\,\ref{fig: one_shot_results}, alghouth one-shot pruning methods consume
% significantly less time especially, they all suffer from dramatic performance gaps compared to IMP, especially at large sparsity. Even the SOTA one-shot pruning method \textsc{ProsPr}\,\cite{alizadeh2022prospect} also suffers from an accuracy drop of over $10\%$ compared to IMP when $99\%$ parameters are pruned.
% % As demonstrated in Figure\,, all one-shot  
% This efficiency-performance trade-off is primarily due to the heuristic nature, which is insufficient to find satisfactory masks with an extreme sparsity using the radical pruning ratio as OMP does.

% \paragraph{Problem Statement}
% Based on the aforementioned dilemma between performance and pruning cycle number in heuristics-based pruning methods, we ask the following question:

% \begin{center}
%     \textit{Beyond heuristics, what is the \textbf{optimization basis} of the successful pruning-retraining mechanism? Can we close the gap between OMP and IMP with \textbf{theoretically-grounded} optimization-based pruning methods?}
% \end{center}








% % { % SL Comments 
% % \section{\SL{Preliminaries and Motivation (1 page)}}

% % \paragraph{\SL{Heuristics-based iterative magnitude pruning.}}
% % \begin{enumerate}
% %     \item Motivation on IMP (e.g., SOTA). 
% %     Define IMP.
% %     Introduces LTH and sparsification-retraining based pruning paradigm (Algorithm like our CVPR paper on LTH for backdoor). 
% %     \item Pros and cons of IMP, and then motivates one-shot magnitude pruning (OMP).
    
% % {[Then, we need to demonstrate the limitations of IMP, and pose the following question:
% % Do we have to prune-retrain a model iteratively, based on a growing pruning  schedule?
% % Then introduces the question of one-shot pruning (i.e., pruning a model directly to a fixed sparsity)? 
% % ]}
% % \end{enumerate}

% % \paragraph{\SL{IMP versus OMP.}}

% % \begin{enumerate}
% %     \item Define and formalize OMP.
% %     \item Motivating results figure: IMP vs. OMP to demonstrate that there exists a performance gap between OMP and IM.
% % \end{enumerate}

% % \paragraph{\SL{Problem statement.}}

% % \SL{[We need to state the problems of our interest in this paper based on the limitations of heuristics-based pruning approaches and OMP vs. IMP. ]}
% % \begin{enumerate}
% %     \item Beyond heuristics, what is the  optimization base of the successful pruning-retraining mechanism?  
% %     \item Assisted by technically-grounded optimization, can we close the gap between OMP and IMP?
% % \end{enumerate}
% % }

==> Deprecated_NO_USE/Version_Camera_08041600_Submission/exp_SL.tex <==
In this section, we present extensive experimental results to show the effectiveness of {\biprune}  
%in both accuracy and   efficiency
across multiple model architectures,  various datasets, and different pruning setups. Compared to IMP, one-shot pruning, and optimization-based pruning baselines, 
we find that {\biprune} can find better winning tickets in most cases and is computationally   efficient. 

\vspace*{-0.1in}
\subsection{Experiment Setup}
\vspace*{-0.1in}
\paragraph{Datasets and models.}
Following the pruning benchmark in \cite{ma2021sanity}, 
we consider 4 datasets including CIFAR-10\,\cite{krizhevsky2009learning}, CIFAR-100\,\cite{krizhevsky2009learning}, Tiny-ImageNet\,\cite{le2015tiny}, ImageNet\,\cite{deng2009imagenet}, and 5
architecture types  including  ResNet-20/56/18/50
% \SL{[do we really need RN here?]}
and VGG-16 \cite{he2016deep,simonyan2014very}. 
%ResNet\,\cite{he2016deep}, VGG\,\cite{simonyan2014very}\} for evaluation. 
Tab.\,\ref{table: impl_details} summarizes these datasets and model configurations and setups.  

% For more details on the dataset-model architecture combination, please refer to Table\,\ref{table: impl_details}.
% We summarize our detailed training setups and hyper-parameter selections in Table\,\ref{table: impl_details}. For both unstructured and structured pruning, we adopt two architecture series ResNet\,\cite{he2016deep} and VGG\,\cite{simonyan2014very} for four representative datasets, namely \emph{i.e.,} CIFAR-10\,\cite{krizhevsky2009learning}, CIFAR-100\,\cite{krizhevsky2009learning}, Tiny-ImageNet\,\cite{le2015tiny}, and ImageNet\,\cite{deng2009imagenet}. 


\vspace*{-0.1in}
\paragraph{Baselines,  training, and evaluation.}
As baselines, we mainly focus on 4 SOTA pruning methods, \ding{172} IMP \cite{frankle2018lottery}, \ding{173} OMP \cite{frankle2018lottery},
% \SL{[refs; be consistent with earlier sections]}
 \ding{174} {\grasp} \cite{wang2019picking} (a one-shot pruning method by analyzing gradient flow at initialization), and \ding{175} {\hydra} \cite{sehwag2020hydra} (an optimization-based pruning method that optimizes masking scores). It is worth noting that there exist various implementations of IMP, \textit{e.g.}, specified by different learning rates and model initialization or `rewinding' strategies \cite{Renda2020Comparing}. To make a fair comparison, we follow the recent IMP benchmark in \cite{ma2021sanity}, which can find the best winning tickets over current heuristics-based pruning baselines.
We also remark that {\hydra} is originally proposed for improving the adversarial robustness of a pruned model, but it can be easily customized for standard pruning when setting the adversary's strength as $0$ \cite{sehwag2020hydra}. 
We choose {\hydra} as a baseline because it can be regarded as a single-level variant of {\biprune} with
%given by a single-level sparse mask optimization task together with 
post-optimization weight retraining.
When implementing {\biprune}, unless specified otherwise, we use the $1$-step SGD in \eqref{eq: theta_step}, and set the learning rates $(\alpha, \beta)$ and the lower-level regularization parameter $\gamma$ as described in the previous section. 
When implementing baselines, we follow their official repository setups.
We evaluate the performance of all methods mainly from two perspectives: 
(1) the test accuracy of the sub-network, and (2) the runtime of pruning to reach the desired sparsity. 
We refer readers to Tab.\,\ref{tab: training_details} and Appendix\,\ref{app: training} for more training and evaluation details, such as training epochs and learning rate schedules.
%, and etc. 
% {We emphasize that except for Fig.\,\ref{fig: structured_performance_cifar}, we adopt the unstructured pruning as our default pruning setting in the main paper. 
% % The other experimental results, without further mentioning, belong to the unstructured pruning regime.
% } 

% In unstructured pruning settings, we compare {\biprune} with various heuristics-based and optimization-based baselines, including IMP\,\cite{frankle2019stabilizing}, OMP, \grasp\,\cite{wang2019picking}, and \hydra\,\cite{sehwag2020hydra}. To make a fair comparison, we adopt the recommended training settings from their papers and we adopt the SOTA implementation following\,\cite{ma2021sanity} for IMP and OMP. {\hydra} is an optimization-based baseline framework, which is originally designed for robust pruning, but can be customized to standard pruning as mentioned in its paper\,\cite{sehwag2020hydra}. 
%For complete and detailed training details please refer to Appendix\,\ref{app: training}.

% \begin{wrapfigure}{r}{85mm}
% \vspace*{-5mm}
% \centerline{
% \begin{tabular}{cc}
% \hspace*{0mm}\includegraphics[width=.3\textwidth,height=!]{figure/Global_Pruning_on_TinyImageNet_ResNet18.pdf}  
% &\hspace*{-6mm}\includegraphics[width=.3\textwidth,height=!]{figure/Global_Pruning_on_ImageNet_ResNet18.pdf}
% \\
% \hspace*{2mm}\footnotesize{(a) Tiny-ImageNet with ResNet-18} &   \footnotesize{(b) ImageNet with ResNet-50}
% \end{tabular}}
% % \vspace*{-2mm}
% \caption{\footnotesize{
% Unstructured pruning test accuracy (\%) v.s. sparsity (\%) on Tiny-ImageNet and ImageNet. Other settings remain the same as Fig.\,\ref{fig: unstructured_performance_cifar}.
% % Models are pruned up to $90\%$ following\,\cite{ma2021sanity}. 
% \YH{ImageNet is still incomplete.}}}
%   \label{fig: unstructured_performance_imagenet}
% %   \vspace*{-4mm}
% \end{wrapfigure}


% We consider two different structured pruning settings with different pruning granularity of a convolutional layer,  termed filter-wise and channel-wise pruning. In general, the parameters of a convolutional layer have a shape of [$c_{\text{out}}$, $c_{\text{in}}$, w, h], which denote the output channel number, input channel number, kernel width and kernel height respectively.
% The filter-wise pruning\,\cite{chen2022coarsening} remove the model 
% parameters following a basic pattern of [$c_{\text{in}}$, w, h] while the channel-wise following [$c_{\text{out}}$, w, h]. The sparsity ratio of each layer is kept the same as the target sparsity $p\%$. Please refer to Fig.\,\ref{fig: illustration} for illustration on the two settings.
% We choose the OMP and IMP as our baselines in both structured pruning settings. Due to the page limit, we only report the results of filter-wise pruning in the main paper and include the channel-wise in Appendix\,\ref{app: add_results}, while the both settings lead to consistent conclusions.


% \paragraph{Evaluation Setups.}
% We mainly evaluate the performance of {\biprune} and the other baselines from two perspectives. 
% %As our method is dedicated to achieve high pruning accuracy (like IMP) with less computational burden (like OMP), we
% particularly pay attention to the following two metrics:
% % to the quality of the sparse networks and the pruning efficiency.
% % evaluate the quality of the found sparse network (see \ding{182}-\ding{183}) and the pruning efficiency (see \ding{184}) when evaluating a method. In particular, we pay attention to the following metrics: 
% (1) the test accuracy of the obtained sub-network, and (2) the runtime of pruning to reach the desired sparsity. 

%  (How good?) the quality of the sub-networks: besides the test accuracy of the target sparsity, we also study the best winning tickets and the sparsest winning tickets that can be found by each method across different sparsities. The former reveals the maximum potential of a pruning method to improve the test accuracy over the dense model. The latter depicts how sparse the method can go without losing any accuracy.
% % : the improvement on the test accuracy of the best winning ticket compared to dense model. \ding{183} (How sparse?) the sparsest winning ticket: winning ticket with the largest sparsity found by each method 
% \ding{183} (How fast?) pruning efficiency: this includes the required time to reach the given sparsity as well as to find the best/sparsest winning tickets.
% % reach the given sparsity as well as 
% % this includes the time spent for finding the sparsest winning ticket and for the whole pruning process. For structured pruning in particular, we also compare the inference efficiency (FLOPs) of the found sparse networks.

\vspace*{-0.1in}
\subsection{Experiment Results}

\vspace*{-0.1in}
\paragraph{{\biprune}   identifies high-accuracy winning tickets.} 
In what follows, we look at the quality of winning tickets identified by {\biprune}.
%\textit{pruning trajectory} (given by test accuracy vs. pruning ratio) of {\biprune} and baseline methods.
\textit{Two  key observations} can be drawn from our results: (1)~{\biprune}   finds winning tickets of higher accuracy and/or higher  sparsity than  the baselines in most cases (as shown in Fig.\,\ref{fig: unstructured_performance_cifar} and Tab.\,\ref{tab: sparsest_wt}); (2)~The superiority of {\biprune} holds for both unstructured pruning and structured pruning (as shown in Fig.\,\ref{fig: structured_performance_cifar} and Fig.\,\ref{fig: structured_performance_cifar_appendix}
% \SL{, and xxx}
). 

% \begin{table}[htb]
% \centering
% \caption{\footnotesize{The sparsest winning tickets found by different methods at different data-model setups. In each cell, $p\%$ ($t$ min) represents the sparsity as well as the time consumption to find the sparsest winning ticket. {\xmark} signifies that no winning ticket  is found  by a   pruning method. Given the data-model setup (\textit{i.e.}, per column),
% the sparsest winning ticket is highlighted in \textbf{bold}.
% \SL{[remove computation time from this table?]
% \SL{[wrap table?]}
% \SL{$aa, +bb$}
% }
% }}
% \label{tab: sparsest_wt}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{c|cccccc}
% \toprule[1pt]
% \midrule
% \multirow{2}{*}{Method} & \multicolumn{4}{c}{CIFAR-10}                               & \multicolumn{2}{c}{CIFAR-100} \\
%                         & ResNet-18    & ResNet-20    & ResNet-56    & VGG-16        & ResNet-18    & ResNet-20      \\ \midrule
% IMP        &  87\% (620 min) &\textbf{74}\% (200 min) & \textbf{74}\% (462 min) & 89\% (501 min) &  87\% (620 min) & \xmark       \\ % Grasp ResNet56 104 min
% OMP                     & 49\% (69 min) & \xmark & \xmark & 20\% (50 min) & 74\% (69 min)       & \xmark         \\
% \grasp                  & \xmark & \xmark & 36\% (104 min) & \xmark & \xmark       & \xmark         \\
% {\hydra}                & \xmark       & \xmark       & 20\% (188 min) & 87\% (108 min)  & \xmark       & 20\% (86 min)   \\
% {\biprune} & \textbf{89}\% (86 min)  & 67\% (65 min)  & \textbf{74}\% (179 min)  & \textbf{93}\% (118 min) &  \textbf{89}\% (86 min) & \textbf{49}\% (65 min) \\ \midrule
% \bottomrule[1pt]
% \end{tabular}%
% }
% \end{table}

% \begin{table}[htb]
% \centering
% \caption{\footnotesize{The sparsest winning tickets found by different methods at different data-model setups. \YY{Winning tickets refer to the sparse models with close performance to the dense ones.} In each cell, $p\%$ ($acc \pm std \%$) represents the sparsity as well as the test accuracy. The test accuracy of dense models can be found in the header. {\xmark} signifies that no winning ticket  is found  by a   pruning method. Given the data-model setup (\textit{i.e.}, per column),
% the sparsest winning ticket is highlighted in \textbf{bold}.
% % \SL{[remove computation time from this table?]
% % \SL{[wrap table?]}
% % \SL{$aa, +bb$}
% % \YY{Dense +-}
% % }
% \YY{test accuracy and std}
% }}
% \label{tab: sparsest_wt}
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{c|cccccc}
% \toprule[1pt]
% \midrule
% \multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10}                               & \multicolumn{2}{c}{CIFAR-100} \\
%                         & ResNet-18    & ResNet-20    & ResNet-56    & VGG-16        & ResNet-18    & ResNet-20      \\ 
%                         & (94.77\%)      & (92.12\%)        & (92.95\%)       & (93.65\%)   & (76.67\%)   &   (68.69\%)      \\\midrule
% IMP        &  87\% (0.01\%$\uparrow$) &\textbf{74}\% (0.03\%$\uparrow$) & \textbf{74}\% (0.04\%$\uparrow$) & 89\% (0.03\%$\uparrow$) &  87\% (0.24\%$\uparrow$) & \xmark       \\ % Grasp ResNet56 104 min
% OMP                     & 49\% (0.03\%$\uparrow$) & \xmark & \xmark & 20\% (0.14\%$\uparrow$)  & 74\% (0.32\%$\uparrow$)    & \xmark         \\
% \grasp                  & \xmark & \xmark & 36\% (0.12\%$\uparrow$)& \xmark & \xmark       & \xmark         \\
% {\hydra}                & \xmark       & \xmark       & \xmark  & 87\% (0.08\%$\uparrow$)  & \xmark       & 20\% (0.25\%$\uparrow$)  \\
% {\biprune} & \textbf{89}\% (0.02\%$\uparrow$) & 67\% (0.02\%$\uparrow$) & \textbf{74}\% (0.18\%$\uparrow$) & \textbf{93}\% (0.1\%$\uparrow$) &  \textbf{89}\% (0.02\%$\uparrow$)  & \textbf{49}\% (0.09\%$\uparrow$)\\ \midrule
% \bottomrule[1pt]
% \end{tabular}%
% }
% \end{table}



\begin{figure}[htb]
\vspace*{-3mm}
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_ResNet20.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_ResNet56s.pdf} &
    \hspace*{-5mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-10_VGG16.pdf} \\
    
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-100_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_CiFAR-100_ResNet20s.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_TinyImageNet_ResNet18.pdf} &
    \hspace*{-5mm} \includegraphics[width=.25\textwidth,height=!]{figure/unstructured/Global_Pruning_on_ImageNet_ResNet50.pdf}
\end{tabular}}
\vspace*{-3mm}
\caption{\footnotesize{Unstructured pruning trajectory given by test accuracy (\%) vs. sparsity (\%) on various dataset-model pairs.
The proposed \textcolor{Green}{\biprune} is compared with \textcolor{blue}{\hydra}\,\cite{sehwag2020hydra}, \textcolor{orange}{IMP}\,\cite{ma2021sanity}, \textcolor{ompcolor}{OMP}\,\cite{ma2021sanity}, \textcolor{Purple}{\grasp}\,\cite{wang2019picking}. And the performance of   dense model and that of the best winning ticket  are marked using   dashed lines in each plot. 
The solid line and shaded area of each pruning method represent  the mean and variance of test accuracies over 3 independent trials. We observe that
{\biprune}  consistently outperforms the other baselines.
Note in the (ImageNet, ResNet-50) setting, we only compare {\biprune} with our strongest baseline IMP due to computational resource constraints.
}}
\vspace*{-3mm}
\label{fig: unstructured_performance_cifar}
\end{figure}



\underline{Fig.\,\ref{fig: unstructured_performance_cifar}} shows the \textit{unstructured pruning trajectory} (given by test accuracy vs. pruning ratio)
% \todo{should we say ``pruning ratio'' instead of ``sparsity ratio'' to be consistent \YH{solved}}
of {\biprune} and baseline methods   in $8$ model-dataset setups.  For comparison, we also present the performance of the original dense model. 
As we can see, the proposed   {\biprune} approach finds the best winning tickets  (in terms of the highest accuracy) compared to the baselines across  all the pruning setups. Note that a winning ticket refers to a sparse model with test accuracy that is at least as good as the dense model (see the marked green dash line). Among the baseline methods, IMP is the  pruning method  most competitive to ours. However, the improvement brought by {\biprune}  is significant with respect to the variance of IMP, except for the $60\% $-$80\%$ sparsity regime in (CIFAR-10, ResNet-20). In the case of (CIFAR-100, ResNet-20)  where IMP can not find any winning tickets (as confirmed by\,\cite{ma2021sanity}),
{\biprune} still manages to find winning tickets with around $0.6\%$ improvement over the dense model.
In \underline{Tab.\,\ref{tab: sparsest_wt}},
we summarize the sparsest  winning tickets along the pruning trajectory identified by different pruning methods.  As we can see, 
{\biprune} can identify the winning tickets with higher sparsity levels than the other methods, except in the case of (CIFAR-10, ResNet-20). 
We also refer readers to Appendix\,\ref{app: add_results} for more experimental results to justify the high quality of winning tickets identified by {\biprune}.

\begin{table}[htb]
\vspace*{-2mm}
\centering
\caption{\footnotesize{The sparsest winning tickets found by different methods at different data-model setups. {Winning tickets refer to the sparse models with an average test accuracy no less than the dense model.} In each cell, $p\%$ (acc$\pm$std\%) represents the sparsity as well as the test accuracy. The test accuracy of dense models can be found in the header. {\xmark} signifies that no winning ticket  is found  by a   pruning method. Given the data-model setup (\textit{i.e.}, per column),
the sparsest winning ticket is highlighted in \textbf{bold}.
}}
\label{tab: sparsest_wt}
\vspace*{-2mm}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c}
\toprule[1pt]
\midrule
\multirow{3}{*}{Method} & \multicolumn{4}{c}{CIFAR-10}                               & \multicolumn{2}{|c}{CIFAR-100} \\
                        & ResNet-18                 & ResNet-20                         & ResNet-56                         & VGG-16                        & ResNet-18                 & ResNet-20      \\ 
                        & (94.77\%)                 & (92.12\%)                         & (92.95\%)                         & (93.65\%)                     & (76.67\%)                 &   (68.69\%)      \\\midrule
IMP                     &  87\% (94.77$\pm$0.10\%)  &\textbf{74}\% (92.15$\pm$0.15\%)   & \textbf{74}\% (92.99$\pm$0.12\%)  & 89\% (93.68$\pm$0.05\%)       & 87\% (76.91$\pm$0.19\%)   & \xmark       \\ % Grasp ResNet56 104 min
OMP                     & 49\% (94.80$\pm$0.10\%)    & \xmark                            & \xmark                            & 20\% (93.79$\pm$0.06\%)       & 74\% (76.99$\pm$0.07\%)   & \xmark         \\
\grasp                  & \xmark                    & \xmark                            & 36\% (93.07$\pm$0.34\%)           & \xmark                        & \xmark                    & \xmark         \\
{\hydra}                & \xmark                    & \xmark                            & \xmark                            & 87\% (93.73$\pm$0.03\%)       & \xmark                    & 20\% (68.94$\pm$0.17\%)  \\
{\biprune}              & \textbf{89}\% (94.79$\pm$0.15\%)   & 67\% (92.14$\pm$0.15\%)  & \textbf{74}\% (93.13$\pm$0.04\%)  & \textbf{93}\% (93.75$\pm$0.15\%)&  \textbf{89}\% (76.69$\pm$0.18\%)  & \textbf{49}\% (68.78$\pm$0.10\%)\\ \midrule
\bottomrule[1pt]
\end{tabular}%
}
% \vspace*{-3mm}
\end{table}


\underline{Fig.\,\ref{fig: structured_performance_cifar}} demonstrates the \textit{structured pruning trajectory}  on the CIFAR-10/100 datasets.
Here we focus on filter pruning, where the filter is regarded as a masking unit in \eqref{eq: prob_bi_level}. We refer readers to Appendix\,\ref{app: add_results} for  channel-wise pruning results.
% Due to the page limit, we only report the results of the filter-wise pruning in the main paper and please refer to Appendix\,\ref{app: add_results} for channel-wise pruning. 
%Fig.\,\ref{fig: structured_performance_cifar} shows the performance overview of structured pruning on CIFAR-10/100. 
Compared to Fig.\,\ref{fig: unstructured_performance_cifar}, Fig.\,\ref{fig: structured_performance_cifar} shows that it becomes more difficult to find winning tickets of high accuracy and sparsity in the structured pruning, and the gap among different methods decreases. This is not surprising, since
filter pruning imposes much stricter pruning structure constraints than irregular pruning. However, {\biprune} still outperforms all the baselines. Most importantly, it identifies clear winning tickets in the low sparse regime even when IMP fails. 

\begin{figure}[b]
\vspace{-0.5mm}
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-10_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-10_ResNet20s.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-100_ResNet18.pdf} &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/structured/Filter-wise_Pruning_on_CIFAR-100_ResNet20s.pdf} \\
    
\end{tabular}}
\vspace*{-4mm}
\caption{\footnotesize{Filter pruning given by test accuracy  (\%) vs. pruning ratio (\%). 
   The visual presentation setting is  the same as Fig.\,\ref{fig: unstructured_performance_cifar}. We observe that {\biprune}   identifies winning tickets of structured pruning in certain sparsity regimes.
    }}
\vspace*{-2mm}
\label{fig: structured_performance_cifar}
\end{figure}

% As structured pruning is a more challenging setting\cite{chen2022coarsening}, all the methods drop more quickly than its unstructured counterparts. Nevertheless, {\biprune} still manages to find winning tickets in most settings. In general, {\biprune} consistently outperforms IMP and OMP in the low-sparsity regime, while the gap becomes less significant when sparsity ratio $p\% > 60\%$. As the only difference between structured and unstructured {\biprune} implementation lies in the threshold operation, the time consumption of Fig.\,\ref{fig: unstructured_performance_cifar}
%  and Fig.\,\ref{fig: structured_performance_cifar} are very similar.



\vspace*{-0.1in}
\paragraph{{\biprune} is computationally efficient.}
In our experiments, another \textbf{key observation} is that 
{\biprune} yields sparsity-agnostic runtime complexity while IMP leads to runtime exponential to the target sparsity.
% \todo{``exponential runtime'' is a big claim. is there a citation for that? With $T$ pruning rounds, runtime is only $T\times$ more, right? \\
% \YY{If we fix the pruning ratio of each pruning round to $r\%$ and want to reach the sparsity $p\%$, we need to prune $\log_{(1-r\%)}(1-p\%)$ rounds. Then the total consumption time will become like Figure 5.}
% }
\underline{Fig.\,\ref{fig: time_compare_res18c10}} shows the computation cost of different methods versus pruning ratios on (CIFAR-10, ResNet-18). 
For example, {\biprune} takes 86 mins to find the sparsest winning ticket (with $89\%$ sparsity in Tab.\,\ref{tab: sparsest_wt}). 
\begin{wrapfigure}{r}{50mm}
%\vspace*{-5mm}
\centerline{
\includegraphics[width=.3\textwidth,height=!]{figure/time_comparison_cifar10_resnet18.pdf}
}
\vspace*{-4mm}
\caption{\footnotesize{Time consumption comparison on (CIFAR-10, ResNet-18) with different pruning ratio $p$. 
% The sparsest winning tickets (WT) of {\biprune} and IMP are marked in red star. 
% {\biprune} achieves sparser winning tickets (89\% v.s. 87\% and using $7\times$ less time than IMP.
% which are with 83\% sparsity. IMP achieves similar performance (see Fig.\,\ref{fig: unstructured_performance_cifar}).to {\biprune} but spends 7 times more training time.
}}
\label{fig: time_compare_res18c10}
\vspace*{-5mm}
\end{wrapfigure}
This yields
$7\times$ less runtime than IMP, which consumes $620$ mins to find a comparable winning ticket with $87\%$ sparsity. 
Compared to the optimization-based baseline {\hydra}, {\biprune} is more efficient as it  does not rely on the extra post-optimization retraining; see Tab.\,\ref{tab: efficiency} for a detailed summary of runtime and number of training epochs required by different pruning methods. 
Further, {\biprune} takes about {1.25 $\times$} more computation time   than {\grasp} and OMP. However, the latter methods lead to worse pruned model accuracy, as demonstrated by their failure to find
%\textit{e.g.}, justified by the failure cases of finding
winning tickets  in  Tab.\,\ref{tab: sparsest_wt}, Fig.\,\ref{fig: unstructured_performance_cifar}, and Fig.\,\ref{fig: structured_performance_cifar}.
% \SL{[Refer to appendix for more results or details?]}

\vspace*{-0.1in}
\paragraph{Rewinding effect on {\biprune}.} 
Another advantage of {\biprune} is that it is \textit{not} sensitive   to  model rewinding. 
Recall that 
rewinding is a strategy used in LTH \cite{frankle2020linear} to determine what model initialization should be used for re-training a pruned sparse model. As shown in \cite{ma2021sanity}, an IMP-identified winning ticket could be sensitive to the choice of a rewinding point.
\underline{Fig\,\ref{fig: ablation_study}(a)} shows the test accuracy of the {\biprune}-pruned model       when it is retrained at different rewinding epochs, where `N/A' in the x-axis represents the case 
%\begin{wrapfigure}{r}{47mm}
of no retraining (and thus no rewinding).
As we can see, a carefully-tuned rewinding scheme does not lead to a significant improvement over {\biprune} without retraining. This suggests that the subnetworks found by {\biprune} are already of high quality, and justifies the improved computation efficiency of   {\biprune} over {\hydra} (which requires post-optimization model retraining), as shown in Fig.\,\ref{fig: time_compare_res18c10}. %We stress that {\biprune}
%We highlight that all of our experiments results 


% \begin{wrapfigure}{r}{50mm}
% %\begin{figure}[htb]
% %\vspace*{-2mm}
% \centerline{
% \includegraphics[width=.3\textwidth,height=!]{figure/Diff_Init_on_CIFAR-10_ResNet20s.pdf}
% }
% \caption{\footnotesize{The sensitivity of {\biprune} to  rewinding epochs on (CIFAR-10, ResNet-20). Each curve represents a certain sparsity level and   "N/A" in the x-asis indicates  {\biprune} without retraining.
% % \SL{Please add dense model and please remove $95.6\%$.}
% }}
% \label{fig: rewind_study}
% % \vspace*{-5mm}
% \end{wrapfigure}
% %\end{figure}


% In what follows, we show that the performance of {biprune} is sensitive to neither post-optimization retraining nor the rewinding epoch, which in contrast plays an indispensable and sensitive role in the success of IMP\,\cite{frankle2019stabilizing}.
% Fig.\,\ref{fig: rewind_study} demonstrates the test accuracy of the sparse model found by {\biprune} when further retrained with different rewinding epochs. For comparison, we also present the performance of the sparse model without retraining, which is denoted as "N/A" in the x-axis. As can be seen, rewinding and retraining in general do not bring significant improvement over the retrain-free setting, indicating the subnetworks found by {\biprune} are already of high quality. Considering that all of our baselines require retraining to further boost the performance after the mask is found (see Tab.\,\ref{tab: efficiency}), our method thus spares the time-consuming retraining and further improves the efficiency. We stress that we study four sparsity ratios from different sparse levels to make sure the conclusion is consistent.

\begin{figure}[htb]
\vspace*{-1mm}
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figure/Diff_Init_on_CIFAR-10_ResNet20s.pdf}\vspace*{-0.5mm} 
    &
    \hspace*{-5mm} \includegraphics[width=.25\textwidth,height=!]{figure/Diff_K_on_CIFAR-10_ResNet20s.pdf} \vspace*{-0.5mm}
    &
    \hspace*{-5mm}  \includegraphics[width=.25\textwidth,height=!]{figure/Diff_gamma_on_CIFAR-10_ResNet20s.pdf}\vspace*{-0.5mm}
    &
    \hspace{-5mm}   \includegraphics[width=.25\textwidth, height=!]{figure/IG_compare.pdf}\vspace*{-0.5mm}
    \\
    \footnotesize{(a)} 
    & 
    \footnotesize{(b1)} 
     & 
    \footnotesize{(b2)} 
     & 
    \footnotesize{(b3)} 
\end{tabular}}
\vspace*{-3mm}
\caption{\footnotesize{The sensitivity of {\biprune} to (a) the rewinding epochs, (b1) the lower-level step number $N$, (b2) the lower-level regularizer $\gamma$, and (b3) the contribution of the IG-term at various pruning ratios on (CIFAR-10, ResNet-20). Each curve or column represents a certain sparsity. In (a), "N/A" in the x-axis indicates {\biprune} without retraining. In (b3), we fix the $\gamma$ to 1.0 and compare the performance of the IG-involved/excluded\,\eqref{eq: GD_bi_level} {\biprune}.
}}
%\vspace*{-6mm}
\label{fig: ablation_study}
\end{figure}

\vspace*{-0.1in}
\paragraph{Sanity check of {\biprune} on specialized hyperparameters.} 


In \underline{Fig.\ref{fig: ablation_study}(b)}, we show  the sensitivity of {\biprune} to   its specialized hyperparameters at lower-level optimization, including 
the number of SGD iterations ($N$) in \eqref{eq: theta_step}, and the regularization parameter $\gamma$ in \eqref{eq: prob_bi_level}.
%and the   learning rate $\alpha$.
\underline{Fig\,\ref{fig: ablation_study}(b1)} shows the test accuracy of {\biprune}-pruned  models versus the choice of $N$. As we can see, more SGD iterations for the lower-level optimization do not improve the performance of {\biprune}. This is because in {\biprune}, the \ref{eq: theta_step} is initialized by a pre-trained model which does not ask for aggressive weight updating. The best performance of {\biprune} is achieved at $N \leq 3$. We choose $N = 1$ throughout the experiments as it is computationally lightest. 
\underline{Fig\,\ref{fig: ablation_study}(b2)} shows the performance of {\biprune} by   varying $\gamma$.
% where `$\infty$'  in the x-axis refers to the case of IG-excluded \eqref{eq: GD_bi_level} (by considering $\gamma \to \infty$ in \ref{eq: m_step}). 
As we can see, the choice of $\gamma \in \{ 0.5, 1\}$ yields the best pruning accuracy across all pruning ratios. If $\gamma$ is too small, the lack of strong convexity of lower-level optimization would hamper the convergence. 
If $\gamma$ is too large, the lower-level optimization would depart from the true model objective and causes a performance drop. 
\underline{Fig.\,\ref{fig: ablation_study}(b3)} demonstrates the necessity of the IG enhancement in {\biprune}. {We compare {\biprune} with its IG-free version by dropping the IG term in \eqref{eq: GD_bi_level}.  We observe that {\biprune} without IG (marked in blue) leads to a significant performance drop ($> 1\%$) at various sparsities.} This highlights that {\em the IG in the \eqref{eq: m_step} plays a critical role in the performance improvements obtained by {\biprune}}, justifying our novel BLO formulation for the pruning problem.
% and a significant performance drop ($> 1\%$) appears consistently in various sparsity levels. 
See Fig.\,\ref{fig: ablation_study_full} for more results on hyperparameter tuning.
% In addition, the accuracy loss encountered at   $\gamma = \infty$ also indicates the necessity of the IG enhancement in {\biprune}. 
% This is because: 1) a very small $\gamma$ does not introduce enough convexity to the lower-level objective and hurts the performance; 2) a too large regularization term intuitively deviates the true objective and also leads to performance degradation. Note that ${1}/{\gamma}$ serves as the coefficient of the IG-associated term in \eqref{eq: upper_update_final}. Thus, we further studied its contribution by manually removing the IG term in our default setting ($\gamma$=1.0), as denoted as "N/A" in the x-axis. Note this operation will make our BLO-based algorithm degrade to an alternating optimization method. 
% As can be seen, a performance drop of around $1\%$ can be spotted across different sparsity levels when compared to its IG-enhanced counterparts. Therefore, as discussed in Sec.\,\ref{bi-level prune methodology}, the IG-enhancement is necessary to good performance and can be achieved nearly for `free' thanks to the bi-linearity of the pruning variables.




%\SL{I stop here.}





% We evaluate the quality of winning tickets from the perspectives of sparsity and accuracy. In general, sparser winning tickets with better test accuracy are preferred. 
% Fig.\,\ref{fig: unstructured_performance_cifar} 
% % and Fig.\,\ref{fig: unstructured_performance_imagenet} 
% compares the performance of different methods in the unstructured pruning setting. Several observations can be drawn. Firstly, our method {\biprune} finds the winning tickets with the best test accuracy (marked by the green dashed line) across all the settings with no exceptions. 
% %\begin{wrapfigure}{r}{50mm}


% In some extreme cases, even IMP can not find any winning tickets (\emph{e.g.}, CIFAR-100 with ResNet-20, confirmed by\,\cite{ma2021sanity}), while {\biprune} still manages to find winning tickets with around $0.5\%$ improvement on the test accuracy. Secondly, as demonstrated in Tab.\,\ref{tab: sparsest_wt}, {\biprune} is able to find winning tickets with larger sparsity than other methods in most cases. Both observations suggest the quality of the sub-networks found by {\biprune} outperforms all the baselines. We compare {\biprune} with more heuristics-based init-pruning baselines in Appendix\,\ref{app: add_results}.


 

==> Deprecated_NO_USE/Version_Camera_08041600_Submission/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

==> Sec1_Old.tex <==
\section{Introduction (1 page)}

% \paragraph{Contributions.}
% Discuss the importance and the development of DNN pruning

% \fakepara{the DNN prevails and pruning is necessary}
Deep neural networks (DNNs) have dramatically revolutionized the state-of-the-art performance in various fields\,\cite{krizhevsky2012imagenet, brown2020language}. As a key to increase the generalization of the DNNs\,\cite{bartlett2021deep}, the over-parameterized structures also bring its own problem. The millions or even billions of parameters not only increase computational costs during inference, but also raise great challenges for deployment on the resource-limited devices\,\cite{han2015deep}. Thus, the model pruning techniques has become the research hot spot recent years to remove redundant parameters and reduce the model size\,\cite{han2015deep, blalock2020state}.
\SL{[Add more song han's work.]}
% Deep neural networks (DNNs) have boosted their performances in many areas, \emph{e.g.,} computer vision and natural language processing \cite{krizhevsky2012imagenet, brown2020language}. However, DNNs of increasingly large sizes, despite their generalization brought by the over-parameterization \cite{bartlett2021deep}, hinder themselves from being deployed on computational resource-limited devices \cite{han2015deep}. Therefore, pruning is proposed and has become one effective method to remove redundant parameters as for improving the inference efficiency and the storage of large DNNs \cite{han2015deep, blalock2020state}.

% \fakepara{LTH is the predominant one while too computationally expensive.}
Among numerous studies on model pruning algorithms\,\cite{lecun1989optimal, ren2018admmnn,  ramanujan2020sHiddenSubnetwork}, the heuristics-based Iterative Magnitude Pruning (IMP) is the current dominant approach to achieve model sparsity 
\SL{without suffering performance loss, as suggested and empirically justified by the Lottery Ticket Hypothesis (LTH) \cite{frankle2018lottery,Renda2020Comparing,frankle2020linear,blalock2020state,chen2020lottery,chen2021lottery}.}
% \SL{and it is justified by} the Lottery Ticket Hypothesis (LTH) serves as one of the most well-known approaches to attain sparse sub-networks without suffering performance loss. 
LTH hypothesizes the existence of a sub-network (the so-called `winning ticket'), when trained from the scratch, can match the performance of the full model. The core idea of LTH lies in repetitively calling the pruning-retraining cycle and prunes a small ratio of the remaining parameters at each round. However, the achieved winning ticket is often at the cost of \SL{much} more computations than training a dense model from scratch, which hinders its scalability towards large dataset and large model architectures. 
\todo{Is LTH an algorithm or a hypothesis that motivates algorithms like IMP? \SL{IMP is defined prior to LTH. LTH is a hypothesis to state that IMP works and can find winning tickets and suggests a formal and refined IMP pipeline to surely find these winning tickets justified by experiments.}}
To improve the efficiency of IMP, numerous heuristics-based one-shot pruning methods\,\cite{lee2018snip, frankle2018lottery,ma2021sanity,  wang2020pick, tanaka2020pruning, alizadeh2022prospect}, \emph{e.g.}, one-shot magnitude pruning (OMP), have been proposed, which directly prunes the model to the target sparsity and achieves significant speedup compared to IMP. However, all the current one-shot methods   encountered \SL{evident} performance drop, leading to small odds to find winning tickets\,\cite{ma2021sanity}.
\todo{substantiate with citations or support otherwise}

% Among numerous studies on designing model pruning algorithms \cite{lecun1989optimal, ren2018admmnn,  ramanujan2020sHiddenSubnetwork}, a rising representative study focuses on obtaining sparse subnetworks out of dense unpruned models \cite{frankle2018lottery, ma2021sanity}. It is claimed that a dense, randomly-initialized neural network contains a subnetwork (so-called "winning ticket") that can match the test accuracy of the original network after training with the same algorithm.

% IMP is the SOTA way to figure out the sparse model
% The heuristics-based iterative magnitude pruning (IMP) is one of the most promising methods to identify the "winning ticket" in model pruning \cite{ma2021sanity}. However, its repetitive training and rewinding procedures make it time-consuming and prevent it from large dataset and architecture schemes. There are also heuristics-based one-shot pruning methods \cite{ma2021sanity, frankle2018lottery, wang2020pick, lee2018snip, tanaka2020pruning, alizadeh2022prospect} that deliver efficient sparsification solutions but can hardly find winning tickets as IMP does. 

% \fakepara{current optimization-based pruning methods save time but are weak. is fundamental improvement possible?}
Another research direction is 
the optimization-based pruning methods \cite{sehwag2020hydra, ramanujan2020sHiddenSubnetwork, lee2020layer, csordas2020neural, ren2018admmnn}, which still follow the pruning-retraining paradigm and adopt sparsity regularization\,\cite{liu2019admm, wang2020neural}  or parameterized masking\,\cite{csordas2020neural, ramanujan2020sHiddenSubnetwork, sehwag2020hydra} to promote sparsity. However, current optimization-based pruning methods still suffer from a non-negligible performance gap from IMP and can hardly find the winning tickets.
\todo{substantiate with citations or support otherwise}
This motivates us to rethink the fundamentals of this research direction: can we advance the optimization basis of the optimization-based pruning and achieve comparable or even better performance than IMP?
% are then motivated to find sub-networks with better performance more efficiently. 
% These methods adopt the pruning-retraining paradigm either by the method of sparsity regularization \cite{liu2019admm, wang2020neural}  or parameterized masking \cite{csordas2020neural, ramanujan2020sHiddenSubnetwork, sehwag2020hydra}. However, they can not find winning tickets but only result in sub-networks with close performance to the dense ones. This motivates us to rethink this direction: is there any missing point that stops us from reaching the winning ticket from the optimization view?

% There are also some one-shot, init-pruned methods but can not achieve as good performance as IMP does. \textsc{OMP}\,\cite{frankle2018lottery}, \textsc{ProsPr}\,\cite{alizadeh2022prospect}, \textsc{Grasp}\,\cite{wang2020pick}, \textsc{Snip}\,\cite{lee2018snip}, \textsc{SynFlow}\,\cite{tanaka2020pruning}

% There are also optimization-based pruning, Hydra to achieve robustness, hidden network to only achieve better performance than OMP. Are there any missing points for optimization-based methods? We should rethink.

% \fakepara{BLO is good framework but algorithm is too complicated.}

\begin{wrapfigure}{r}{60mm}
\vspace*{-4mm}
\centerline{
\includegraphics[width=58mm]{figure/main_compare.pdf}
}
\caption{\footnotesize{
A performance snapshot of the proposed {\biprune} method vs. the IMP baseline and the original dense model across three pruned ResNet models (ResNet-20, ResNet-56, and ResNet-18) with 74\% sparsity on CIFAR-10. The marker size indicates the model size (\textit{i.e.}, the remaining model parameters). And the uni-color   region corresponds to the same model type used by different pruning methods.
% of test accuracy of pruned models (with 74\% sparsity) and 
% CIFAR-10 test accuracy and training time of three different network architectures by {\biprune} and IMP at the sparsity ratio of 74\%.
% % compared to dense models. 
% The size of markers indicates model parameter counts.
}}
\label{fig: intro}
\vspace*{-4mm}
\end{wrapfigure}


To tackle the above challenge, we revisit the pruning problem from a fresh and novel viewpoint of bi-level optimization (BLO). 
In the new formulation, we show that BLO provides a technically-grounded optimization basis for an efficient implementation of the pruning-retraining learning paradigm. 
% In the new formulation, the pruning and retraining tasks are cast as the upper- and lower-level problem with disentangled variables and objectives. 



To the best of our knowledge, this is the first work making a rigorous connection between pruning and BLO. Technically, we propose a novel \textbf{bi}-level optimization-enabled \textbf{p}runing method (termed {\biprune}).  We further show {\biprune} takes advantage of the bi-linearity of the pruning variables and avoids the computationally intensive nature of the common BLO methods. More specifically, {\biprune} can be solved as easily as the first-order alternating optimization problem. Practically, extensive experiments demonstrate the superiority of the proposed {\biprune} in terms of accuracy, sparsity, and efficiency. {\biprune} achieves the best winning tickets in all settings with only OMP-level time consumption. As Fig.\,\ref{fig: intro} shows, {\biprune} achieves winning tickets with 5$\times$ speedup compared to IMP on CIFAR-10 with ResNet-18 in the sparsity of 74\%.
\todo{MINOR: in fig~\ref{fig: intro} make axis labels, legend and arch name larger}

% Inspired from studies that apply parameterized masks to search better sub-networks, we propose the first study into bi-level optimization based pruning ({\biprune}), separating the mask searching and the model weight tuning. Such disentanglement indicates the flexibility to use mismatched pruning and retraining objectives. On the other hand, the bi-level architecture enables the coupling between model weights and pruning masks through the implicit gradient-based routine.

% Hydra style; Layer-wise style; Chen Fan literature mentioned Bernoulli based masking; These studies inspired us to rethink optimization-based pruning from a bi-level point of view, which disentangles weights and masks naturally, and enjoys the benefits of the more accurate estimation of upper-level gradients. 

% \fakepara{Our technical summary on BLO with bi-linear nature.}

% However, BLO generally brings in extra computational costs, which may hinder the efficiency by optimization-based pruning. We will show in Sec.\,\ref{bi-level prune methodology} that, thanks to the bi-linearity of {\biprune} optimizes, the second-order derivative introduced by the implicit gradient can be solved as easily as the first-order derivative only alternative optimization. We further demonstrate that, with extensive experiments, BLO not only brings sparser and more accurate winning ticket, but also improves the efficiency of the whole process. As shown in Fig.\,\ref{fig: unstructured_performance_cifar}, our {\biprune} method consistently outperforms other methods in terms of accuracy, sparsity, and efficiency. 

% Thanks to the bi-linear formulation brought by the coupling of the masks and weights, we can come to the first-order derivative only form to solve the pruning-retraining pipeline. 



% Finally, we conclude experimental results on both structured and unstructured pruning with 5 model architectures and 4 popular datasets. We show that 



Our main contributions are listed as the following aspects:

\noindent $\bullet$ (Formulation-wise) We reformulate the model pruning problem as a bi-level optimization (BLO) problem. We show that the new formulation not only advances the optimization foundation of the pruning problem, but also provides a natural interpretation of the widely-accepted pruning-retraining paradigm. More importantly, the new formulation disentangles model pruning and retraining variables and provides more flexibility to design mismatched objectives at the upper and lower optimization levels.
% To our best knowledge, we are the first to rethink the optimization-based pruning from a bi-level point of view. We show that the bi-level optimization (BLO) not only inherits the spirit of the pruning-retraining paradigm but also brings in the design flexibility for model pruning.

\noindent $\bullet$ (Algorithmic-wise), we propose a new pruning algorithm {\biprune} based on our new BLO formulation and the implicit gradient theory. Different from the ordinary computationally intensive BLO methods, we theoretically show that {\biprune} can be solved as easily as the first-order optimization by taking advantage of the bi-linear nature of the pruning variables. 
% We propose the bi-level pruning (BiP) algorithm and prove that the implicit gradient (IG) term brought by the bi-level formulation can be solved with only first-order derivatives. The bi-linearity of the pruning problem optimizes allows simplification of the IG computation, accelerating the execution of {\biprune}.  

\noindent $\bullet$ (Experiment-wise) We conduct extensive experiments across 4 datasets (CIFAR-10/100, Tiny-ImageNet and ImageNet), 5 model architectures, and 2 pruning settings (unstructured and structured pruning). We show that {\biprune} combines the high accuracy of the predominant iterative magnitude pruning (IMP) and the high efficiency of the one-shot pruning schemes. Specifically, (i) {\biprune} achieves higher test accuracy than IMP and finds the best winning tickets in all settings. (ii) {\biprune} enjoys high pruning efficiency (comparable to one-shot pruning schemes), and achieves $2\sim7\times$ speedup over IMP for the same level of model accuracy and sparsity.
% We conduct extensive experiments to validate our method {\biprune} on diverse datasets (\emph{i.e.,} CIFAR-10/100, Tiny-ImageNet, and ImageNet) across multiple network architectures, including various ResNets and VGG. Specifically, our unstructural winning tickets achieve up to 2\% improvement over the unpruned dense models and 3-7$\times$ speedup compared to IMP for the same level of model accuracy and sparsity.


\clearpage

==> Sec3_SL.tex <==
In this section, we begin by providing a brief   background of neural  network pruning, including the predominant   iterative magnitude pruning (IMP) method and the 
associated lottery ticket hypothesis (LTH)
\cite{frankle2018lottery} to find high-quality subnetworks (known as `winning tickets') that--when trained in isolation--reach test accuracy comparable to or even better than the original dense network. 
However, the superior performance of IMP is accompanied by a prohibitive computation cost, as will be exemplified in Fig.\,\ref{fig: one_shot_results}. In  order to overcome the computational difficulty of IMP, we next introduce the  one-shot pruning method and elaborate on its comparison with IMP. Spurred by the pros and cons of current pruning methods, we eventually state the problem to be studied in this paper. 
 

\paragraph{{Heuristics-based IMP.}}
The heuristics-based IMP is the  currently prevailing approach  to
identify the `winning ticket' in model pruning, so as to attain model sparsity without suffering  performance loss\,\cite{blalock2020state,frankle2018lottery,Renda2020Comparing,frankle2020linear,chen2020lottery,chen2021lottery}. 
For example, the current  state-of-the-art (SOTA) implementation of IMP in \cite{ma2021sanity} can lead to a pruned ResNet-20 on
% \SL{[This example  number needs to be   better aligned with the later figure, then you can cite it here.]}
CIFAR-10 with 74\% sparsity and $92.12\%$ test accuracy, {
which is comparable to the performance of the original dense model}; see Fig.\,\ref{fig: one_shot_results}. 
% For the larger-size {ResNet-18} model, IMP   can identify a sparser network with   {$95\%$ sparsity and $94.81\%$ test accuracy, yielding the $0.5\%$ improvement over the original dense model}; \SL{see Fig.\,xxx in Sec.\,xxx}.
The algorithm of IMP typically contains two key ingredients: \textbf{(i)} a \textit{temporally-evolved pruning schedule} (given by the growing model sparsity over pruning iterations), and \textbf{(ii)} the \textit{pruning-retraining learning mechanism} applied at each pruning round. 
% To be more specific, 
% IMP  repeatedly trains, prunes, and resets the network over multiple rounds (say $n$ rounds). 
For (i), supposing that there exist $n$ pruning rounds, each round  prunes $(p\%)^{\frac{1}{n}} $ of the model
weights that survive the previous round, where $p\%$ denotes the final pruning ratio to be achieved.
%This leads to a pruning mask $\mathbf m$ at each round. 
For (ii), 
the non-zero remaining weights at each pruning round are re-set to the  weights at initialization or at an early-training epoch \cite{Renda2020Comparing}, and   re-trained till convergence. 
In brief, IMP  repeatedly trains, prunes, and resets the network over multiple rounds. 

 

% A common example, the Lottery Ticket Hypothesis (LTH), can achieve comparable or even better performance with a sparsity of over $95\%$ in its state-of-the-art (SOTA) implementation\,\cite{ma2021SanityCheckLTH}. 
% In general, the heuristics-based IMP adopts a sparsifying-retraining paradigm which consists of multiple iterative cycles: \underline{\textit{(1)}} \textbf{training} dense model with several epochs; \underline{\textit{(2)}} \textbf{pruning} $p\%$ redundant model weights with certain heuristics-based criteria (\emph{e.g.} model weight magnitude) to obtain the new mask; \underline{\textit{(3)}} \textbf{fine-tuning} the sparse network with the found mask and rewound weights for accuracy recovery. 

\begin{wrapfigure}{r}{85mm}
\vspace*{-5mm}
\centerline{
\begin{tabular}{cc}
\hspace*{0mm}\includegraphics[width=.3\textwidth,height=!]{figure/performance_comparison.pdf}  
&\hspace*{-4mm}\includegraphics[width=.31\textwidth,height=!]{figure/time_comparison_long.pdf}
% \\
% \hspace*{2mm}\footnotesize{(a) Test accuracy vs. pruning ratio.} &   \footnotesize{(b) Runtime of pruning.}
\end{tabular}}
\vspace*{-2mm}
\caption{\footnotesize{
Illustration of the pros and cons of different pruning methods executed over (ResNet-20, CIFAR-10).
(a) Test accuracy vs. different pruning ratios: IMP significantly outperforms one-shot pruning methods (\textsc{OMP}\,\cite{frankle2018lottery}, \textsc{ProsPr}\,\cite{alizadeh2022prospect}, \textsc{Grasp}\,\cite{wang2020pick}, \textsc{Snip}\,\cite{lee2018snip}, \textsc{SynFlow}\,\cite{tanaka2020pruning}). (b) Computation time of pruning to different sparsity levels:  IMP becomes much more computational intensive when pruning is targeted for a higher sparsity level. 
%We highlight we adopt the SOTA implementation of OMP  following\,\cite{ma2021sanity} and other methods following their original settings.
% \SL{For (a): Update x-y axis and mark the $95\%$ or $99\%$ pruning point.}
% \SL{For (b): [X-axis: Pruning method, add the dense model training time.]}
% \SL{Illustration of  the pros and cons of different pruning methods executed over (ResNet-xxx, CIFAR-10).
% (a) Test accuracy against pruning ratio: IMP significantly outperforms one-shot pruning methods (OMP [refs], ....). (b) Computation time of pruning to different sparsity levels:  IMP becomes much more computational intensive when pruning is targeted for a higher sparsity level ($99\%$ vs. $60\%$).
% }
% Performance and efficiency comparison between IMP (LTH) and various one-shot pruning methods on CIFAR10 and ResNet20. One-shot methods save pruning time at the cost of significant performance drop compared to IMP (LTH).
% \SL{Why ResNet20? Not ResNet18?}
}}
  \label{fig: one_shot_results}
  \vspace*{-7mm}
\end{wrapfigure}

%\SL{[I stop here]}
Yet, the superior pruning accuracy   of IMP is at the cost of  computation efficiency. For ease of illustration, Fig.\,\ref{fig: one_shot_results} shows the example of pruning ResNet-20 over CIFAR-10 and demonstrates   the accuracy and the computation time of various pruning methods versus the growing sparsity ratio.
%and (b) the computation time of model pruning with different sparsity levels.
% \SL{For ease of illustration, Fig.\,\ref{fig: one_shot_results} shows a pruning example that unveils (a) the accuracy performance of various pruning methods versus the growing sparsity ratio, and (b) the computation time of model pruning with different sparsity levels.}
As we can see, IMP outperforms   the other pruning baselines and finds 
the sparsest winning ticket (marked by the red star in Fig.\,\ref{fig: one_shot_results}a) using $n = 6$ pruning rounds. 
However, this leads to $3\times$ more than the cost of training a dense model from scratch.
% \SL{the $95\%$-sparsity ResNet-18 model with $94.81\%$ test accuracy on CIFAR-10 takes $n = xxx$ pruning rounds. This leads to $xxx$-min runtime, which is $xxx$ times higher than training a dense model and $xxx$ times higher than pruning to the $60\%$  sparsity level.} 
%and thus hampers the pruning efficiency 
%
\iffalse
Although IMP-based pruning approaches have become the rising star sub-field in pruning, its current success largely sacrifices the pruning efficiency. Within each pruning cycle, the sparse structure is obtained by removing a small fixed pruning ratio (\emph{e.g.}, $20\%$ in LTH) of the \textbf{remaining weights} to make the final sparse model match the full performance of the dense model. Thus, the required pruning iterative numbers as well as their training time grow exponentially as the sparsity increases. For example, the SOTA implementation of LTH\,\cite{ma2021SanityCheckLTH} has to go through 22 pruning cycles to arrive at a sparsity of $99\%$. In such a case, the immense training time consumption has become one clear obstacle of IMP from scaling to large model architectures and datasets\,\cite{zhang2021efficient}.
\fi 
%
\paragraph{IMP vs. one-shot pruning.}
To reduce the computation cost of IMP, different kinds of `accelerated' pruning methods were developed \cite{frankle2018lottery,lee2018snip, wang2020pick,tanaka2020pruning, alizadeh2022prospect, zhang2021efficient}; And many of them
  fall into the \textit{one-shot pruning} category: The network is directly pruned to the eventual target sparsity level  and retrained once. 
%: the network is trained once, p% of weights are pruned, and the surviving weights are reset.
% which refines the sparse mask directly to the given sparsity only one time. 
In particular, the one-shot magnitude pruning (OMP) has served as an important baseline that  simplifies IMP directly \cite{frankle2018lottery}.
\textsc{OMP} obeys the pruning-retraining paradigm, but it  prunes the model to the target sparsity using only one pruning round. 
% \SL{Although some existing work\,\cite{ma2021SanityCheckLTH} observed that OMP and the other one-shot pruning methods (e.g., ProsPr\,\cite{alizadeh2022prospect}) could find winning tickets and achieve similar accuracy performance to IMP. However, this conclusion is model/dataset-specific. }
% Although some preliminary results showed that 
% existing work\,\cite{ma2021sanity}(\YH{cite TBD}) observed that OMP and the other one-shot pruning methods (e.g., \textsc{ProsPr}\,\cite{alizadeh2022prospect}) could find winning tickets and achieve similar accuracy performance to IMP at low sparsity levels. However, this conclusion is model/dataset-specific. 
However,  the promise of current one-shot pruning methods is dataset/model-specific \cite{ma2021sanity, su2020sanity_random_win} and mostly lie in the low-sparsity regime \cite{alizadeh2022prospect}.
As systematically studied in \cite{ma2021sanity, frankle2020pruning}, there exists a clear performance gap between one-shot pruning and IMP.
Fig.\,\ref{fig: one_shot_results} also justifies the above limitation.
% However, the degradation in accuracy of the one-shot methods is still significant compared to IMP (LTH), making them impractical to real world applications\,\cite{frankle2020pruning}.
As we can see, although one-shot pruning  is   computationally light (Fig.\,\ref{fig: one_shot_results}b), it suffers from an evident accuracy drop compared to IMP (Fig.\,\ref{fig: one_shot_results}a), especially at the large sparsity levels.
%For example, \textsc{OMP} and \textsc{ProsPr} \cite{alizadeh2022prospect}, the SOTA methods of one-shot pruning,   yield  over $2\%$ and $10\%$ accuracy drop compared to IMP at the $74\%$ and  $98\%$ sparsity level, respectively.
Thus,  there exists a strong demand for the algorithmic advancement of model pruning that can   enjoy the dual advantages of one-shot pruning and IMP.
%\textit{i.e.}, improve the tradeoff  between computation efficiency and pruning accuracy. 
% Even the SOTA one-shot pruning method \textsc{ProsPr}\,\cite{alizadeh2022prospect} also suffers from an accuracy drop of over $10\%$ compared to IMP when $99\%$ parameters are pruned.
% As demonstrated in Figure\,, all one-shot  
%\todo{I don't see 99\% sparsity level in Figure~\ref{fig: one_shot_results}. Do we mean 90\%?
%
%\YY{Solved.}}
%
%the observed accuracy-efficiency tradeoff
%the accuracy-efficiency tradeoff of one-shot pruning is based on the heuristics-based one-shot pruning 
%This efficiency-performance trade-off is primarily due to the heuristic nature, which is insufficient to find satisfactory masks with an extreme sparsity using the radical pruning ratio as OMP does.
%
\paragraph{Problem Statement.}
As described above, the existing  one-shot pruning methods do not suffice to close the performance gap with IMP. One possible root cause is its strong   dependence   on  the heuristics-based weight sparsification strategy. This leaves the question of  whether 
computation efficiency and pruning accuracy could be co-improved through a more rigorous and dedicated optimization-based approach. 
% a theoretically-grounded optimization-based approach can renovate one-shot pruning so as to improve the computation complexity of pruning while attaining the accuracy performance comparable to IMP.
% Based on the aforementioned dilemma between performance and pruning cycle number in heuristics-based pruning methods, we ask the following question:
Thus, we ask:  \textit{Beyond heuristics, how to establish the \textbf{optimization basis} of a successful pruning mechanism that can attain high pruning  accuracy (like IMP) as well as high   computation efficiency (like one-shot pruning)?}
% \begin{center}
%     \textit{Beyond heuristics, how to establish the \textbf{optimization basis} of a successful pruning mechanism that can close the gap between pruning accuracy (e.g., achieved by IMP) and computation efficiency (e.g., achieved by OMP)?}
% \end{center}


%\newpage 

